Service Rate, Busy Period & Throughput Analysis of a Horizontal Traffic Queue

We consider a horizontal traffic queue (HTQ) on a periodic road segment, where vehicles arrive according to a spatio-temporal Poisson process, and depart after traveling a distance that is sampled independently and identically from a spatial distribution. When inside the queue, the speed of a vehicle is proportional to a power $m >0$ of the distance to the vehicle in front. The service rate of HTQ is equal to the sum of the speeds of the vehicles, and has a complex dependency on the state (vehicle locations) of the system. We show that the service-rate increases (resp., decreases) in between arrivals and departures for $m<1$ (resp., $m>1$) case. For a given initial condition, we define the throughput of such a queue as the largest arrival rate under which the queue length remains bounded. We extend the busy period calculations for M/G/1 queue to our setting, including for non-empty initial condition. These calculations are used to prove that the throughput for $m=1$ case is equal to the inverse of the time required to travel average total distance by a solitary vehicle in the system, and also to derive a probabilistic upper bound on the queue length over a finite time horizon for the $m>1$ case. Finally, we study throughput under a release control policy, where the additional expected waiting time caused by the control policy is interpreted as the magnitude of the perturbation to the arrival process. We derive a lower bound on throughput for a given combination of maximum allowable perturbation, for $m<1$ and $m>1$ cases. In particular, if the allowable perturbation is sufficiently large, then this lower bound grows unbounded as $m \to 0^+$. Illustrative simulation results are also presented.

==> 02- submission/abstract.tex <==
\begin{abstract}

We consider a horizontal traffic queue (HTQ) on a periodic road segment, where vehicles arrive according to a spatio-temporal Poisson process, and depart after traveling a distance that is sampled independently and identically from a spatial distribution. When inside the queue, the speed of a vehicle is proportional to a power $m >0$ of the distance to the vehicle in front. The service rate of HTQ is equal to the sum of the speeds of the vehicles, and has a complex dependency on the state (vehicle locations) of the system. We show that the service-rate increases (resp., decreases) in between arrivals and departures for $m<1$ (resp., $m>1$) case. 
For a given initial condition, we define the throughput of such a queue as the largest arrival rate under which the queue length remains bounded. We extend the busy period calculations for M/G/1 queue to our setting, including for non-empty initial condition. These calculations are used to prove that the throughput for $m=1$ case is equal to the inverse of the 
time required to travel average total distance by a solitary vehicle in the system, and also to derive a probabilistic upper bound on the queue length over a finite time horizon for the $m>1$ case. Finally, we study throughput under a release control policy, where the additional expected waiting time caused by the control policy is interpreted as the magnitude of the perturbation to the arrival process. We derive a lower bound on throughput for a given  
combination of maximum allowable perturbation, for $m<1$ and $m>1$ cases. In particular, if the allowable perturbation is sufficiently large, then this lower bound grows unbounded as $m \to 0^+$. Illustrative simulation results are also presented.

%We then characterize stability of the configuration with uniform inter-vehicular spacings for closed (i.e., with no arrivals or departures) and open systems. Our analysis relies on dynamical properties of Kullback-Leibler divergence of the vector of inter-vehicular spacings with respect to uniform spacings, and on leveraging connections between the proposed system and processor sharing queues. We also present simulation results to illustrate phase transition in the throughput of the proposed horizontal traffic queue under nonlinear car following models. 
\end{abstract}

==> 02- submission/busy-period-properties.tex <==
\section{Busy Period Properties of the Horizontal Traffic Queue}
\label{sec:busy-period}

The system is called \emph{busy} when there is at least one vehicle on the road, or equivalently, the workload is positive. Once the system gets empty, it becomes \emph{idle} up to the time of next arrival. Thus, the system alternates between busy and idle periods. Accordingly, while the first busy period might start from a non-zero initial condition, if the first busy period terminates, then the subsequent busy periods will start from the zero initial condition. In this paper, unless otherwise stated explicitly, we shall implicitly assume a zero initial condition when referring to a busy period. 

\subsection{Expected Busy Period Duration}
The next lemma provides an expression for the expectation of the busy period duration in the linear case.

 \begin{lemma}\label{lemma:busy-period-mean}
 For any $\lambda < L/\bar \psi$, $L > 0$, $m=1$,  $\varphi \in \Phi$, $\psi \in \Psi$, the mean value of the busy period duration is equal to $\bar \psi / (L - \lambda \bar \psi)$.
% \be
% E[B]=\frac{L-\bar\varphi}{L-\lambda(L-\bar\varphi)}
% \ee
 \end{lemma}
% \ksmargin{revise the proof according to final cdc version \mmcomment{, Done}}
  \begin{proof}
A busy period, say of duration $B$, is initiated by the arrival of a vehicle, say $j$, when the system is idle. 
%Let $d_b$ be the amount of work brought to the system, i.e., the distance to be travelled, by the vehicle that starts the busy period. 
Let the number of vehicles that arrive during the busy period be $N_{bn}$. Note that $N_{bn}$ does not include the vehicle initiating the busy period. Therefore, the workload brought into the system during the busy period is equal to $w_B=\sum_{i=j}^{j+N_{bn}} d_i$.
%Let $w_B$ be the total work added to the system during a busy period of length $B$, i.e., 
%\be\label{eq:total-work-busyperiod}
%w_B=\sum_{j=1}^{N_{B}+1}(L-v_{b+j})=(N_B+1)L-\sum_{j=1}^{N_{B}+1}v_{b+j}
%\ee
%where $N_{B}$ is the number of vehicles that arrive during a busy period of length $B$.  
The expected value of $N_{bn}$ can be obtained by conditioning on the duration of the busy period: 
\be\label{eq:nb-expectation}
E[N_{bn}]=E\left[E[N_{bn}|B]\right]=E[\lambda B]=\lambda E[B]
\ee
where the second equality follows from the fact that the arrival process is a Poisson process. 
Since the event $\{N_{bn}+1=n\}$ is independent of $\{d_{j+i},i > n\}$, $N_{bn}+1$ is a stopping time for the sequence $\{d_{j+i},i\geq 1\}$. Therefore, using Wald's equation, e.g., see \cite[Theorem 3.3.2]{Ross:96}, and \eqref{eq:nb-expectation}, the expected value of the workload $w_B$ added to the system during the busy period $B$ is given by: 
\be\label{eq:wb-expectation}
E[w_B]=(E[N_{bn}]+1) \, \bar \psi=(\lambda E[B]+1) \, \bar \psi.
\ee



\begin{figure}[htb!]
 \centering
 \includegraphics[width=5.5cm]{busy-period-new-notation} 
  \caption{(a) Queue length process and (b) workload process during a busy period. }
    \label{fig:busy-period}
\end{figure}

Since the workload decreases at a constant rate $L$ during a busy period, we have $B=w_B/L$ (see Figure \ref{fig:busy-period} for an illustration). Therefore, $E[B]=E[w_B]/L$, which when combined with \eqref{eq:wb-expectation}, establishes the lemma. 
\qed
\end{proof}

%\ksmargin{is Proposition~\ref{prop:busy-prob} used anywhere in the paper ?\mmcomment{No, just a result by itself, but it has some implications. For the $\lambda>\lambda^*$, this probability is greater than one which means that system is always busy a.s.}}
%\begin{proposition}
%\label{prop:busy-prob}
%The limiting probability that the system is busy at time $t$ is given by
%\be

%\ee
%\end{proposition}
%\begin{proof}
%The queue alternates between busy and idle periods. Whenever the system gets idle we say a renewal happens since after that everything starts probabilistically again. Thus, the process is an alternating renewal process. Let $Z=B+D$ be the time between renewals where $B$ and $D$ are the duration of busy and idle periods, respectively.  Note that $Z$ is a non-lattice random variable. By using the results for the alternating renewal process and key renewal theorem, e.g., see \cite[Theorems 3.4.2 and 3.4.4]{Ross:96}, we have
%\be
%\lim_{t\to\infty}{\Pr\{\text{system busy at \emph{t}}\}}=\frac{E[B]}{E[B]+E[I]}
%\ee
%Lemma \ref{lemma:busy-period-mean} gives $E[B]$ and we know the inter-arrival times are exponential with mean $1/\lambda$, so  $E[I]=1/\lambda$. This establishes the proposition. 
%\end{proof}

%\begin{proposition}
%\label{prop:upperbound-on-mean-waitingtime}
%For any $\lambda<L/\bar \psi$, $L > 0$, $m=1$, $\varphi, \psi \in \Psi$, the mean queue length is upper bounded by $\lambda\bar \psi / (L - \lambda \bar \psi)$
%\end{proposition}
%\ksmargin{Should we just have this as a remark rather than a proposition ? In any case, the proof needs rewording}
%\begin{proof}
%It is easy to see that the mean waiting time is no more than the mean duration of the busy period. That is
%\begin{equation*}
%E[T]\leq E[B]
%\end{equation*}
%Now, we apply Little's law to the above.  Therefore, the above combined by Lemma \ref{lemma:busy-period-mean} and Little's law gives the result. 
%\end{proof}

\begin{remark}
\label{remark:waiting-time}
Since the mean busy period duration is an upper bound on the mean waiting time, Lemma \ref{lemma:busy-period-mean} also gives an upper bound on the mean waiting time. One can then use Little's law~\cite{Kleinrock:75}\footnote{Little's law has previously been used in the context of processor sharing queues, e.g., in \cite{Altman.ea:06}.} to show that the mean queue length is upper bounded by $\lambda\bar \psi / (L - \lambda \bar \psi)$.
\end{remark}

Let $\mathcal{I}(t):=\int_0^t\delta_{\{w(s)=0\}}\de s$ be the cumulative \emph{idle time} up to time $t$. The following result characterizes the long run proportion of the idle time in the linear case.
\begin{proposition}
\label{prop:long-run-idle-time}
For any $\lambda<L/\bar \psi$, $m=1$, $L > 0$, $\varphi \in \Phi, \psi \in \Psi$, the long-run proportion of time in which HTQ is idle is given by the following:
$$\lim_{t\to\infty} \frac{\mathcal{I}(t)}{t}=1-\frac{\lambda \bar \psi}{L}>0 \quad a.s.$$
\end{proposition}

\begin{proof}
HTQ alternates between busy and idle periods. Let $Z=I+B$ be the duration of a cycle that contains an idle period of length $I$ followed by a busy period of length $B$. Idle period, $I$, has the same distribution as inter-arrival times i.e. an exponential random variable with mean $1/\lambda$, and the mean value of $B$ is given in Lemma \ref{lemma:busy-period-mean}. Note that duration of cycles, $Z$, are i.i.d. random variables. Thus, the busy-idle profile of the system is an alternating renewal process where renewals correspond to the moments at which the system gets idle.  Suppose the system earns reward at a rate of one per unit of time when it is idle (and thus the reward for a cycle equals the idle time of that cycle i.e. $I$). Then, the total reward earned up to time $t$ is equal to the total idle time in $[0,t]$ (or $\mathcal{I}(t)$), and by the result for renewal reward process (see \cite{Ross:96}, Theorem 3.6.1), with probability one,
$\lim_{t\to\infty} \mathcal{I}(t)/t=E[I]/(E[B]+E[I])$.  
\qed
%Whenever the system gets idle we say a renewal happens since after that everything starts probabilistically again. Thus, the process is an alternating renewal process. Let $Z=B+I$ be the time between renewals where $B$ and $I$ are the duration of busy and idle periods, respectively. Suppose we earn reward at rate of one per unit time when the system is idle (and thus the reward for cycle, Z, equals the idle time of that cycle i.e. $I$). Then the total reward earned by time $t$ is just the total idle time in $[0,t]$ (or $\int_0^t\delta(N(s)=0)\de s$), and thus by Theorem \ref{thm:long-run-reward} we get,
%\be
%\lim_{t\to\infty} \frac{\int_0^t\delta(N(s)=0)\de s}{t}=\frac{E[I]}{E[B]+E[I]}
%\ee
%Lemma \ref{lemma:busy-period-mean} gives $E[B]$ and we know the inter-arrival times are exponential with mean $1/\lambda$, so  $E[I]=1/\lambda$. This establishes the proposition. 
\end{proof}







%\begin{proposition}\label{prop:max-throughput}
%The maximum throughput of the system is $\lambda^*=L/(L-\bar\varphi)$.
%\end{proposition}
%\begin{proof}
%This result immediately follows by Lemmas \ref{lemma:unstable} and \ref{lemma:stable}. 
%\end{proof}
%
%\begin{remark}
%For a special case when all of the vehicles arrive at origin ($x=0$) i.e. $\varphi=\delta_{\{x=0\}}$, the maximum throughput is $\lambda^*=1$ 
%\end{remark}

\subsection{Busy Period Distribution}
\label{sec:busy-period}
%\ksmargin{is the value of $n_0$ relevant for the analysis ?}
%\mmmargin{is this a good opening sentence for this section? }
In this section, we compute the cumulative distribution function for the number of new arrivals during a busy period for a HTQ with constant service rate, say $p>0$. This could, e.g., correspond to \eqref{eq:inter-vehicle-distance-dynamics} for $m=1$. However, our analysis in this section, is not restricted to this specific model, but applies to any HTQ with constant service rate $p$. 
This cumulative distribution for the number of new arrivals during a busy period, while of independent interest, will be used to derive lower bounds on the throughput in the super-linear case in Section~\ref{subsec:superlinear}. Our analysis is inspired by that of M/G/1 queue, e.g., see \cite{Ross:96}, where our consideration for non-zero initial condition appears to be novel. 

Let us consider an arbitrary busy period spanning time interval $(0,t)$, without loss of generality. For non-zero initial condition, one has to distinguish between the first and subsequent busy periods. Let the workload at the beginning of the arbitrary busy period, denoted as $d_0$, be sampled from $\theta$. The relationship between $\theta$ and $\psi$ is as follows. 
If the system starts with a non-zero initial initial condition with initial workload $w_0>0$, then the value of the $d_0$ for the first busy period will be deterministic and equals $w_0$, and hence $\theta=\delta_{w_0}$. However, for subsequent busy periods, or if the initial condition is zero, $d_0$ is sampled from $\theta=\psi$. %On the other hand, for a system with $w=0$, the value of $d_0$ is always sampled from $\theta=\psi$. 
The workload brought to the system by arriving vehicles, $\{d_i\}_{i=1}^\infty$, equals to the distance that  vehicles wish to travel and are sampled identically and independently from the distribution $\psi$. When the system is busy, the workload decreases at a given constant rate $p > 0$. The busy period ends when the workload becomes zero. 
\begin{remark}
We emphasize that $d_0$ denotes the workload at the beginning of a busy period (see Figure \ref{fig:normalized-distance} for further illustration), and hence is not equal to zero when the queue starts from a zero initial condition. 
\end{remark}

 

In order to align our calculations with the standard M/G/1 framework, where service rate is assumed to be unity, we consider normalized workloads, $\tilde{d}_i:=d_i/p$ for all $i \in \{0,1,\cdots\}$ (see Figure \ref{fig:normalized-distance} for an illustration). Correspondingly, let the distributions for the normalized distances be denoted as $\tilde{\theta}$ and $\tilde{\psi}$. Let the arrival time of the $k$-th new vehicle during $(0,t)$ be denoted as $T_k$, and let $N_{bn}$ denote the number of arrivals in $(0,t)$, i.e., the total number of arrivals over the entire duration of the busy period, including the vehicle which initiates the busy period, is $N_{bn} + 1$. 

 A busy period ends at time $t$, and $N_{bn}=n-1$ if and only if, 
\begin{enumerate}[(i)]
\item $T_k\leq \tilde d_0+\cdots+ \tilde d_{k-1}, \qquad k=1,\cdots,n-1$ 
\item $\tilde d_0+\cdots+ \tilde d_{n-1}=t$
\item There are exactly $n-1$ arrivals in $(0,t)$
\end{enumerate} 
%The analysis of busy period period distribution for HTQs is the reminiscent of busy period calculations for $M/G/1$ queues. 
%%In M/G/1 queues, a server serves jobs in a First-Come First-Served fashion; whereas, in HTQs, vehicles are served simultaneously. 
%The difference lies under the fact that in a system with single server the workload decreases at the rate of $1$ sec/sec; however, for HTQs which are a generalization of processor sharing queues, workload decreases at the rate of $s(y)$ that is, in this section, assumed to be constant and equal to $p>0$. We further generalize our results by considering non-zero as well as zero initial workload, $w_0$. 
%
%When a system starts with a non-zero initial workload, $w_0>0$, the distribution of the first busy period is different from other busy periods and is a function of the $w_0$; however, for a system with $w_0=0$, the distribution of all of the busy periods is the same. When $w_0>0$, we say the first busy period is type 1 and the rest of busy periods are type 2. However, when $w_0=0$, all of the busy periods are type 2. A type 2 busy period starts by an arrival of a vehicle when the system is idle, and ends when a vehicle leaves the system empty. In a type 1 busy period, however, the initial workload is non-zero and busy period get started from a non-idle state \mmcomment{(see Figure \ref{} for an illustration)}. 
%
%Let $d_2,d_3,\cdots$ denote the sequence of distances that each vehicle, upon arrival, wishes to travel. In other words, this sequence can be interpreted as the sequence of the amount of workload each vehicle brings to the system. These distances are independent and identically distributed according to $\psi$. Also, let $d_1$ be the initial workload that is (present) brought to the system at the beginning of a (type 1) type 2 busy period that its distribution is $\theta$. Note that in a type 2 busy period, $d_1$ is a random variable and has the same distribution as $d_2,d_3,\cdots$ i.e. $\theta =\psi$; however, in a type 1 busy period, $d_1=w_0>0$ is a deterministic variable i.e. $\theta=\delta_{\{d_1=w_0\}}$  \mmcomment{(see Figure \ref{} for an illustration)}.  In other words,
%\be\label{eq:d1-distribution}
%\theta(x) = \begin{cases}\delta_{\{x=w_0\}} & \text{type 1 busy period} \\ \psi(x) & \text{type 2 busy period} \end{cases} \quad \forall x\geq 0
%\ee

%In any busy period, each arrival, say $j$-th arrival, increases the amount of time that server has to work in that busy period by $d_j/p$ (see Figure \ref{fig:normalized-distance} for an illustration). Therefore, we define $\tilde d_i:=d_i/p$ for all $i=1,2,\cdots$ and name them as \emph{normalized distances}. The distribution of normalized distances for $ i=\{2,3,\cdots\}$ can be obtained as, 
% \be\label{eq:two-pdf-relation}
% \tilde \Psi (x) = \Pr(\tilde d_i\leq x) = \Pr(d_i \leq px) = \Psi(px)  
% \ee
% and for $i=1$ as
% \be\label{eq:d1-cdf}
% \Theta(x) = \Pr(\tilde d_1\leq x)= \Theta (px)
% \ee
%and correspondingly the probability distribution functions are denoted by $\tilde \psi$ and $\tilde \theta$. 

%By \eqref{eq:two-pdf-relation}, one can realize that if $\varphi$ is continuous, $\tilde\varphi(x)=p \varphi(px)$.

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=8cm]{normalized-distance} 
\caption{Evolution of workload during first two busy periods for an HTQ with constant service rate $p$, and starting from a non-zero initial condition. In the first busy period, $d_0$ is equal to the workload $w_0$ associated with the non-zero initial condition. In the second busy period, $d_0$ is equal to the workload brought by the first vehicle that initiates that busy period.}
\label{fig:normalized-distance}
\end{center}
\end{figure}


%Let designate the time at which a busy period starts by $0$, and $S_k$ denote the time until $k$ additional vehicles have arrived and $N_{bn}$ denote the number of arrivals in $(0,t)$. A busy period will last a time $t$, and $N_{bn}=n-1$ if, and only if, 
%\begin{enumerate}[(i)]
%\item $S_k\leq \tilde d_1+\cdots+ \tilde d_k, k=1,\cdots,n-1$ 
%\item $\tilde d_1+\cdots+ \tilde d_n=t$
%\item There are $n-1$ arrivals in $(0,t)$
%\end{enumerate} 
%For a type 2 busy period, we define $N_{bp}:=N_{bn}+1$ that is the number of customers served in a type 2 busy period. Note that the above conditions imply that $N_{bp}=n$.
%
%In a type 1 busy period, the above three conditions imply that the busy period will last a time $t$ and $N_{bn}=n-1$ new vehicles are joined to the system before the end of busy period. 

By treating densities as if they are probabilities, we get:
\begin{align}
\label{eq:prop-busy-des}
\Pr & (B =t \text{ and }N_{bn} = n -1)\nonumber \\
=&  \Pr(\tilde d_0+\cdots+ \tilde d_{n-1}=t, n-1 \text{ arrivals in $(0,t)$}, T_k\leq \tilde d_0+\cdots+ \tilde d_{k-1}, k=1,\cdots,n-1) \nonumber \\
=& \int_0^t\Pr(T_k\leq \tilde d_0+\cdots+ \tilde d_{k-1}, k=1,\cdots,n-1| n-1 \text{ arrivals in $(0,t)$}, \tilde d_0+\cdots+ \tilde d_{n-1}=t, \tilde d_0 =z) \nonumber \\
%\label{eq:busy-period-prob-integ}
& \times \Pr(n-1 \text{ arrivals in $(0,t)$}, \tilde d_1+\cdots+ \tilde d_{n-1}=t-z)\, \tilde \theta(z)  \, \de z 
%\label{eq:busy-period-prob-integ}
\end{align}
where we recall that $B$ is the random variable corresponding to the busy period duration. By the independence of normalized distances and the arrival process, the second probability term in the integrand in \eqref{eq:prop-busy-des} can be expressed as
\begin{align}
\label{eq:prop-busy-part2}
\Pr(n-1 \text{ arrivals in $(0,t)$}, \tilde d_1+\cdots+ \tilde d_{n-1}=t-z)=e^{-\lambda t}\frac{(\lambda t)^{n-1}}{(n-1)!} \tilde \psi_{n-1}(t- z) 
\end{align}
where $\tilde\psi_n$ is the $n$-fold convolution of $\tilde\psi$ with itself. 

In the first probability term in \eqref{eq:prop-busy-des}, it is given that the system receives $n-1$ arrivals in $(0,t)$ and since the arrival process is a Poisson process, the ordered arrival times, $\{T_1,T_2,\cdots,T_{n-1}\}$, are distributed as the ordered values of a set of $n-1$ independent uniform $(0,t)$ random variables $\{a_1,a_2,\cdots,a_{n-1}\}$ (see Theorem 2.3.1 in \cite{Ross:96}). Thus,
%\ksmargin{\eqref{eq:busy-period-given-n-prob} probably needs a bit more explanation}
\begin{align}\label{eq:busy-period-given-n-prob}
\Pr & (T_k\leq \tilde d_0+\cdots+ \tilde d_{k-1}, k=1,\cdots,n-1| n-1 \text{ arrivals in $(0,t)$}, \tilde d_0+\cdots+ \tilde d_{n-1}=t,\tilde d_0 =z) \nonumber \\
&  =  \Pr(a_k\leq \tilde d_0+\cdots+\tilde d_{k-1}, k=1,\cdots,n-1|\tilde d_0+\cdots+\tilde d_{n-1} =t,\tilde d_0 =z)
\end{align}
% In order to compute the probability in \eqref{eq:busy-period-given-n-prob}, we need the following lemma  The proof can be found in \cite{Ross:96}.

%\begin{lemma}
%Let $\tilde d_1, \tilde d_2, \cdots \tilde d_n$ be i.i.d. non-negative random variables, then 
%$$E[\tilde d_1+ \cdots +\tilde d_k|\tilde d_1+ \cdots +\tilde d_n=y]=\frac{k}{n}y,\qquad k=1,\cdots,n$$
%\end{lemma}

%\begin{lemma}
%Let $\tau_1, \cdots, \tau_n$ denote the ordered values from a set of $n$ independent uniform $(0,t)$ random variables. Let $\tilde d_1, \tilde d_2, \cdots \tilde d_n$ be i.i.d. non-negative random variables that are also independent of $\{\tau_1, \cdots, \tau_n\}$, then 
%\begin{align}
%\Pr(\tilde d_1+ \cdots +\tilde d_k<\tau_k,k=1,\cdots,n |\tilde d_1+ \cdots +\tilde d_n=y)
% = \begin{cases}1-y/t&0<y<t \\ 0 & \text{otherwise}\end{cases}
%\end{align}
%\end{lemma}
%


%\begin{lemma}\label{lemma:busy-period-type2-prob}
%Let $\tau_1, \cdots, \tau_{n-1}$ denote the ordered values from a set of $n-1$ independent uniform $(0,t)$ random variables. Let $\tilde d_1, \tilde d_2, \cdots \tilde d_n$ be i.i.d. non-negative random variables that are also independent of $\{\tau_1, \cdots, \tau_{n-1}\}$, then 
%\begin{align}
%\Pr(\tilde d_1+ \cdots +\tilde d_k\leq\tau_k,k=1,\cdots,n-1 |\tilde d_1+ \cdots +\tilde d_n=t)
% = 1/n
%\end{align}
%\end{lemma}




By noting that $t-U$ will also be a uniform $(0,t)$ random variable whenever $U$ is, it follows that $a_1,\cdots,a_{n-1}$ has the same joint distribution as $t-a_{n-1},\cdots,t-a_1$. Thus, replacing $a_k$ with $a_{n-k}$ for $k\in\{1,\cdots,n-1\}$ in \eqref{eq:busy-period-given-n-prob}, we get
\begin{align}\label{eq:prob-manipulation}
 \Pr&(a_k  \leq \tilde d_0+\cdots+\tilde d_{k-1}, k=1,\cdots,n-1|\tilde d_0+\cdots+\tilde d_{n-1} =t,\tilde d_0 =z) \nonumber \\
 &  =\Pr(t-a_{n-k}  \leq \tilde d_0+\cdots+\tilde d_{k-1}, k=1,\cdots,n-1|\tilde d_0+\cdots+\tilde d_{n-1} =t,\tilde d_{0} =z)  \nonumber \\
 & = \Pr(t-a_{n-k}  \leq  t-(\tilde d_{k}+\cdots+\tilde d_{n-1}), k=1,\cdots,n-1|\tilde d_0+\cdots+\tilde d_{n-1} =t,\tilde d_0 =z)  \nonumber \\
  & = \Pr(a_{n-k}  \geq  \tilde d_{k}+\cdots+\tilde d_{n-1}, k=1,\cdots,n-1|\tilde d_0+\cdots+\tilde d_{n-1} =t,\tilde d_0 =z)  \nonumber \\
  & = \Pr(a_{n-k}  \geq  \tilde d_{k}+\cdots+\tilde d_{n-1}, k=1,\cdots,n-1|\tilde d_0+\cdots+\tilde d_{n-1} =t,\tilde d_0 =z) = \begin{cases}  z/t &  z<t \\
                          0      & \text{otherwise}
    \end{cases}
\end{align}
where the last equality follows from Lemma \ref{lemma:busy-period-type1-prob}.
%For a type 2 busy period:
%\begin{align}\label{eq:busy-t2-part3}
% \Pr(\tau_k & \leq \tilde d_1+\cdots+\tilde d_k, k=1,\cdots,n-1|\tilde d_1+\cdots+\tilde d_n =t) \nonumber \\
%  & = \Pr(\tau_{n-k}  \geq  \tilde d_{k+1}+\cdots+\tilde d_n, k=1,\cdots,n-1|\tilde d_1+\cdots+\tilde d_n =t) \nonumber \\
%  & = \Pr(\tau_{n-k}  \geq  \tilde d_{n-k}+\cdots+\tilde d_1, k=1,\cdots,n-1|\tilde d_1+\cdots+\tilde d_n =t)=1/n
%\end{align}
%where the first equality follows by \eqref{eq:prob-manipulation}, and the second equality follows since $\tilde d_1,\cdots,\tilde d_n$ has the same joint distribution as $\tilde d_n, \cdots, \tilde d_1$. Also, the last equality follows by Lemma \ref{lemma:busy-period-type2-prob}.
If we let $H_p(t,n,\theta):=\Pr\{B\leq t, N_{bn}=n-1\}$ when the service rate equals $p$, and $d_0$ has distribution $\theta$; then, by plugging \eqref{eq:prop-busy-part2} and \eqref{eq:prob-manipulation} in \eqref{eq:prop-busy-des}, we get
\begin{equation*}
\frac{d}{dt}H_p(t,n,\theta) = e^{-\lambda t}\frac{(\lambda t)^{n-1}}{t(n-1)!}\int_0^t z \tilde\psi_{n-1}(t-z)\tilde \theta(z)\de z
\end{equation*}


By recalling the two special cases of interest to us: $\theta=\delta_{w_0}$ for a given non-zero initial workload $w_0$, and $\theta=\psi$ for zero initial condition, and using Lemma \ref{lemma:t-n},  we get that 
%\ksmargin{should mention somewhere that $\tilde{\psi}(x) =0$ if $x<0$ \mmcomment{I added it.}}
\begin{equation}
\label{eq:G-def}
G_p(t,n,\theta):=\frac{d}{dt}H_p(t,n,\theta)=\begin{cases} e^{-\lambda t}\frac{(\lambda t)^{n-1}w_0}{t(n-1)!p}\tilde \psi_{n-1}(t-w_0/p) & \theta = \delta_{w_0} \\ e^{-\lambda t}\frac{(\lambda t)^{n-1}}{n!}\tilde \psi_n(t) & \theta = \psi \end{cases}
%\qquad \frac{d}{dt}D_p^{(2)}(t,n)=e^{-\lambda t}\frac{(\lambda t)^{n-1}}{n!}\tilde \psi_n(t)
\end{equation}
%\ksmargin{there seem to be a few typos in the expression for cdf}

For $r \in \NN$, let $G_{r,p}(t,n,\theta)$ be the $r$-fold convolution of $G_p(t,n,\theta)$, defined in \eqref{eq:G-def}, with respect to $t$. In words, $G_{r,p}(t,n,\theta)$ is the probability that the number of new arrivals in each of (any) $r$ busy periods is equal to $n-1$, and that the sum of durations of all the busy periods is equal to $t$. Similarly, for non-zero initial condition, let $G_{p_1}(\theta_1) * G_{r-1,p_2}(\theta_2) (t,n)$ be the probability that the number of new arrivals in each of (any) $r$ busy periods is equal to $n-1$, and that the sum of durations of all the busy periods is equal to $t$, when the constant service rate for the first busy period is $p_1$ and is $p_2$ for the rest of the $r-1$ busy periods.

%Integrating \eqref{eq:G-def} with respect to $t$, we get 
%\begin{equation}
%\label{eq:busy-period-joint-distribution}
%H_p(t,n,\theta)=\begin{cases} \int_{w_0/p}^te^{-\lambda s}\frac{(\lambda s)^{n-1}}{t(n-1)!}\tilde \psi_{n-1}(t-w_0/p) \, \de s & \theta = \delta_{w_0} \\ \int_0^te^{-\lambda s}\frac{(\lambda s)^{n-1}}{n!}\tilde \psi_n(s) \, \de s & \theta = \psi \end{cases}
%\end{equation}
%
%The joint distribution for the busy period in \eqref{eq:busy-period-joint-distribution} can be marginalized to get appropriate quantities of interest. In particular, if we let $C_p(M,\lambda,\theta):=\Pr(N_{bn}\leq M-1\}$ when the  service rate equals $p$, and $d_0$ has distribution $\theta$; then the cumulative distribution function for the number of new arrivals during the busy period is given by:
%\begin{align}
%\label{eq:busy-period-numofarrival-distribution}
%C_p(M,\lambda,\theta)=\lim_{t\to +\infty} \sum_{n=1}^M H_p(t,n,\theta)
% \end{align}
 
 
%If we let 
%\be
%D_p^{(i)}(t,n):=\Pr\{\text{a type $i$ busy period}\leq t, N_{bn}=n-1, \text{ service rate}= p \}, \;\; i=1,2
%\ee
%then by plugging \eqref{eq:prop-busy-part2} and \eqref{eq:prob-manipulation} in \eqref{eq:prop-busy-des}, we get
%\be
%\frac{d}{dt}D^{(i)}_p(t,n) = e^{-\lambda t}\frac{(\lambda t)^{n-1}}{t(n-1)!}\int_0^tz\tilde\psi_{n-1}(t-z)\tilde \theta(z)\de z
%\ee
%and then by \eqref{eq:d1-distribution} and \eqref{eq:d1-cdf} and Lemma \ref{lemma:busy-period-type1-prob} in Appendix, we see
%\be
%\frac{d}{dt}D_p^{(1)}(t,n)=\begin{cases} e^{-\lambda t}\frac{(\lambda t)^{n-1}w_0}{t(n-1)!p}\tilde \psi_{n-1}(t-w_0/p) & w_0/p<t \\ 0 & \text{otherwise} \end{cases}, \qquad \frac{d}{dt}D_p^{(2)}(t,n)=e^{-\lambda t}\frac{(\lambda t)^{n-1}}{n!}\tilde \psi_n(t)\ee
%or 
%\begin{align}\label{eq:busy-period-and-nbp-joint}
%& D_p^{(1)}(t,n,w_0)= \int_{w_0/p}^te^{-\lambda y}\frac{(\lambda y)^{n-1}}{t(n-1)!}\tilde \psi_{n-1}(y-w_0/p)\de y, \quad
%D_p^{(2)}(t,n)= \int_0^te^{-\lambda y}\frac{(\lambda y)^{n-1}}{n!}\tilde \psi_n(y)\de y
%\end{align}
% \mmmargin{we never use these two notations. I just defined them because the title of this section is ``busy period distribution". Do we really need this ? }

%\sout{
% Finally, the distribution of the length of a busy period for a system with constant service rate of $p$ is given by:}
%\begin{align}\label{eq:busy-period-dist}
%B_p^{(1)}(t,w_0)&:=\Pr(\text{a type 1 busy period}\leq t, \text{ service rate}=p,w_0>0)=\sum_{n=1}^{\infty}D^{(1)}_p(t,n) \nonumber \\%=\sum_{n=1}^\infty\int_0^te^{-\lambda t}\frac{(\lambda t)^{n-1}}{n!}\de\tilde \Phi_n(t)
%B_p^{(2)}(t)&:=\Pr(\text{a type 2 busy period}\leq t, \text{ service rate}=p)=\sum_{n=1}^{\infty}D^{(2)}_p(t,n) 
%\end{align}
% Moreover, by marginalizing over $t$, one can obtain the distribution of $N_{bn}$ for type 1 ($i=1$) and type 2 ($i=2$) busy periods as:
% \begin{align}
%C_p^{(i)}(M,\lambda):=\Pr(N_{bn}\leq M-1, \text{ service rate}= p,\lambda)=\sum_{n=1}^M D_p^{(i)}(t\to\infty,n), \quad i=1,2
% \end{align}
 
%and for a type 2 busy period, the distribution of $N_{bp}$ is given as:
% \be\label{eq:nbp-dist}
% C_p^{(2)}(M,\lambda):=\Pr(N_{bp}\leq M, \text{ service rate}= p, \lambda)=\sum_{n=1}^M D_p^{(2)}(t\to\infty,n)
% \ee



==> 02- submission/busy-period.tex <==
\subsection{Analysis for $m>1$ case}
In this section, we assume that system starts from an empty initial condition and then we derive a probabilistic lower bound on the throughput of the system. For our analysis we focus on busy period and the number of vehicles served in a busy period. 

We first assume an upper bound on the queue length, i.e. $N(t)\leq M \; \forall t\geq0$, which by Lemma \ref{lem:service-rate-bounds} gives a lower bound on the service rate of the system i.e. $s(y(t))\geq L^mM^{1-m}\; \forall t\geq 0$. Then, we use this lower bound on the service rate to compare the system with a system with the same temporal-spatial arrival process but a slower decrease rate of workload . We use this comparison as a tool to find a lower bound on the probability of achieving the assumed upper bound on the queue length. This result leads to a probabilistic lower bound on the throughput of the system which is stated in Theorem \ref{}. Our analysis heavily depends on the probability distribution of busy periods which is described in the next section.


 
 \subsubsection{From busy period to throughput}
%\begin{lemma}\label{lemma:cdf-poisson}
%\mmmargin{find a proper reference}
%The cumulative distribution function of a Poisson random variable with mean $\mu > 0$ is decreasing in $\mu$.
%\end{lemma}
%\begin{proof}
%Let $X$ be a Poisson random variable with mean $\mu > 0$, then the cdf of $X$ for a fixed $n\in\mathbb{N}$ is given as \cite{?},\
%\be
%f(\mu) = \Pr(X\leq n) = \frac{\int_{\mu}^\infty t^{n}e^{-t}\de t}{n!}
%\ee 
%Since the integrand in the numerator is positive, the above function is decreasing in $\mu$.
%\end{proof}


 
  \begin{proposition}\label{prop:nbp-lower-bound}
 For any $m>1$, $w_0=0$, $L>0$, $\lambda > 0$ $\varphi \in \Psi$ and $M\in\{2,3,\cdots\}$, given $N(t)<M$ $\forall t>0$, then 
  $$\Pr(N_{bp}\leq M)\geq C^{(2)}_{L^m M^{1-m}}(M,\lambda)\qquad \forall n\in\mathbb{N}$$
 \end{proposition}
 \begin{proof}
 \mmmargin{service is not greater than this lower bound for all t because of idle time. revise it}
 For $m>1$, by Lemma \ref{lem:service-rate-bounds}, and the upper bound given on the queue length,
 \be
 s(t)\geq L^mM^{1-m} = p \quad \forall t>0
 \ee 
 
 We consider another system with the same realization of temporal-spatial arrival process but fixed service rate of $p$ and name it as the \emph{slower} system. Let $B_1$ and $B_2$ be random variables that denote the length of a busy period in actual and slower system, respectively. Since the realization of arrival processes are the same for both systems, and the decrease rate of workload in slower system is smaller it is clear that,
 \be\label{eq:workload-actual-slower}
 w_1(t)\leq w_2(t) \quad \forall t>0
 \ee
where $w_1(t)$ and $w_2(t)$ denote the the workload processes in actual and slower system, respectively. 

Now, let $t_s$ be the time at which a (random) busy period in the slower system ends and $t_1$ be the time at which the next busy period in that system ends (see Figure \ref{fig:b1-b2} for an illustration). Obviously, $w_1(t_s)=w_1(t_f)=0$. Also, by \eqref{eq:workload-actual-slower}, $w_2(t_s)=w_2(t_f)=0$. Let $t_1\in(t_s,t_f)$ be the time of the first arrival after $t=t_s$. Note that this time is the same in both systems. Therefore, in the slower system, the busy period that lies in $[t_s,t_f]$ has the length of $t_f-t_1$.  Let $t_2\in[t_1,t_f]$ be the time at which the actual system gets idle for the first time after $t=t_1$. We want to show that $t_2\leq t_f$. By contradiction, assume $t_2> t_f$. Thus, $w_1(t_f)>0$, but $w_2(t_f)=0$. This contradicts \eqref{eq:workload-actual-slower} and proves that $t_2\leq t_f$. This implies that the longest busy period in actual system contained in $[t_s,t_f]$ is no longer than the busy period in actual system. This argument holds for any busy period in slower system. Thus,  with probability one, 
 \be\label{eq:relation-b1-b2}
 B_1\leq B_2
 \ee  
 
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=9cm]{b1-b2} 
\caption{Workload process for two systems with the same realization temporal-spatial arrival process, a system with slower service rate (solid line) and a system with a faster service rate (dashed line).}
\label{fig:b1-b2}
\end{center}
\end{figure}

Now, let $N_{bp}$ and $\tilde N_{bp}$ be the number of customers served in a busy period in the actual system and slower system, respectively. Note that $N_{bp}$ and $\tilde{N}_{bp}$ are Poisson random variables with mean $\lambda B_1$ and $\lambda B_2$, respectively and by \eqref{eq:relation-b1-b2}, $\lambda B_1\leq \lambda B_2$. Poisson random variable is stochastically increasing in its mean (see e.g. \cite{Ross:96}), therefore
\be
\tilde{N}_{bp}\geq_{\text{st}}{N}_{bp}
\ee 
which establishes this proposition. %There exists a random variable $B_1^*$, independent of $B_2$, with the same distribution of $B_1$ such that, with probability one, $B_1^*\leq B_2$. Now, consider two Possoin random variables with means $\lambda B_1^*$ and $\lambda B_2$. Thus, by Lemma \ref{lemma:cdf-poisson}, $f(\lambda B_1^*)\geq f(\lambda B_2)$. Therefore, for any $M\in\mathbb{N}$,
 %\be
 %f(\lambda B_1^*)\leq f(\lambda B_2)
 %\ee 
 \end{proof}
 
\mmmargin{have we defined this notation ($n_0$) earlier?}
 \begin{proposition}\label{prop:nbn-lower-bound}
 For any $m>1$, $w_0>0$, \mmcomment{$n_0\in\mathbb{N}$}, $L>0$, $\lambda > 0$, $\varphi \in \Psi$ and $M\in\{2,3,\cdots\}$, given $N(t)<M$ $\forall t>0$, then 
  $$\Pr(N_{bn}\leq M)\geq C^{(1)}_{L^m (M+n_0)^{1-m}}(M,\lambda,w_0)\qquad \forall n\in\mathbb{N}$$
 \end{proposition}
 \begin{proof}
 The proof is very similar to the proof of Proposition \ref{prop:nbp-lower-bound}; however, in this case the upper bound on the queue length is $M+n_0$, and the lower bound on the service rate is $L^m(M+n_0)^{1-m}$. 
 \end{proof}



 
 %\begin{lemma} \label{lemma:st-order-queulength-nbp}
% The total number of customers served in a busy period of length $B$ is stochastically larger than the queue length in that busy period i.e. 
% $$N_{bp}\geq_{\text{st}}N(t)\;\; \forall t\in[0,B]$$
 %\end{lemma}
 %\begin{proof}
% For any $t\in[0,B]$ and $M\geq 1$, $N_{bp}\leq M$ implies $N(t)\leq M$. However, the converse is not true. This implies that event $N_{bp}\leq M$ is a subset of event $N(t)\leq M$, and therefore, ${\Pr(N(t)\leq M)\geq \Pr(N_{bp}\leq M)}$ which implies ${\Pr(N_{bp}> M)\geq \Pr(N(t)> M)}$. This establishes this lemma. 
% \end{proof}  
 
  \begin{lemma} \label{lemma:st-order-queulength-nbp}
 For any $m>1$, $L>0$, $\lambda>0$, $\varphi \in \Psi$, $w_0=0$,%The total number of customers served in a busy period is stochastically larger than the queue length in that busy period i.e. 
 $$N_{bp}\geq_{\text{st}}N(t)\quad \forall t\geq 0$$
 \end{lemma}
 \begin{proof}
 Conditioned on the length of busy period, $B$, 
 \be
 N_{bp}\leq M | B = b \implies N(t)\leq M | B = b \quad \forall t\in[0,b]
 \ee
 where here $t=0$ denotes the time at which busy period starts. Then,
 \be
 \Pr(N_{bp}\leq M | B = b) \leq \Pr(N(t)\leq M | B = b) \quad \forall t\in[0,b]
 \ee
 and by taking the expectation of the above with respect to length o busy period, we get 
 \be
  \Pr(N_{bp}\leq M) \leq \Pr(N(t)\leq M) \quad \forall t>0
 \ee
 which establishes this lemma. 
 \end{proof}  

%Now, we one can use Proposition \ref{} and Lemma \ref{} in order to probabilistically characterize the throughput of the system. Let fix a $\delta\in[0,1]$ in Definition \ref{}. Then, by Proposition \ref{} and Lemma \ref{}, we have the following relationship,
 %Now, we can establish the following relationship,
 Now, we are ready to state the main result in the following theorem which gives a probabilistic lower bound on the throughput of the system for $m>1$.
 \begin{theorem}
 Given $\delta\in(0,1)$, $L>0$, $m>1$, $\varphi\in\Psi$, $w_0=0$, then
 $$\lambda_{\max}(m, L, \varphi,\delta)\geq \max_{M\geq 2}\;\max\{\lambda>0 \;| C^{(2)}_{L^m M^{1-m}}(M,\lambda)\geq1-\delta\}$$
 \end{theorem}
 \begin{proof}
For a given upper bound on the queue length, $M\in\{2,3\cdots\}$, 
 \be\label{eq:prob-bound-queue}
 \Pr(N\leq M) \geq \Pr(N_{bp}\leq M) \geq  C^{(2)}_{L^m M^{1-m}}(M,\lambda)
 \ee
 where the first inequality follows by Lemma \ref{lemma:st-order-queulength-nbp} and the second inequality follows by Proposition \ref{prop:nbp-lower-bound}. Therefore, based on Definition \ref{def:throughput},  $\tilde \lambda = \max\{\lambda>0 \;| C_{L^m M^{1-m}}(M,\lambda)=1-\delta\}$ gives a lower bound on $\lambda_{\max}$. In Definition \ref{def:throughput}, however, only boundedness of queue length matters. Thus, one can maximize $\tilde \lambda$ over $M\geq 2$ to get tighter lower bound. 
 
 
 %The above inequality provides a tool to probabilistically characterize the throughput of the system. Let fix a $\delta\in[0,1]$ in Definition \ref{def:throughput} and assume an upper bound, $M$, for the queue length of the system. One can use \eqref{eq:prob-bound-queue} in order to find the maximum $\lambda$ such that 
 %\be\label{eq:relation-queue-nbp}
 %\Pr(N\leq M) \geq B_{L^mM^{1-m}}(N_{bp}\leq M)\geq 1-\delta
 %\ee
 %It should be noted that this $\lambda$ will be a function of $M$ as well as other arguments described in Definition \ref{def:throughput}. The value of $\lambda$ computed in this way ensures that, starting from empty initial condition, the queue length will not exceed $M$ with probability $1-\delta$. 
 \end{proof}
 
 
  \begin{theorem}
 Given $\delta_1,\delta_2\in(0,1)$, $L>0$, $m>1$, $\varphi\in\Psi$, $w_0>0$, $n_0\in\mathbb{N}$ then
 $$\lambda_{\max}(m, L, \varphi,\delta)\geq \max_{M_1,M_2\geq 2}\;\max\{\lambda>0 \;| C^{(1)}_{L^m (M+n_0)^{1-m}}(M,\lambda,w_0)C^{(2)}_{L^m (M_2)^{1-m}}(M,\lambda)\geq(1-\delta_1)(1-\delta_2)\geq (1-\delta)\}$$
 \end{theorem}
 \begin{proof}
\mmcomment{work in progress ...} 
 
 \end{proof}
 
 In order to further clarify the analysis in this section, the following example shows the application of these results in order to probabilistically characterize the throughput of the system for a specific spatial distribution. 
 
 \begin{example}[Deterministic traveled distances] Assume that vehicles, upon arrival, wish to travel a deterministic distance of length $L>0$ i.e. $\varphi(x)=\delta_{\{x=L\}}$ and their motion is determined by a car following model with $m>1$. Also, further assume that the queue length does not exceed $M\in\{2,3,\cdots\}$. In this case, the lower bound on the service rate is $p=L^mM^{1-m}$. Application of \eqref{eq:busy-period-and-nbp-joint} gives,
  \be\label{eq:busy-period-joint-deterministic}
  D_p(t,N_{bp}=n) = \int_0^te^{-\lambda y}\frac{(\lambda y)^{n-1}}{n!}\delta_{\{y=nL/p\}}\de y=\begin{cases}0 & t\leq nL/p\\ e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!}& t> nL/p\end{cases}
  \ee
% and by \eqref{eq:nbp-dist},
%\be
%B_p(N_{bp}=n)= e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!}
%\ee
and by Lemma \ref{lemma:st-order-queulength-nbp} and Proposition \ref{prop:nbp-lower-bound},
\be
 \Pr(N\leq M)\geq \Pr(N_{bp}\leq M)\geq C_{L^m M^{1-m}}(M,\lambda) = \sum_{i=1}^M e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!} \geq1-\delta.
\ee
The above inequality can be used in order to find the maximum throughput for which queue length remains bounded by $M$ with probability of at least $1-\delta$.
 \end{example}



==> 02- submission/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we formulated and analyzed a novel horizontal traffic queue. A key characteristic of this queue is the state dependence of its service rate. We establish useful properties of the service rate dynamics. We also extend calculations for M/G/1 busy period distributions to our setting, even for non-empty initial condition. These results allow us to provide tight results for throughput in the linear case, and probabilistic bounds on queue length over finite time horizon in the super-linear case. We also study throughput under a batch release control policy, where the additional waiting induced by the control policy is interpreted as a perturbation to the arrival process. We provide lower bound on the throughput for a maximum permissible perturbation. In particular, if the allowable perturbation is sufficiently large, then this lower bound grows unbounded as $m \to 0^+$. Simulation results suggest a sharp phase transition in the throughput as the car-following behavior transitions from super-linear to sub-linear regime. 

In future, we plan to sharpen our analysis to theoretically demonstrate the phase transition behavior. 
This could include, for example, considering other release control policies with better perturbation properties. The increasing nature of the throughput in the super-linear regime for large values of $L$, as illustrated in Figure~\ref{fig:throughput-simulations}, is possibly because the car-following model considered in this paper does not impose any explicit upper bounds on the speed of the vehicles. We plan to extend our analysis to such practical constraints, as well as to higher order, e.g., second order, car-following models, and models emerging from consideration of inter-vehicle distance beyond the vehicle immediately in front. The connections with processor sharing queue, as highlighted in this paper, suggest the possibility of utilizing the construct of measure-valued state descriptors~\cite{Grishechkin:94,Gromoll.Puha.ea:02} to derive fluid and diffusion limits of the proposed horizontal traffic queues. In particular, one could interpret the measure-valued state descriptor to play the role of traffic density in the context of traffic flow theory. Along this direction, we plan to investigate connections between the fluid limit of horizontal traffic queues, and PDE models for traffic flow. 

==> 02- submission/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
We consider a horizontal traffic queue (HTQ) on a periodic road segment, where vehicles arrive according to a spatio-temporal Poisson process, and depart the queue after traveling a distance that is sampled independently and identically from a spatial distribution. When inside the queue, the speed of a vehicle is proportional to a power $m>0$ of the distance to the vehicle in front. For a given initial condition, we define the throughput of such a queue as the largest arrival rate under which the queue length remains bounded. We provide rigorous analysis for the service rate, busy period distribution, and throughput of the proposed HTQ. 

Our motivation for studying HTQ comes from advancements in connected and autonomous vehicle technologies that allow to program individual vehicles with rules that can optimize system level performance. Within this application context, one can interpret the results of this paper as rigorously characterizing the impact of a parametric class of car-following behavior on system throughput. 

%Rapid advancements in vehicle-to-vehicle and vehicle-to-infrastructure  communications, combined with autonomous driving have the potential to dramatically improve the performance of urban transportation systems. Such high levels of automation will present great opportunities for architecting new interactions rules, e.g., in the form of car following, lane changing and route choice behaviors. 
%%The ability to use V2V and V2I technologies to extend the interaction range of vehicles will add further richness to the possible interactions rules. 
%While these new possibilities present new ways for tackling congestion and improving safety and performance, the increased complexity of the design space poses serious challenges for the system designer. In particular, mathematically rigorous results on the impact of microscopic interaction rules on macroscopic performance measures for transportation systems are severely lacking. In this paper, we address this drawback in the existing literature by providing rigorous analysis of throughput for horizontal traffic queues under a class of kinematic car following models.

In the linear case ($m=1$), i.e., when the speed of every vehicle is proportional to the distance to the vehicle directly in front, the periodicity of the road segment implies that the sum of the speeds of the vehicles is proportional to the total length of the road segment, i.e., it is constant. This feature allows us to exploit the equivalence between workload and queue length to show that, independent of the initial condition and almost surely, the throughput is the inverse of the time required by a solitary vehicle to travel average distance. 

In the non-linear case ($m \neq 1$), the cumulative service rate of HTQ queue is constant if and only if all the inter-vehicle distances are equal. For all other inter-vehicle configurations, we show that the service rate is strictly decreasing (resp., strictly increasing) in the super-linear, i.e., $m>1$ (resp., sub-linear, i.e., $m<1$) case. The service rate exhibits an another contrasting behavior in the sub- and super-linear regimes. In the super-linear case, the service rate is maximum (resp., minimum) when all the vehicles are co-located (resp., when the inter-vehicle distances are equal), and vice-versa for the sub-linear case. Using a combination of these properties, we prove that, when the length of the road segment is at most one, the throughput in the super-linear (resp., sub-linear) case is upper (resp., lower) bounded by the throughput for the linear case.

We prove the remaining bounds on the throughput for the non-linear case as follows. The standard calculations for joint distributions of duration and number of arrivals during a busy period for M/G/1 queue are extended to the HTQ setting, including for non-empty initial conditions. 
%The marginals of these distributions are then used to get probabilistic bounds on the maximum queue length during a busy period, which in turn gives lower bound on the service rate.
These joint distributions are used to derive probabilistic upper bounds on queue length over finite time horizons for HTQ for the $m>1$ case. Such bounds are optimized to get lower bounds on throughput defined over finite time horizons. Simulation results show good comparison between such lower bounds and numerical estimates.
 
We also analyze throughput in the sub-linear and super-linear cases under perturbation to the arrival process, which is attributed to the additional expected waiting time induced by a release control policy that adds appropriate delay to the arrival times to ensure a desired minimum inter-vehicle distance $\triangle>0$ at the time of a vehicle joining the HTQ. Since the minimum inter-vehicle distance is non-decreasing in between arrivals and jumps, this implies an upper bound on the queue length which is inversely proportional to $\triangle$. We derive a lower bound on throughput for a given  
combination of maximum allowable perturbation. In particular, if the allowable perturbation is sufficiently large, then this lower bound grows unbounded, as $m \to 0^+$.  

%\ksmargin{remove redundant references, \mmcomment{Done!}}

 
Queueing models have been used to model and analyze traffic systems. The focus here has been primarily on vertical queues, under which vehicles travel at maximum speed until they hit a congestion spot where all vehicles queue on top of each other.
% 
% Queueing systems are a compelling modeling framework traffic due to their capability to capture congestion, to allow entry and exit of vehicles, and to facilitate study of relevant metrics for system performance such as capacity or throughput and system time. 
% %Vertical and horizontal queues are two major categories of traffic queuing models. 
% Vertical queueing models are characterized by the fact that vehicles travel at maximum speed until they hit a congestion spot (e.g., a signalized traffic intersection) where all vehicles queue on top of each other. 
The queue length and waiting time of a minor traffic stream at an unsignalized intersection where major traffic stream has high priority is studied in \cite{Tanner:62} and \cite{Heidemann:91}. 
In \cite{Heidemann:94}, a vertical single server queue is utilized to model the queue length distribution at signalized intersections.
%In traffic queues, the service rate highly depends on the state of the system. 
In \cite{Jain.Smith:97}, a state-dependent queuing system is used to model vehicular traffic flow where the service rate depends on the number of vehicles on each road link. 
%Although the service rate in traffic queues depend on the congestion, this dependency is through microscopic congestion and not macroscopic congestion such as queue length. 
 %The accuracy of the vertical queues can be improved by considering finite capacity queues to incorporate congestion and blocking. In a vertical queue, the service policy is First-Come First-Served and the service rate usually is derived from fundamental traffic diagram and depends on the state of the system only through a macroscopic sense (e.g. traffic density) 

 On the other hand, the \emph{horizontal traffic queue} terminology has been primarily used to study macroscopic traffic flow, e.g., see \cite{Helbing:03}. While such models capture the macroscopic relationship between traffic flow and density, a rigorous description and analysis of an underlying queue model is lacking. Indeed, to the best of our knowledge, there is no prior work on the analysis of a traffic queue model that explicitly incorporates car-following behavior. 
% 
%  without rigorous formulation and of an underlying queueing model. 
% 
% spill backs and wave propagation. However, in the existing literature of horizontal traffic queue \cite{Hofleitner.ea:12}, the queue process is treated as macroscopic quantity by relating the propagation speed, traffic density and flow to the queue length and waiting time. Therefore, macroscopic information is derived from fundamental traffic diagram and it does not depend on the interaction rules between vehicles. To the best of our knowledge, for the first time in this literature, we analyzed a HTQ with linear car-following model in our recent work \cite{Motie.Savla.CDC15}. In this paper, we further study HTQs by incorporating non-linear car-following model to achieve a state dependent service which is natural in the context of traffic queues.  

The proposed HTQ has an interesting connection with processor sharing (PS) queues, and this connection does not seem to have been documented before.
A characteristic feature of PS queues is that all the outstanding jobs receive service simultaneously, while keeping the total service rate of the server constant. The simplest model is where the service rate for an individual job is equal to $1/N$, where $N$ is the number of outstanding jobs. In our proposed system, one can interpret the road segment as a server simultaneously providing service to all the vehicles, with the service rate of an individual vehicle equal to its speed. This natural analogy between HTQ and PS queues, to the best of our knowledge, was reported for the first time in our recent work~\cite{Motie.Savla.CDC15}.
The $1/N$ rule applied to our setting implies that all the vehicles travel with the same speed. Clearly, such a rule, or even the general discriminatory PS disciplines, e.g., see \cite{Kleinrock:67}, are not applicable to the car following models considered in this paper. Indeed, the proposed HTQ is best described as a state-dependent PS queue. 

% One can interpret the vehicles as jobs, and the road as a server. In this case, all the jobs are processed simultaneously, and the service rate of a given job is time-varying, and is equal to its instantaneous speed. The workload present in the system at any time is equal to the sum of the distances remaining to be traveled by the vehicles present in the system. The time-varying and state-dependent nature of the service rate also puts the proposed HTQ within the class of state-dependent queueing systems. However, the complex dependence of service rate on the state (i.e., vehicle locations) precludes use of existing tools from processor sharing queues and state-dependent queues for rigorous throughput analysis. 

In the PS queue literature, the focus has been on the sojourn time and queue length distribution. For example, see \cite{Ott:84} and \cite{Yashkov:83} for M/G/1-PS queue and 
\cite{Grishechkin:94} for G/G/1-PS queue. Fluid limit analysis for PS queue is provided in \cite{Chen.ea:97} and \cite{Gromoll.Puha.ea:02}. 
%For instance, for M/G/1-PS queue, the distribution of the sojourn time (see e.g. \cite{Ott:84} and \cite{Yashkov:83}) has been extensively investigated. Also, for G/G/1-PS queues, the limiting behavior of the queue length and sojourn time in the heavy traffic \cite{Grishechkin:94} and the fluid limit of the queue length  \cite{Chen.ea:97} and \cite{Gromoll.Puha.ea:02} have been studied. 
However, relatively less attention has been paid to the throughput analysis of state-dependent PS queues. %\ksmargin{please check if my rewording is correct}
In \cite{Moyal:08,Kherani.Kumar:02,Chen.Jordan:07}, throughput analysis for state-dependent PS queues is provided, where throughput is defined as the quantity of work achieved by the server per unit of time.
%
%In \cite{Moyal:08}, a stability criterion for processor sharing queues with state-dependent throughput has been proposed. However, the throughput in that paper is defined as the quantity of work achieved by the server per unit of time. For the same definition of the throughput, in \cite{Kherani.Kumar:02} and \cite{Chen.Jordan:07}, analytical expressions for throughput are derived.    
Stability analysis for a single server queue with workload-dependent service and arrival rate is provided in \cite{Bambos.Walrand:89} and \cite{Bekker:05}. However, the dependence of service rate on the system state in the HTQ proposed in the current paper is complex, and hence none of these results are readily applicable. 
%For example, the sharp transition in the throughput of HTQ from being finite to unbounded, as the car-following behavior transitions from sub-linear to sub-linear regime is an interesting phenomenon, and, to the best of our knowledge, does not have an analogue in the state-dependent queueing literature.

In summary, there are several novel contributions of the paper. First, we propose a novel horizontal traffic queue and place it in the context of processor-sharing queues and state-dependent queues. We establish monotonicity properties of service rates in between jumps (i.e., arrivals and departures), and derive bounds on change in service rates at jumps. 
Second, we adapt busy period calculations for M/G/1 queue to our current setup, including for non-empty initial conditions. These results allow us to provide tight results for throughput in the linear case, and probabilistic bounds on queue length over finite time horizon in the super-linear case. We also study throughput under a batch release control policy, whose effect is interpreted as a perturbation to the arrival process. We provide lower bound on the throughput for a maximum permissible perturbation for sub- and super-linear cases. In particular, we show that, for sufficiently large perturbation, this lower bound grows unbounded as $m \to 0^+$. It is interesting to compare our analytical results with simulation results, which suggest a sharp transition in the throughput from being unbounded in the sub-linear regime to being bounded in the super-linear regime. While our analytical results do not exhibit such a phase transition yet, their novelty is in providing rigorous estimates of any kind on the throughput of horizontal traffic queues under nonlinear car following models.
%
%prove a scaling of the minimum inter-vehicle distance in terms of the queue length, which in turn allows to show that the throughput is unbounded in the sub-linear case. 
%provide tight bounds on throughput in several scenarios. Third, we provide an instance of how tools from cooperative dynamical systems can be used to establish cardinal ordering between dynamical systems, even with different sizes. While not the main topic of the paper, we also comment on interpreting the proposed HTQ as a generalized processor sharing queue, and on using fluid limit of HTQ as a means to derive macroscopic constitutive laws in traffic flow theory.

The rest of the paper is organized as follows. We conclude this section with key notations to be used throughout the paper. The setting for the proposed horizontal traffic queue and formal definition of throughput are provided in Section~\ref{sec:problem-formulation}. Section~\ref{sec:service-rate-monotonicity} contains useful properties on the dynamics in service rate in between and during jumps. Key busy period properties for the M/G/1 queue are extended to the HTQ case in Section~\ref{sec:busy-period}. Throughput analysis is reported in Section~\ref{sec:throughput-analysis}. Simulations are presented in \ref{sec:simulations}. Concluding remarks and directions for future work are presented in Section~\ref{sec:conclusions}. A few technical intermediate results are collected in the appendix. 

\subsection*{Notations}
%\ksmargin{isn't $\tilde{\mc S}^L_n$ the interior of $\mc S^L_n$ ? If so, rather use the notation $\text{int}(\mc S_n^L)$}
Let $\RR$, $\RR_+$, and $\RR_{++}$ denote the set of real, non-negative real, and positive real numbers, respectively. 
%\sout{\kscomment{We use $x \in \RR_{o}^n$ to denote $x \in \RR^n$ satisfying the order $x_1 \leq \ldots \leq x_n$. $\RR^n_{+,o}$ and $\RR^n_{++,o}$ are defined similarly.}} 
Let $\NN$ be the set of natural numbers. 
%\mmmargin{these notations seem to be useful only for Lemma \ref{lemma:two-size-compare} and Proposition \ref{prop:queue-length-2m} but I think they are not consistent with those sections}
%\mmcomment{Given two vectors $x_1 \in \RR^{\mc A_1}$ and $x_2 \in \RR^{\mc A_2}$ for finite sets $\mc A_1$ and $\mc A_2$ with $|\mc A_1| \leq |\mc A_2|$, and an injective map $\map{\rho}{\mc A_1}{\mc A_2}$, , we use $x_1 \geq_{\rho} x_2$ (resp., $x_1 \leq_{\rho} x_2$) to imply $x_{1,i} \geq x_{2,\rho(i)}$ (resp., $x_{1,i} \leq x_{2,\rho(i)}$) for all $i \in \mc A_1$. }
If $x_1$ and $x_2$ are of the same size, then $x_1 \geq x_2$ implies element-wise inequality between $x_1$ and $x_2$. If $x_1$ and $x_2$ are of different sizes, then $x_1 \geq x_2$ implies inequality only between elements which are common to $x_1$ and $x_2$ -- such a common set of elements will be specified explicitly.  
%\ksmargin{Define $\mod$ also when $a<0$ \mmcomment{Done!}}
For a set $\mathcal{J}$, let $\text{int}(\mathcal{J})$ and  $|\mathcal{J}|$ denote the interior and cardinality of $\mathcal{J}$, respectively.
Given $a \in\RR$, and $b > 0$, we let $\mod(a,b):=a-\lfloor \frac{a}{b}\rfloor b$. Let $\mc S_N^L$ be the $N-1$-simplex over $L$, i.e., $\mc S_N^L=\setdef{x \in \RR_+^N}{\sum_{i=1}^N x_i = L}$. When $L=1$, we shall use the shorthand notation $\mc S_N$. %\kscomment{let $\tilde{\mc S}_n^L$ be a subset of $\mc S^L_n$ that does not contain the elements that have zero components i.e. $\tilde{\mc S}_n^L=\setdef{x \in \RR_{++}^n}{\sum_{i=1}^n x_i = L}$.}  
%\ksmargin{probably, we need to proofread the paper to be consistent with this notation}
When referring to the set $\until{N}$, for brevity, we let the indices $i=-1$ and $i=N+1$ correspond to $i=N$ and $i=1$ respectively.
 Also, for $p, q \in \mc S_N$, we let
%$H(p)$ denote the entropy of a probability vector $p$, and 
$D(p || q)$ denote the K-L divergence of $q$ from $p$, i.e., $D(p || q):= \sum_{i=1}^N p_i \log\left(p_i/q_i\right)$.
We also define a permutation matrix,  $P^- \in \{0,1\}^{N \times N}$,  as follows:
\begin{align*}
%\label{eq:matrix-definitions-alternate}
P^-:=\begin{bmatrix}
\zerobf_{N-1}^T & 1 \\
I_{N-1} & \zerobf_{N-1}
\end{bmatrix}
\end{align*}
where  $\zerobf_N$ and $\onebf_N$ stand for vectors of size $N$, all of whose entries are zero and one, respectively. We shall drop $N$ from $\mathbf{0}_N$ and $\mathbf{1}_N$ whenever it is clear from the context.





==> 02- submission/linear.tex <==
\subsection{Linear Case: $m=1$}
\label{sec:linear}
In this section, we provide an exact characterization of throughput for the linear case, i.e., when $m=1$. Recall that, for $m=1$, the service rate $s(y)=\sum_{i=1}^N y_i \equiv L$ is constant.

%In this case, the sum of speeds of all the vehicles present in the system at any time is constant, and is equal to $L$. 
%The sum of speeds of all vehicles is also equal to the rate of decrease of \emph{workload} in the queue. 
%%The workload for HTQ is the sum of distance left to be travelled for all the vehicles in the system. 
%%
%%
%%
%% 
%%
%%
%The workload $w(t)$ at time $t$ is the sum of the distances remaining to be travelled, i.e., residual distances, for all vehicles present at time $t$. In order to write an expression for $w(t)$, we define $s(t):=\sum_{i=1}^{A(t)} d_i$ as the residual added to the system by the $A(t)$ vehicles that arrive over $[0,t]$, and $I(t):=\int_0^t\delta_{\{w(s)=0\}}\de s$ as the cumulative \emph{idle time} up to time $t$. Therefore, $w(t)$ can be represented as 
%\be\label{eq:workload}
%w(t)=w(0) + s(t) -L(t-I(t))
%\ee
%where $w(0)$ is the initial workload.
%%
%%, and $I(t)$ denotes the cumulative \emph{idle time} up to time $t$, i.e., $I(t)=\int_0^t\delta_{\{w(s)=0\}}\de s$. 
%Since the residual distance of every vehicle is upper bounded by the total road length at every time instant, we have
%\be\label{eq:workload-upperbound}
%w(t) \leq n(t)\, L \, , \qquad \forall \, t \geq 0 \, .
%\ee

%The first two terms in the right hand side of \eqref{eq:workload} is the total workload added to the system by initial vehicles in the system and those arrived in $(0,t]$. On the other hand, the last term gives the amount of work provided by the server over $[0,t]$, so \eqref{eq:workload} gives the remaining workload in the system at time $t$. 
%An implication of \eqref{eq:workload-upperbound} is that unbounded workload implies unbounded queue length in our setting. We use this relationship to establish an upper bound on the throughput as follows.

%In our analysis, we use the workload process as a performance metric to determine the maximum throughput of the system.  Lemmas \ref{lemma:unstable} and \ref{lemma:stable} characterize the throughput of the system. 
%tWe first derive the expectation of busy periods of the queuing system and then establish the results for the maximum throughput. 
%\ksmargin{$\lambdamax$ here does not involve $\delta$ !}
\begin{proposition}\label{prop:unstable}
For any $L > 0$, $\varphi \in \Phi$, $\psi \in \Psi$, $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$ and :
$$
\lambdamax(L,m=1,\varphi,\psi,x_0,\delta=0) \leq L/\bar{\psi} \, .
$$ 
\end{proposition}
\begin{proof}
By contradiction, assume $\lambdamax>L/\bar{\psi}$. Let $r(t):=\sum_{i=1}^{A(t)} d_i$ be the workload added to the system by the $A(t)$ vehicles that arrive over $[0,t]$. Therefore, 
%$w(t)$ can be represented as,
\be\label{eq:workload-linear}
w(t)=w_0+r(t)-L(t-\mathcal{I}(t))
\ee
where $w_0$ is the initial workload. The process $\{r(t), \, t\geq 0\}$ is a renewal reward process, where the renewals correspond to arrivals of vehicles and the rewards correspond to the distances $\{d_i\}_{i=1}^{\infty}$ that vehicles wish to travel in the system upon arrival before their departures. 
%\ksmargin{can this be extended to general inter-arrival time distributions ? \mmcomment{yes ! }}
Inter-arrival times are exponential random variables with mean $1/\lambda$, and the reward associated with each renewal is independently and identically sampled from $\psi$, whose mean is $\bar{\psi}$.  
%
%time a renewal occurs we receive a reward which is the amount of work brought by the arrived vehicle. Let $R_i=L-v_i$ be the amount of reward at the time of $i$-th renewal and note that $\{R_i\}_{i=1}^\infty$ is an i.i.d sequence of random variables and $E[R_i]=E[R]=L-\bar\varphi$, 
%
Therefore, e.g., \cite[Theorem 3.6.1]{Ross:96} implies that, with probability one,  
\be
\label{eq:slln-renewal}
\lim_{t\to\infty}\frac{r(t)}{t}=\lambda \bar{\psi}
\ee
Thus, for all $\varepsilon \in \left(0,\lambda \bar{\psi} -L\right)$, there exists a $t_0\geq0$ such that, with probability one,
\be\label{eq:s-t-lowerbound}
\frac{r(t)}{t}\geq\lambda \bar \psi-\varepsilon/2> L + \varepsilon/2 \qquad \forall \, t \geq t_0.
\ee
Since $w_0$ and $\mathcal{I}(t)$ are both non-negative, \eqref{eq:workload-linear} implies that $w(t)\geq r(t) - Lt$ for all $t \geq 0$. 
%
%we have
%\be\label{eq:workload-lowerbound}
%W(t)\geq S(A(t))+Lt
%\ee
This combined with \eqref{eq:s-t-lowerbound} implies that, with probability one, $w(t) \geq \varepsilon t /2$ for all $t \geq t_0$, and hence 
$\lim_{t\to\infty}w(t)= + \infty$. This combined with \eqref{eq:workload-upperbound} implies that, with probability one, $\lim_{t\to\infty}N(t)=+\infty$. 
%Therefore, the steady-state number of vehicles in the system is infinity and this gives the lemma. 
\qed
\end{proof}

\begin{theorem}\label{thm:stable}
For any $L > 0$, $\varphi \in \Phi$, $\psi \in \Psi$, $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$:
$$
\lambdamax(L,m=1,\varphi,\psi,x_0,\delta=1) = L/\bar{\psi} \, .
$$ 
\end{theorem}
\begin{proof}
Assume that for some $\lambda < L/\bar{\psi}$, there exists some initial condition $(x_0,n_0)$ such that the queue length grows unbounded with some positive probability. 
Since the workload brought by every vehicle is i.i.d., and the inter-arrival times are exponential, without loss of generality, we can assume that the queue length never becomes zero. That is, the idle time satisfies $\mathcal{I}(t) \equiv 0$. Moreover, \eqref{eq:slln-renewal} implies that, for every $\varepsilon \in \left(0, L- \lambda \bar{\psi} \right)$, there exists $t_0 \geq 0$ such that, with probability one,
\begin{equation}
\label{eq:s-t-upperbound}
\frac{r(t)}{t} \leq \lambda \bar{\psi} + \varepsilon/2 < L - \varepsilon/2 \qquad \forall t \geq t_0
\end{equation} 

Combining \eqref{eq:workload-linear} with \eqref{eq:s-t-upperbound}, and substituting $\mathcal{I}(t) \equiv 0$, we get $w(t) < w_0 - \varepsilon t /2$, which implies that workload, and hence queue length, goes to zero in finite time after $t_0$, leading to a contradiction.  
%
%Taking into account Proposition~\ref{prop:unstable}, the only thing that remains to be proven is that, with probability one, the queue length remains bounded for any $\lambda < \frac{L}{\bar{\psi}}$ and any initial condition $x_0$. 
Combining this with the upper bound proven in Proposition~\ref{prop:unstable} gives the result. 
%
%By contradiction, assume that, there is a non-zero probability with which the queue length grows unbounded i.e. $\lim_{t\to\infty}N(t)=\infty$ starting from some initial condition $(x_0,n_0)$. On those sample paths we have $\lim_{t\to\infty} \frac{I(t)}{t}=0 $ which contradicts Proposition \ref{prop:long-run-idle-time}. 
%
%%By contradiction, we assume that the queue length grows unbounded i.e. $\lim_{t\to\infty}N(t)=\infty$ with some probability $\delta>0$ . Then we have
%%\be
%%\lim_{t\to\infty} \frac{\int_0^t\delta(N(s)=0)\de s}{t}=0
%%\ee
%%which contradicts Proposition \ref{prop:long-run-idle-time}. This contradiction proves that for any $\lambda<L/\bar \psi$, with probability one, the queue length remains bounded 
% 
\qed
\end{proof}

\begin{remark}
Theorem~\ref{thm:stable} implies that the throughput in the linear case is equal to the inverse of the 
time required to travel average total distance by a solitary vehicle in the system. In the linear case, the throughput can be characterized with probability one, independent of the initial condition of the queue. %Our throughput guarantees for the sub-linear case, though not tight, will also possess such property of being independent with respect to initial condition, and being true with probability one. However, our analysis for the super-linear case does not exhibit such nice properties. 
\end{remark}





==> 02- submission/nonlinear.tex <==
\subsection{Monotonicity of Throughput in $m$ and $x_0$}
\label{sec:non-linear}

%\ksmargin{write proof for Lemma~\ref{lem:throughput-bound-nonlinear}}
%One can easily get the following bounds for the nonlinear case.
%\begin{lemma}
%\label{lem:throughput-bound-nonlinear}
%For any $L > 0$, $\varphi \in \Phi$, $\psi \in \Psi$, $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$:
%$$
%\lambdamax(L,m,\varphi,\psi,x_0,\delta=1) \leq L/\bar{\psi} \quad \forall m \geq 1, \quad \& \quad  \lambdamax(L,m,\varphi,\psi,x_0,\delta=1) \geq L/\bar{\psi} \quad %\forall m \in (0,1]
%$$
%\end{lemma}
%\begin{proof}
%\end{proof}

In this section, we show the following monotonicity property of $\lambdamax$ with respect to $m$ for small values of $L$: for given $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$, $L \in (0,1)$, $\varphi \in \Phi$, and $\psi \in \Psi$, throughput is a monotonically decreasing function of $m$. 
%
%Figure \ref{fig:throughput-simulations} illustrates throughput values, for various values of $m\geq 0$, obtained through simulations.  The simulation results illustrate the monotonicity of $\lambdamax$ with respect to $m$ for small values of $L$, and this is formally proven in Proposition \ref{prop:queue-length-2m}. Moreover, simulation results suggest that throughput is unbounded for $m\in[0,1)$ (See Figure \ref{fig:throughput-simulations}). 
For this section, we rewrite \eqref{eq:dynamics-moving-coordinates} in $\RR_+^N$, i.e., without projecting onto $[0,L]^N$. Specifically, let the vehicle coordinates be given by the solution of 
% The following lemma compares two car-following behaviors chosen from \eqref{eq:speed-moving-coordinates} when no arrival or departure is allowed. It shows that the system with higher exponent lags behind the other one. %In other words, vehicles move faster in the system with smaller exponent. 
%\ksmargin{need to add more explanation here}
%\kscomment{For this section, we rewrite the dynamics from \eqref{eq:dynamics-moving-coordinates} to express the vehicle coordinates in $\RR_+^n$ instead of projecting on to $[0,L]^n$. }The corresponding dynamics is given by:
\begin{equation}
\label{eq:x-dynamics-in-Rn}
\dot{x}_i = y_i^m, \qquad x_i(0)=x_{0,i}, \qquad i \in \until{N} 
\end{equation} 
Let $X(t;x_0,m)$ denote the solution to \eqref{eq:x-dynamics-in-Rn} at $t$ starting from $x_0$ at $t=0$. We will compare $X(t;x_0,m)$ under different values of $m$ and initial conditions $x_0$, over an interval of the kind $[0,\tau)$, in between arrivals and departures. 
We recall the notation that, if $x_{0}^1$ and $x_{0}^2$ are vectors of different sizes, then $x_{0}^1 \leq x_{0}^2$ implies element-wise inequality only for components which are common to $x_{0}^1$ and $x_{0}^2$. In Lemma~\ref{lemma:two-size-compare} and Proposition~\ref{prop:queue-length-2m}, this common set of components corresponds to the set of vehicles common between $x_{0}^1$ and $x_{0}^2$.
 
% \begin{lemma}\label{lemma:two-m-compare}
%Consider two HTQs with \mmcomment{$L=1$} and the same initial condition, $x_0$, and no arrival or departure is allowed. These systems implements different car following model given as,
%$$\dot x_{1,i} =g_1(x)_i=y_{1,i}^{m_1}, \quad \text{and} \quad \dot x_{2,i} = g_2(x)_i=y_{2,i}^{m_2}$$
%where  $m_2\geq m_1\geq 0$. Then, 
%$$x_2(t;x_0)\preceq x_1(t;x_0) \quad \forall t\geq0$$
% \end{lemma}
% \begin{proof}
%First, observe that for all $y\in\mc S_n$, $y_i^{m_2}\leq y_i^{m_1}$ for all $i\in{\{1,2,\cdots,n\}}$. This implies, $g_2(x)\preceq g_1(x)$ for all $x$. This fact combined with Lemma \ref{lem:monotonicity-same-size} in Appendix establishes this lemma.
% \end{proof}
%Now, the following Lemma compares two systems with the same car-following behavior, but different dimensions and shows that the presence of an arrival, makes other vehicles to slow down an evolve slower. 
%
%For the next lemma, 

\begin{lemma}
\label{lemma:two-size-compare}
For any $L \in (0,1]$, $x^1_{0} \in \RR_+^{n_1}$, $x^2_{0} \in \RR_+^{n_2}$, $n_1, n_2 \in \NN$,
$$
x^1_{0} \leq x^2_{0}, \, \, n_2 \leq n_1, \, \,  0 < m_2 \leq m_1 \implies X(t;x^1_{0},m_1) \leq X(t;x^2_{0},m_2) \qquad \forall \, t \in [0,\tau)
$$ 
\end{lemma}
%
%\begin{lemma}\label{lemma:two-size-compare}
% Consider two HTQs with \mmcomment{$L=1$}, identical car-following behavior \eqref{eq:speed-moving-coordinates} and $x_0$ with size $n$.  At time $t=t_0>0$, for the first time, one new vehicle arrives at an arbitrary location in the first system, but the second system remains unchanged. For all $t>t_0$, both systems remain closed (i.e. no more arrival or departure). Let $x^{(1)}(t)\in \mathbb{R}^n$ and $x^{(2)}(t)\in \mathbb{R}^n$ denote the position of the initial $n$ vehicles at time $t$ in the first and second system, respectively. Then, 
%$$x^{(1)}(t)\preceq x^{(2)}(t) \quad \forall t\geq 0$$
% \end{lemma}
 \begin{proof}
The proof is straightforward when $n_1=n_2$. This is because, in this case, since $y_i \leq L\leq1$,  $m_2 \leq m_1$ implies $y_i^{m_2} \geq y_i^{m_1}$ for all $i \in \until{n_1}$. Using this with Lemmas~\ref{lem:monotonicity-same-size} and \ref{lem:car-following-type-K} gives the result. 
 
% First, observe that for all $y\in\mc S_n$, $y_i^{m_2}\leq y_i^{m_1}$ for all $i\in{\{1,2,\cdots,n\}}$. This implies, $g_2(x)\preceq g_1(x)$ for all $x$. This fact combined with Lemma \ref{lem:monotonicity-same-size} in Appendix establishes this lemma.
In order to prove  the result for $n_2 < n_1$, we show that $X(t; x^1_{0}, m_1) \leq X(t; x^2_{0}, m_1) \leq X(t; x^2_{0}, m_2)$. Note that the second inequality follows from the previous case. Therefore, it remains to prove the first inequality. Let $(i_1, \ldots, i_{n_2})$ be the set of indices of $n_2$ vehicles such that $0 \leq x^2_{0,i_1} \leq \ldots \leq x^2_{0,i_{n_2}} \leq L$. Similarly, let $(i_1, i_1+1, \ldots, i_2, i_2+1, \ldots)$ be the indices of $n_1$ vehicles in the order of increasing coordinates in $x_0^1$. Our assumption on the initial condition implies that $x^1_{0,i_k} \leq x^2_{0,i_k}$ for all $k \in \until{n_2}$. For brevity, let $x^1(t) \equiv X(t;x_0^1,m_1)$, and $x^2(t) \equiv X(t;x_0^2,m_1)$. It is easy to check that, for all $t \in [0,\tau)$, and all $k \in \until{n_2}$, 
\begin{equation}
\label{eq:xdot-ub}
\dot{x}^1_{i_k} = \left(x^1_{i_{k}+1} - x^1_{i_k}\right)^{m_1} \leq \left(x^1_{i_{k+1}} - x^1_{i_k}\right)^{m_1}
\end{equation}
Let $t \in [0,\tau)$ be the first time instant when $x^1_{i_k}(t)=x^2_{i_k}(t)$ for some $k \in \until{n_2}$. Then, recalling $x^1_{i_{k+1}}(t) \leq x^2_{i_{k+1}}(t)$, \eqref{eq:xdot-ub} implies that $\dot{x}_{i_k}^1(t) \leq \left(x^2_{i_{k+1}} - x^2_{i_k} \right)^{m_1} = \dot{x}^2_{i_k}(t)$. The result then follows from Lemma~\ref{lem:monotonicity-same-size}.  
% 
% 
%The result holds with equality for $0\leq t \leq t_0$ since both systems start with the same initial condition and implement the same car-following behavior. The second system remains closed for all $t\geq 0$ and the dynamics is given by $\dot x^{(2)}=h(x^{(2)})$ where $h$ is a $n$ dimensional vector generator.  Let us assume, without loss of generality, that the new arrival of the first system is located between $j$th and $(j+1)$st vehicles and let $x_{j'}\leq x_{j+1}$ denote its location.   
% Immediately after $t=t_0$, the first system switches to a $n+1$ dimensional system; however, we want to keep track of only the initial $n$ vehicles. For this purpose, we can approximate the dynamics of the initial $n$ vehicles as,
% \begin{align}\label{eq:lag-new-arrival}
%{ \dot x_i^{(1)}} &=(x_{i+1}^{(1)}-x_i^{(1)})^m = h(x^{(1)})_i\quad \forall i\neq j , j+1 \nonumber \\
% { \dot x_j^{(1)}}& =(x_{j'}-x_{j}^{(1)})^m \leq (x_{j+1}^{(1)}-x_{j}^{(1)})^m = h(x^{(1)})_j
% \end{align} 
%This implies that $\dot x^{(1)} =f(x^{(1)})\preceq h(x^{(1)})$ for all $x^{(1)}\in \mathbb{R}^n$. This combined with the fact that $x^{(1)}(t_0)=x^{(2)}(t_0)$ and Lemma \ref{lem:monotonicity-same-size} establishes the result. 
\qed
 \end{proof}
 
%\ksmargin{needs rewording} 
%\kscomment{ Basically, the above Lemma shows an intuitive fact about the system. It shows for $m\geq 1$ ($m<1$) each vehicles will slow down (speed up) in the presence of new arrival and they lag behind (go ahead of) the vehicles in a system without arrival. 
%} 
 
% \begin{remark}\label{remark:higher-dim-compare}
% By using the similar arguments as in Lemma \ref{lemma:two-size-compare}, one can show that removal (or departure) of one vehicle from a system, makes the remaining vehicles to speed up and evolve faster. 
% \end{remark}

Lemma~\ref{lemma:two-size-compare} is used to establish monotonicity of throughput as follows.
\begin{proposition}
\label{prop:queue-length-2m}
For any $L \in (0,1]$, $\varphi \in \Phi$, $\psi \in \Psi$, $\delta \in (0,1)$, $x^1_{0} \in [0,L]^{n_1}$, $x^2_{0} \in [0,L]^{n_2}$, $n_1, n_2 \in \NN$:
$$
x^1_{0} \leq x^2_{0}, \, \, n_2 \leq n_1, \, \,  0 < m_2 \leq m_1 \implies \lambdamax(L,m_1,\varphi,\psi,x^1_0,\delta)  \leq \lambdamax(L,m_2,\varphi,\psi,x^2_0,\delta)
$$
\end{proposition}
\begin{proof}
For brevity in notation, we refer to the queue corresponding to $m_1$, and initial condition $x_0^1$ as HTQ-S. We refer to the other queue as HTQ-F. Let $\lambda$, $\varphi$ and $\psi$ common to HTQ-S and HTQ-F be given.  Let $x^1(t) \equiv X(t; x^1_0, m_1)$ and $x^2(t) \equiv X(t; x^2_0, m_2)$, and let $N_s(t)$ and $N_f(t)$ be the queue lengths in the two queues at time $t$. It suffices to show that $N_s(t) \geq N_f(t)$ for a given realization of arrival times, arrival locations, and travel distances. In particular, this also implies that the departure locations are also the same for every vehicle, including the vehicles present at $t=0$, in both the queues.  
%We show this using Lemma~\ref{lemma:two-size-compare}.
%\end{proof}
%
%\begin{proposition}\label{prop:queue-length-2m}
%Consider two HTQ  with the same $\lambda>0$, $\varphi, \psi\in\Psi$, $x_0$ and \mmcomment{$L=1$}. Let $m_1$ and $m_2$ ($m_2\geq m_1 \geq 0$) be the exponents of the car-following behavior \eqref{eq:speed-moving-coordinates} implemented by the first and second system, respectively. Then, 
%$$N_1(t)\leq N_2(t) \quad \forall t\geq 0$$
%where $N_1(t)$ and $N_2(t)$ denote the queue length of the first and second system at time $t$, respectively. 
%\end{proposition}
% 
% \begin{proof}

Indeed, it is sufficient to show that $x^1(\tau) \leq x^2(\tau)$ and $N_s(\tau)\geq N_f(\tau)$ where $\tau$ is the time of first arrival or departure from either HTQ-S or HTQ-F. Accordingly, we consider two cases, corresponding to whether $\tau$ corresponds to arrival or departure. 

Since $x^1(t) \leq x^2(t)$ for all $t \in [0,\tau)$ from Lemma~\ref{lemma:two-size-compare}, and the departure locations of all the vehicles in HTQ-S and HTQ-F are identical, the first departure from HTQ-S can not happen before the first departure in HTQ-F. Therefore, $N_s(\tau) \geq N_f(\tau)$. Since $x^1(\tau^-) \leq x^2(\tau^-)$, and $x^2(\tau)$ is a subset of $x^2(\tau^-)$, we also have $x^1(\tau) \leq x^2(\tau)$. 

When $\tau$ corresponds to the time of the first arrival, since the arrivals happen at the same location in HTQ-S and HTQ-F, and since $x^1(\tau^-) \leq x^2(\tau^-)$, rearrangement of the indices of the vehicles to include the new arrival at $t=\tau$ implies that $x^1(\tau) \leq x^2(\tau)$. Moreover, since $N_s(\tau^-) \geq N_f(\tau^-)$, and the arrivals happen simultaneously in both HTQ-S and HTQ-F, we have $N_s(\tau) \leq N_f(\tau)$. 
%
%Lemma~\ref{lemma:two-size-compare} implies that, if $i_k$ is the index of the vehicle which departs from HTQ2, then $x^1_{i_k}(\tau) \leq x^2_{i_k}(\tau)$. This also implies that the first
%
%, and hence the number of departures over $[0,\tau)$ is at most one, i.e., $N_1(\tau) \geq N_2(\tau)$
%
%Consider the same realization of the tempora-spatial arrival process for both systems. let $t_{d_j}$ be the time at which $j$th departure happens in the second system. We claim that $N_1(t_{d_j}^+)\leq N_2(t_{d_j}^+)$ for all $j\in\{1,2,3,\cdots\}$.
%%Let fix a realization of the arrival process as $A=\{a_1,a_2,\cdots\}$ where $a_i$ represents the time of $i$th arrival.  
%%This means that after each departure epoch in the second system, the queue length in the first system is no more than the second one. 
%Since the realization of arrival process is considered to be the same for both systems, this will imply the result of this proposition. We proceed by using induction to show that this claim holds.
%
%
%
%For the base case, since systems start with the same initial condition, by Lemma \ref{lemma:two-m-compare}, we know that the vehicles in the first system move faster. This means that the earliest departure is from the first system at time $t=t_0\leq t_{d_1}$. In $[t_0,t_{d_1}]$, there could be zero or more departures from the first system. In either cases, we have $N_1(t_{d_1}^+)\leq N_2(t_{d_1}^+)$ and the claim holds the base case.  
%
%Now, assume that the claim holds for the $k$th departure from the second system, we show that it also holds for the $(k+1)$st departure. By the induction hypothesis, $N_1(t_{d_k}^+)\leq N_2(t_{d_k}^+)$. Let $e=N_2(t_{d_k}^+) - N_1(t_{d_k}^+)$. Now, two cases can happen: (1) $e=0$, and (2) $e>0$. In the first case, by Lemmas \ref{lemma:two-m-compare}, \ref{lemma:two-size-compare} and Remark \ref{remark:higher-dim-compare} we know that the position of the $i$th vehicle in the second system is ahead or equal to the position of the $i$th vehicle in the second system, but let consider a conservative scenario in which the position of the $i$th vehicle in both systems are equal. Again, by further usage of Lemma \ref{lemma:two-m-compare}, one can observe that the earliest departure will from the first system. By using the same arguments as for base case of induction, it can be shown that claim holds. For the second case, consider a conservative scenario in which the earliest departure will be from the second system. Thus, we get $N_2(t_{d_{k+1}})-N_1(t_{d_{k+1}})=e-1\geq 0$, which automatically proves the claim. Thus, by this induction, we showed that our claim holds and this establishes this proposition. 
\qed
\end{proof}

\begin{remark}
Proposition \ref{prop:queue-length-2m} establishes monotonicity of throughput only for $L\in(0,1]$. This is consistent with our simulation studies, e.g., as reported in Figure \ref{fig:throughput-simulations}, according to which, the throughput is non-monotonic for large $L$. 
%
%In fact, simulations suggest that, for $L$ sufficiently large, this monotonicity is not true (See Figure \ref{fig:throughput-simulations}).
\end{remark}
For the analysis of the linear car following model, we exploited the fact that the total service rate of the system is constant. However, for the nonlinear model, i.e., $m \neq 1$, the total service rate depends on the number and relative locations of vehicles. The state dependent service rate of nonlinear models makes the throughput analysis much more complex. In the next section, we find probabilistic bound on the throughput in the super-linear case.
%
%Let $\{\tau_1, \tau_2, \ldots \}$, with $0 \leq \tau_1 < \tau_2 < \ldots$, \footnote{\kscomment{The strict inequality holds with probability one}.} correspond to \emph{jumps}, i.e., arrival and departure epochs. 
%We first analyze the dynamics in between jumps, i.e., over an interval of the type $[\tau_{\ell},\tau_{\ell+1})$ under \eqref{eq:inter-vehicle-distance-Rn}-\eqref{eq:dynamics-moving-coordinates}. 

%\subsection{Dynamics in between jumps}
%For brevity in notation, and without loss of generality, we let $[\tau_{\ell},\tau_{\ell+1})=[0,\tau)$, and $n=N(\tau_{\ell})$ be the constant queue length during this time interval, and let $x_0=x(\tau_{\ell}) \in \RR_+^n$ be the vehicle coordinates at the beginning of the time interval. 

%\input{KL-divergence}

%\input{quadratic}

%\input{additional-results}






%\input{super-linear}
%\input{sub-linear}


==> 02- submission/problem-formulation.tex <==
\section{The Horizontal Traffic Queue (HTQ) Setup}
\label{sec:problem-formulation}
%Consider the following setup for a horizontal traffic queue (HTQ). 
Consider a periodic road segment of length $L$; without loss of generality, we assume it be a circle. Starting from an arbitrary point on the circle, we assign coordinates in $[0,L]$ to the circle in the clock-wise direction (See Figure \ref{fig:htq}). Vehicles arrive on the circle according to a spatio-temporal process: the arrival process $\{A(t),t\geq0\}$, is assumed to be a Poisson process with rate $\lambda>0$, and the arrival locations are sampled independently and identically from a spatial distribution $\varphi$ and mean value $\bar \varphi$. Without loss of generality, let the support of $\varphi$ be $\text{supp}(\varphi)=[0,\ell]$ for some $\ell\in[0,L]$. 
Upon arriving, vehicle $i$ travels distance $d_i$ in a counter-clockwise direction, after which it departs the system. 
%Upon arrival at coordinate $v_i$, the corresponding vehicle travels in the clock-wise direction for distance $d_i$, and departs the system once it reaches the coordinate $v_i + d_i$.
%a periodic road segment of length $L$ from external world at coordinates  \ksmargin{somehow it seems that $\varphi$ is irrelevant}
%\ksmargin{The notation $C$ is in conflict with notation for busy period distribution: \mmcomment{I changed it to $R$}}
The travel distances $\{d_i\}_{i=1}^\infty$ are sampled independently and identically from a spatial distribution $\psi$ with support $[0,R]$ and mean value $\bar \psi$. %\ksmargin{is the footnote useful ?}
%\footnote{Note that the finite support of $\varphi$ and $\psi$ implies that they have finite variances.} 
Let the set of $\varphi$ and $\psi$ satisfying the above conditions be denoted by $\Phi$ and $\Psi$ respectively. % \ksmargin{do we need to impose some regularity conditions on $\varphi$ and $\psi$ ?}
The stochastic processes for arrival times, arrival locations, and travel distances are all assumed to be independent of each other.
%If $v_i + d_i \geq L$ for some vehicle, then the coordinate of departure location for that vehicle is $\mod \left(v_i + d_i, L \right)$.  


\begin{figure}[htb!]
 \centering
 \includegraphics[width=5cm]{htq-colorful} 
  \caption{Illustration of the proposed HTQ with three vehicles.}
    \label{fig:htq}
\end{figure}




%\begin{remark}
%\label{rem:coordinate-modulus}
%Considering the periodic geometry of our setup, unless stated otherwise, whenever we mention a coordinate, we implicitly assume it to be modulus $L$. For example $x=5L/2$ corresponds to $x=L/2$.
%\end{remark}




%\sout{We say that the HTQ is \emph{idle} whenever there is no vehicle in the system and process $\{I(t),t\geq 0\}$ represents the cumulative amount of idle time up to time $t$.}

%ksmargin{do we need the notation $A(t)$ ?}
%Vehicle $i$ brings $L-v_i$ amount of the work to the system which is the distance between its arrival location and departure point. 
%Let $\{S(i), i=1,2,\cdots\}$ be the \emph{service process} where $S(i)$ records the total amount of work added to the system by first $i$ vehicles i.e. $S(i)=\sum_{j=1}^i(L-v_j)$. 
%We consider a first order kinematic model for vehicle motion during its stay in the queue, where the speed of a vehicle is proportional to a power of the distance to the vehicle directly in front of it. 

% \mmcomment{We describe the dynamics of vehicle coordinates under first order car following models in between jumps, and during jumps. }

\subsection{Dynamics of vehicle coordinates between jumps}
Let the time epochs corresponding to arrival and departure of vehicles be denoted as $\{\tau_1, \tau_2, \ldots\}$. We shall refer to these events succinctly as \emph{jumps}. We now formally state the dynamics under this car-following model. 
We describe the dynamics over an arbitrary time interval of the kind $[\tau_j,\tau_{j+1})$. Let $N \in \NN$ be the fixed number of vehicles in the system during this time interval. 
%\sout{It will be useful to express the dynamics in $\RR_+$ as well as in the natural coordinates in $[0,L]$.} 
Define the inter-vehicle distances associated with vehicle coordinates $x \in [0,L]^N$ as follows:
%\textbf{Dynamics in $\RR_+^n$}: Let $x(\tau_{\ell})=\left(x_1(\tau_{\ell}), \ldots,x_n(\tau_{\ell}) \right) \in \RR_+^n$ be the coordinates of the vehicles at the beginning of the time interval, arranged in a clock-wise order such that $x_1(\tau_{\ell}) \leq \ldots \leq x_n(\tau_{\ell})$. For this purpose, we define the inter-vehicular distances as:
\begin{equation}
\label{eq:inter-vehicle-distance-Rn}
%\begin{split}
y_i(x)  = \mod \left(x_{i+1} - x_i, L\right), \quad i \in \until{N} 
%\\
%y_n(x) & = L+ x_1 - x_n.
%\end{split}
\end{equation}
where we implicitly let $x_{N+1} \equiv x_1$ (See Figure \ref{fig:htq} for an illustration). Note that the normalized inter-vehicle distances $y/L$ are probability vectors. 
When inside the queue, the speed of every vehicle is proportional to a power $m >0$ of the distance to the vehicle directly in front of it. 
We assume that this power $m > 0$ is the same for every vehicle at all times. Then, starting with $x(\tau_{j}) \in [0,L]^N$, the vehicle coordinates over $[\tau_{j},\tau_{j+1})$ are given by:
%\begin{equation}
%\label{eq:speed-moving-coordinates}
%\dot{x}_i = y_i^m(x), \qquad i \in \until{n},
%\end{equation}
%or, equivalently,
\begin{equation}
\label{eq:dynamics-moving-coordinates}
x_i(t) = \mod \left( x_i(\tau_{j}) + \int_{\tau_{j}}^t y_i^m(x(z)) \, dz, L \right), \qquad \forall \, i \in \until{N}, \quad \forall \, t \in [\tau_{j},\tau_{j+1}) \, ,
\end{equation}
%where $y(x)$ is given by \eqref{eq:inter-vehicle-distance-Rn}.
%\mmmargin{add a figure here...}
%\textbf{Dynamics in $[0,L]^n$}:
%Let $x(\tau_{\ell})=\left(x_1(\tau_{\ell}), \ldots,x_n(\tau_{\ell}) \right) \in [0,L]^n$ be the coordinates of the vehicles at the beginning of the time interval, arranged in a clock-wise order such that $x_1(\tau_{\ell}) \leq \ldots \leq x_n(\tau_{\ell})$. For this purpose, we define the inter-vehicular distances as:
%\begin{equation}
%\label{eq:inter-vehicular-distance}
%\begin{split}
%%\alpha
%y_i(x) & =  x_{i+1} - x_i, \quad i \in \until{n-1} \setminus \{k\} \\
%y_n(x) & = L+ x_1 - x_n, \quad n = k \\
%y_n(x) & = x_1 - x_n, \quad n \neq k \\
%y_k(x)  & = L+x_{k+1} - x_k, \quad n \neq k.
%\end{split}
%\end{equation}
%The instantaneous speed of every vehicle is given by the same expression as in \eqref{eq:dynamics-moving-coordinates}, with $y(x)$ given by \eqref{eq:inter-vehicular-distance}. The vehicle coordinates are then given by:
%\begin{equation}
%\label{eq:dynamics-fixed-coordinates}
%x_i(t)=\mod \left(x_i(\tau_{\ell}) + \int_{\tau_{\ell}}^t y_i^m(x(s)) \, ds , L\right) \qquad \forall \, i \in \until{n}, \quad \forall \, t \in [\tau_{\ell},\tau_{\ell+1})\, ,
%\end{equation}
%where we recall the definition of $\mod$ function from Section~\ref{sec:introduction}.

\begin{remark}
%\begin{enumerate}
%\item 
It is easy to see that the clock-wise ordering of the vehicles is invariant under \eqref{eq:inter-vehicle-distance-Rn}-\eqref{eq:dynamics-moving-coordinates}. 
%\item \kscomment{The solution to \eqref{eq:inter-vehicle-distance-Rn}-\eqref{eq:dynamics-moving-coordinates} satisfies $x_n(t)-x_1(t) \leq L$ for all $t \in [\tau_{\ell}, \tau_{\ell+1})$.}
%\ksmargin{add a short explanation here}
%\item If $\tilde{x}(t)$ and $\hat{x}(t)$ denote the vehicle coordinates under \eqref{eq:inter-vehicle-distance-Rn}-\eqref{eq:dynamics-moving-coordinates} and \eqref{eq:inter-vehicular-distance}-\eqref{eq:dynamics-fixed-coordinates} respectively, starting from the same initial condition $x(\tau_{\ell})$, then $\hat{x}_i(t)=\mod \left(\tilde{x}_i(t),L\right)$ for all $i \in \until{n}$ and for all $t \in [\tau_{\ell},\tau_{\ell+1})$.
%\end{enumerate}
\end{remark}

%The dynamics in inter-vehicle distances however is the same in both coordinate system. If $y(\tau_{\ell})$ is the inter-vehicular distance at $t=\tau_{\ell}$, computed through \eqref{eq:inter-vehicle-distance-Rn} or \eqref{eq:inter-vehicular-distance}, then its subsequent values over $[\tau_{\ell},\tau_{\ell+1})$ are given by the solution to:
The dynamics in inter-vehicle distances is given by:
\begin{equation}
\label{eq:inter-vehicle-distance-dynamics}
%\begin{split}
\dot{y}_i = y^m_{i+1} - y_i^m, \qquad i \in \until{N} 
%\\
%\dot{y}_n & = y^m_1 - y^m_n.
%\end{split}
\end{equation}
where we implicitly let $y_{N+1} \equiv y_1$.

\subsection{Change in vehicle coordinates during jumps}
%We describe the change in vehicle coordinates during jumps in $[0,L]$; the change in $\RR_+$ can be described analogously. 
Let $x(\tau^-_{j}) =\left(x_1(\tau^-_{j}), \ldots, x_N(\tau^-_{j})\right) \in [0,L]^N$ be the vehicle coordinates just before the jump at $\tau_{j}$. If the jump corresponds to the departure of vehicle $k \in \until{N}$, then the coordinates of the vehicles $x(\tau_{j}) =\left(x_1(\tau_{j}), \ldots, x_{N-1}(\tau_{j})\right) \in [0,L]^{N-1}$ after re-ordering due to the jump, for $i \in \until{N-1}$, are given by:
 \begin{equation*}
		x_i(\tau_{j})=\left\{\begin{array}{ll}
		\ds x_i(\tau^-_{j}) 	& i\in \until{k-1} \\[15pt]
		\ds x_{i+1}(\tau^-_{j})	& i\in \{k+1, \ldots, N-1\}\,.\end{array}\right.
	\end{equation*}

 Analogously, if the jump corresponds to arrival of a vehicle at location $z \in [0,\ell]$ in between the locations of the $k$-th and $k+1$-th vehicles at time $\tau_{j}^-$, then the coordinates of the vehicles $x(\tau_{j}) =\left(x_1(\tau_{j}), \ldots, x_{N+1}(\tau_{j})\right) \in [0,L]^{N+1}$ after re-ordering due to the jump, for $i \in \until{N+1}$, are given by:
 \begin{equation*}
 \begin{split}
 x_{k+1}(\tau_{j}) & = z \\
		x_i(\tau_{j}) & =\left\{\begin{array}{ll}
		\ds x_i(\tau^-_{j}) 	& i\in \until{k} \\[15pt]
		\ds x_{i-1}(\tau^-_{j})	& i\in \{k+2, \ldots, N+1\}\,.\end{array}\right.
		\end{split}
	\end{equation*}

\subsection{Problem statement}
Let $x_0 \in [0,L]^{n_0}$ be the initial coordinates of $n_0$ vehicles present at $t=0$. An HTQ is described by the tuple $\left(L, m, \lambda, \varphi, \psi, x_0\right)$. 
%\kscomment{We use HTQ and \emph{system} interchangeably in the paper.} \ksmargin{it would be better of we used either HTQ or system consistently in the paper}
%We let $X(t) \in \real^n$ denote the coordinates of vehicles at time $t$ 
%
%
%Let $x_i(t) \in [0,L]$ be the location of the $i$-th vehicle at time $t$, and $N(t)$ be the number of vehicles on the road at time $t$. Let $k_1, \ldots, k_{N(t)}$ be the indices of the vehicles present at time $t$, such that $x_{k_i}(t) \leq x_{k_{i+1}}(t)$ for all $i \in \until{N(t)-1}$. Note that this ordering remains invariant between arrival and departure epochs. The speed of each vehicle, $\dot{x}_{k_i}=y_{k_i}$, $i=1, \ldots, N(t)$,  is given by:
%%\ksmargin{do we need all the notations used in \eqref{eq:car-following-model}}
%\begin{equation}
%\label{eq:car-following-model}
%\begin{split}
%y_{k_i} & =  \left( x_{k_{i+1}} - x_{k_i} \right)^m, \quad i = 1, \ldots, N(t)-1 \\
%y_{k_{N(t)}} & = \left( L+ x_{k_1}-x_{k_{N(t)}} \right)^m,
%\end{split}
%\end{equation}
%where $m \geq 0$ is the parameter for the kinematics.
%Note that \eqref{eq:car-following-model} implies that the speed of the vehicle closest to the exit point is influenced by its relative distance with respect to vehicle number $k_1$. This is a consequence of our circular road setup. The variables $y_i$ represent the inter-vehicular spacings.
%\ksmargin{Emphasize that $X()$ and $N()$ are stochastic}
Let 
%$X(t;L, m, \lambda \varphi, \psi, x_0)$ denote the coordinates of vehicles in a given HTQ $\left(L, m, \lambda, \varphi, \psi, x_0\right)$ at time $t \geq 0$, and let 
$N(t;L, m, \lambda, \varphi, \psi, x_0)$ be the corresponding queue length, i.e., the number of vehicles at time $t$ for an HTQ $\left(L, m, \lambda, \varphi, \psi, x_0\right)$. For brevity in notation, at times, we shall not show the dependence of $N$ on parameters which are clear from the context.


%Since this is a novel state-dependent queue, in this paper, we establish useful properties of this queueing system such as monotonicity of the service in between jumps, and busy period distribution. Then, we show the application of these properties in establishing useful bounds on throughput that is defined in the following. 

In this paper, our objective is to provide rigorous characterizations of the dynamics of the proposed HTQ. A key quantity that we study is throughput, defined below.  
 
%\ksmargin{clarify what distribution is $\Pr$ with respect to} 
\begin{definition}[Throughput of HTQ]\label{def:throughput}
Given $L > 0$, $m > 0$, $\varphi \in \Phi , \psi \in \Psi$, $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$ and $\delta \in [0,1)$, 
%\begin{enumerate}
%\item 
the throughput of HTQ is defined as:
\begin{equation}
\label{eq:throughput-def}
\lambdamax(L,m,\varphi,\psi,x_0,\delta):= \sup \left\{\lambda \geq 0: \, \Pr \left( N(t;L, m, \lambda, \varphi, \psi, x_0) < + \infty, \quad \forall t \geq 0  \right) \geq 1 - \delta  \right\}.
\end{equation}
%\end{enumerate}
\end{definition}

%Our objective in this paper is to rigorously characterize $\lambdamax(m,L,\varphi,\psi,x_0,\delta)$. In particular, we study sufficient conditions on $\left(L, m, \lambda, \varphi, \psi, x_0\right)$, under which the queue length remains bounded. We are particularly interested in 
%analyzing the dependency of the boundedness of queue length on $\lambda$ and $x_0$ for given $\left(L, m, \varphi, \psi \right)$.

Figure~\ref{fig:throughput-simulations} shows the complex dependency of throughput on key queue parameters such as $m$ and $L$. In particular, it shows that for every $L$, $\varphi$, $\psi$, $x_0$ and $\varphi$, the throughput exhibits a phase transition from being unbounded for $m \in (0,1)$ to being bounded for $m>1$. Moreover, Figure~\ref{fig:throughput-simulations} also suggests that, for sufficiently small $L$, throughput is monotonically non-increasing in $m$, and that it is monotonically non-decreasing in $m>1$, for sufficiently large $L$. Also, it can be observed that initial condition can also affect the throughput. We now develop analytical results that match the throughput profile in Figure~\ref{fig:throughput-simulations} as closely as possible. To that purpose, we will make extensive use of novel properties of \emph{service rate} and \emph{busy period} of the proposed HTQ, which could be of independent interest. 


\begin{figure}
\centering
\subfigure[]{\includegraphics[width=6cm]{phase-transition-4L-n0}}
\centering
\hspace{0.3in}
\subfigure[]{\includegraphics[width=6cm]{phase-transition-5L-n100}}\\
\subfigure[]{\includegraphics[width=6cm]{phase-transition-4L-n0-unif}}
\centering
\hspace{0.3in}
\subfigure[]{\includegraphics[width=6cm]{phase-transition-5L-n100-unif}}
\caption{Throughput for various combinations of $m$, $L$, and $n_0$.  The parameters used in individual cases are:  (a) $\varphi=\delta_{0}$, $\psi = \delta_L$, and $n_0=0$ (b) $\varphi=\delta_{0}$, $\psi = \delta_L$, and $n_0=100$ (c) $\varphi=U_{[0,L]}$, $\psi = U_{[0,L]}$, and $n_0=0$ (d) $\varphi=U_{[0,L]}$, $\psi = U_{[0,L]}$, and $n_0=100$. In all the cases, the locations of initial $n_0$ vehicles were chosen at equal spacing in $[0,L]$.
 \label{fig:throughput-simulations}}
\end{figure}


%\kscomment{With a slight abuse of notation, we shall use $\lambdamax(m,L,\varphi,\psi,\delta)$ to imply $\lambdamax(m,L,\varphi,\psi)$.}

%Our main result is the following:
%\ksmargin{For the deterministic case, I think that the throughput depends on $N(0)$}
%\begin{theorem}
%\label{thm:main}
%For $L = 1$ and any $\varphi$,
%\begin{equation*}
%\lambdamax(m,L,\varphi) = \left\{\ba{ll} 
%+ \infty & 0 \leq m < 1 \\
%1/(1-\bar{\varphi}) & m=1 \\
%0 & m > 1 
%\ea\right.
%\end{equation*}
%\end{theorem}

%\ksmargin{$\ymin$ not defined yet}
%\begin{remark}
%%\begin{enumerate}
%%\item 
%Theorem~\ref{thm:main} illustrates phase transitions of throughput for horizontal traffic queues with respect to $m$. The total service rate at any time is given by $\sum_{i=1}^{N(t)} y_i^m(t)$. If $\ymin(t)>0$, and hence $y_i(t) < 1$ for all $i \in \until{N(t)}$, then the total service rate tends to $0^+$ as $m \to + \infty$, and it tends to $N(t)$ as $m \to 0^+$. This implies that the throughput tends to $0^+$ as $m \to +\infty$, and tends to $+\infty$ as $m \to 0^+$. However, the fact that the throughput takes these extreme values at almost all values of $m$ makes Theorem~\ref{thm:main} non-trivial.
%%\end{enumerate}
%\end{remark}

%\subsection{Connections with Processor Sharing and State-dependent Queues}

==> 02- submission/service-rate-monotonicity.tex <==
\section{Service Rate Properties of the Horizontal Traffic Queue}
\label{sec:service-rate-monotonicity}
For every $y \in \mc S_N^L$, $N \in \NN$, $L>0$, we let 
$\ymin:=\min_{i \in \until{N}} y_i$, and $\ymax:=\max_{i \in \until{N}} y_i$ denote the minimum and maximum inter-vehicle distances respectively. It is easy to establish the following monotonicity properties of $\ymin$ and $\ymax$.

\begin{lemma}[Inter-vehicle Distance Monotonicity Between Jumps]
%\ksmargin{write proof of Lemma~\ref{lem:vehicle-distance-monotonicity}}
\label{lem:vehicle-distance-monotonicity}
For any  $y \in \mc S^L_N$, $N \in \NN$, $L>0$, under the dynamics in \eqref{eq:inter-vehicle-distance-dynamics}, for all $m>0$
$$
\frac{d}{dt} \ymin \geq 0 \qquad \& \qquad \qquad \frac{d}{dt} \ymax \leq 0.
$$
\end{lemma}
\begin{proof}
Let $\ymin(t) = y_j(t)$, i.e., the $j$-th vehicle has the minimum inter-vehicle distance at time $t\geq 0$.
Therefore, \eqref{eq:inter-vehicle-distance-dynamics} implies that $\dot{y}_{\min}(t) = \dot{y}_j(t)=y_{j+1}^m(t) - y_j^m(t)\geq 0$. One can similarly show that $\ymax$ is non-increasing.
\qed
\end{proof}

Due to the complex state-dependence of the departure process, the queue length process is difficult to analyze. We propose to study a related scalar quantity, called \emph{workload} formally defined as follows, where we recall the notations introduced in 
Section~\ref{sec:problem-formulation}.

\begin{definition}[Workload]
The workload associated with the HTQ at any instant is the sum of the distances remaining to be travelled by all the vehicles present at that instant. That is, if the current coordinates and departure coordinates of all vehicles are $x \in [0,L]^N$ and $q \in \RR_+^N$ respectively,  with $q \geq x$, then the workload is given by:
$$
w(x,q):= \sum_{i=1}^N (q_i-x_i).
$$   
\end{definition}


Since the maximum distance to be travelled by any vehicle from the time of arrival to the time of departure is upper bounded by $R$, we have the following simple relationship between workload and queue length at any time instant:
\be\label{eq:workload-upperbound}
w(t) \leq N(t)\, R \, , \qquad \forall \, t \geq 0 \, .
\ee
An implication of \eqref{eq:workload-upperbound} is that unbounded workload implies unbounded queue length in our setting. We shall use this relationship to establish an upper bound on the throughput. %\ksmargin{maybe include the example from slides here, \mmcomment{if this comment is not relevant anymore, please remove it.}}
However, a finite workload does not necessarily imply finite queue length. In order to see this, consider the state of the queue with $N$ vehicles, all of whom have distance $1/N$ remaining to be travelled. Therefore, the workload at this instant is $1/N \times N= 1$, which is independent of $N$. 

When the workload is positive, its rate of decrease is equal to \emph{service rate} in between jumps, defined next.

\begin{definition}[Service Rate]
When the HTQ is not idle, its instantaneous service rate is equal to the sum of the speeds of the vehicles present in the system at that time instant, i.e., $s(x)=\sum_{i=1}^N y_i^m(x)$.
\end{definition}

 %which is equal to the sum of speeds of all the vehicles, i.e., $s(x)=\sum_{i=1}^n y_i^m$. 
Since the service rate depends only on the inter-vehicle distances, we shall alternately denote it as $s(y)$. For $m=1$, $s(y)=\sum_{i=1}^N y_i \equiv L$, i.e., the service rate is independent of the state of the system, and is constant in between and during jumps. This property does not hold true in the nonlinear ($m \neq 1$) case. Nevertheless, one can prove interesting properties for the service rate dynamics. We start by deriving bounds on service rate in between jumps. 

\begin{lemma}[Bounds on Service Rates]
\label{lem:service-rate-bounds}
For any $y \in \mc S_N^L$, $N \in \NN$, $L>0$, under the dynamics in \eqref{eq:inter-vehicle-distance-dynamics},
\begin{enumerate}
\item $L^m N^{1-m} \leq s(y) \leq L^m$ if $m > 1$;
\item $L^m \leq s(y) \leq L^m N^{1-m}$ if $m \in (0,1)$.
\end{enumerate}
\end{lemma}
\begin{proof}
Normalizing the inter-vehicular distances by $L$, the service rate can be rewritten as 
\begin{equation}
\label{eq:service-rate-normalized}
s(y)=L^m \sum_{i=1}^N \left(\frac{y_i}{L}\right)^m. 
\end{equation}
Therefore, for $m > 1$, $s(y) \leq L^m \sum_{i=1}^N \frac{y_i}{L}=L^m$. One can similarly show that, for $m \in (0,1)$, $s(y) \geq L^m$. In order to prove the remaining bounds, we note that $\sum_{i=1}^N z_i^m$ is strictly convex in $z=[z_1, \ldots, z_N]$ for $m > 1$, and that the minimum of $\sum_{i=1}^N z_i^m$ over $z \in \mc S_N$ occurs at $z= \onebf/N$, and is equal to $N^{1-m}$. Similarly, for $m \in (0,1)$, $\sum_{i=1}^N z_i^m$ is strictly concave in $z$, and its maximum over $z \in \mc S_N$ occurs at $z= \onebf/N$, and is equal to $N^{1-m}$. Combining these facts with \eqref{eq:service-rate-normalized}, and noting that $y/L \in \mc S_N$, gives the lemma.
\qed
\end{proof}

\begin{lemma}[Service Rate Monotonicity Between Jumps]
\label{lem:service-rate-dynamics-between-jumps}
For any  $y \in \mc S^L_N$, $N \in \NN$, $L>0$, under the dynamics in \eqref{eq:inter-vehicle-distance-dynamics}, 
$$
\frac{d}{dt} s(y) \leq 0 \quad \text{      if } m > 1 \qquad \& \qquad \frac{d}{dt} s(y) \geq 0\quad \text{ if } m \in (0,1) \, ,
$$
where the equality holds true if and only if $y=\frac{L}{N}\onebf$.
\end{lemma}
\begin{proof}
The time derivative of service rate is given by:
\begin{align}
\frac{d}{dt} s(y) & = \frac{d}{dt} \sum_{i=1}^N y_i^m =  m \sum_{i=1}^N y_i^{m-1} \dot{y}_i \nonumber \\ 
\label{eq:service-rate-derivative}
& =  m \sum_{i=1}^N y_i^{m-1} \left( y_{i+1}^m - y_i^m\right) 
\end{align}
where the second equality follows by \eqref{eq:inter-vehicle-distance-dynamics}. The result then follows by application of Lemma~\ref{lem:appendix-general-summation}, and by noting that $g(z)=z^m$ is a strictly increasing function for all $m>0$, and $h(z)=z^{m-1}$ is strictly decreasing if $m \in (0,1)$, and strictly increasing if $m>1$.
\qed
\end{proof}

%\begin{proof}
%Throughput this proof, we implicitly let the indices $n+1$ and $-1$ in the subscripts be equal to indices $1$ and $n$ respectively. The time derivative of service rate is given by:
%\begin{align}
%\frac{d}{dt} s(y) & = \frac{d}{dt} \sum_{i=1}^n y_i^m =  m \sum_{i=1}^n y_i^{m-1} \dot{y}_i \nonumber \\ 
%\label{eq:service-rate-derivative}
%& =  m \sum_{i=1}^n y_i^{m-1} \left( y_{i+1}^m - y_i^m\right) 
%\end{align}
%For $i \in \until{n}$, let $I_i$ be the interval with end points $y_i^m$ and $y_{i+1}^m$. 
%%Similarly, let $I_n$ be the interval with end points $y_n^m$ and $y_1^m$. 
%For $i \in \until{n}$, let $f_i(z):=\sgn{y_{i+1}^m - y_i^m} y_i^{m-1} \onebf_{I_i}(z)$. With $f(z):=\sum_{i=1}^n f_i(z)$,
% \eqref{eq:service-rate-derivative} can then be written as the following:
%\begin{equation}
%\label{eq:line-integral}
%\frac{d}{dt} s(y) = m \int_{\ymin^m}^{\ymax^m} f(z) \, dz.
%\end{equation}
%We now show that, for every $z \in [\ymin^m, \ymax^m] \setminus \{y_i^m: i \in \until{n}\}$,  $f(z)$ is non-negative if $m \in (0,1)$, and is non-positive if $m > 1$. 
%This, together with \eqref{eq:line-integral}, will then prove the lemma.
%
%It is easy to see that every such $z$ belongs to an even number of intervals in $\{I_i: \, i \in \until{n}\}$, say $I_{\ell_1}, I_{\ell_2}, \ldots$, with $\ell_1 < \ell_2 < \ldots$ (see Figure \ref{fig:intervals} for an illustration).
%We now show that $f_{\ell_1}(z) + f_{\ell_2}(z)$ is non-negative if $m \in (0,1)$, and is non-positive if $m > 1$. The same argument holds true for $f_{\ell_3}(z)+f_{\ell_4}(z), \ldots$. 
%Assume that $y_{\ell_1} \leq y_{\ell_2}$; the other case leads to the same conclusion. By definition of $f_i$'s, $f_{\ell_1}(z)=y_{\ell_1}^{m-1}$ and $f_{\ell_2}(z)=-y_{\ell_2}^{m-1}$. $y_{\ell_1} \leq y_{\ell_2}$ implies that $y_{\ell_1}^{m-1} \geq y_{\ell_2}^{m-1}$ if $m \in (0,1)$, and $y_{\ell_1}^{m-1} \leq y_{\ell_2}^{m-1}$ if $m > 1$. This then establishes the required signs of $f_{\ell_1}(z) + f_{\ell_2}(z)$ for the two regimes of $m$. 
%
%
%\begin{figure}[htb!]
% \centering
% \includegraphics[width=15.5cm]{intervals} 
%  \caption{A schematic view of (a) $f_i(z), i=\{1,2,3,4\}$ and (b) $f(z)=\sum_{i=1}^4f_i(z)$ for a $y\in\mc S_4^L$ \kscomment{($L=1?$)} with $\ymin = y_2 < y_4 < y_3 < y_1 = \ymax$ for \kscomment{$m=?$}. }
%    \label{fig:intervals}
%\end{figure}
%
%
%
%%\begin{align}
%%\frac{1}{m}\frac{d}{dt} s(y) & = \frac{1}{m}\frac{d}{dt} \sum_{i=1}^n y_i^m =  \sum_{i=1}^n y_i^{m-1} \dot{y}_i =  \sum_{i=1}^n y_i^{m-1} \left( y_{i+1}^m - y_i^m\right) \nonumber \\ 
%%& = \sum_{i=1}^n y_{i+1} y_{i+1}^{m-1} y_i^{m-1} - \sum_{i=1}^n y_i y_i^{m-1} y_i^{m-1} \nonumber \\
%%\label{eq:service-rate-derivative}
%%& = \sum_{i=1}^n y_i y_i^{m-1} y_{i-1}^{m-1} - \sum_{i=1}^n y_i y_i^{m-1} y_i^{m-1}
%%\end{align}
%\end{proof}
%We now establish relationship between the two terms in \eqref{eq:service-rate-derivative} using the following lemma.
%
%\begin{lemma}
%Given two random variables  $X$ and $Y$ with identical distribution, for any two nondecreasing functions $f,g$ such that $f(X)$ and $g(X)$
%have finite variances, one can have:
%\begin{equation}
%\label{eq:E-Hoeffding}
%{\bf E}  \left[f(X)g(Y)\right] \leq {\bf E}  \left[f(X)g(X)\right]
%\end{equation}
%\end{lemma}

The following lemma quantifies the change in service rate due to departure of a vehicle. 

\begin{lemma}[Change in Service Rate at Departures]
\label{lem:service-rate-jumps}
Consider the departure of a vehicle that changes inter-vehicle distances from $y \in \mc S_N^L$ to $y^- \in \mc S_{N-1}^L$, for some $N \in \NN \setminus \{1\}$, $L > 0$. If $y_1 \geq 0$ and $y_2 \geq 0$ denote the inter-vehicle distances behind and in front of the departing vehicle respectively, at the moment of departure, then the change in service rate due to the departure satisfies the following bounds:
\begin{enumerate}
\item if $m > 1$, then $0 \leq s(y^-) - s(y) \leq (y_1+y_2)^m \left(1-2^{1-m} \right)$;
\item if $m \in (0,1)$, then $0 \leq s(y) - s(y^-) \leq \min\{y_1^m,y_2^m\}$.
\end{enumerate}
%\begin{enumerate}
%\item if $m > 1$, then $s(y^+) - s(y) \leq 0 \, ,  \qquad s(y^-) - s(y) \geq 0$
%\item if $m \in (0,1)$, then:
%$$
%s(y^+) - s(y) \geq 0 \, , \qquad 0 \leq s(y) - s(y^-) \leq \min\{y_1^m,y_2^m\}
%$$
%\end{enumerate}
\end{lemma}
\begin{proof}
%Let us first consider the change in service rates due to new arrival.  Therefore, $s(y^+)-s(y) = y_1^m + y_2^m - (y_1 + y_2)^m$.  
If $m>1$, then $\left(\frac{y_1}{y_1+y_2}\right)^m + \left(\frac{y_2}{y_1+y_2}\right)^m \leq \frac{y_1}{y_1+y_2} + \frac{y_2}{y_1+y_2} = 1$, i.e., $s(y^-)-s(y) = (y_1 + y_2)^m - y_1^m - y_2^m \geq 0$. One can similarly show that $s(y)-s(y^-) \geq 0$ if $m \in (0,1)$.

In order to show the upper bound on $s(y^-)-s(y)$ for $m>1$, we note that the minimum value of $z^m + (1-z)^m$ over $z \in [0,1]$ for $m > 1$ is $2^{1-m}$, and it occurs at $z=1/2$. Therefore, 
\begin{align*}
s(y^-)-s(y) = (y_1 + y_2)^m - y_1^m - y_2^m & = (y_1 + y_2)^m \left(1 - \left(\frac{y_1}{y_1+y_2}\right)^m - \left(\frac{y_2}{y_1+y_2}\right)^m \right) \\
& \leq (y_1+y_2)^m \left(1-2^{1-m} \right)
\end{align*}

The upper bound on $s(y)-s(y^-)$ for $m \in (0,1)$ can be proven as follows. Since $y_1^m \leq (y_1 + y_2)^m$, $s(y) - s(y^-) = y_1^m + y_2 ^m - (y_1 + y_2)^m \leq y_2^m$.  
Similarly, $s(y)-s(y^-) \leq y_1^m$. Combining, we get $s(y)-s(y^-) \leq \min \{y_1^m, y_2^m\}$. Note that, in proving this, we nowhere used the fact that $m \in (0,1)$. However, this bound is useful only for $m \in (0,1)$. 
\qed
\end{proof}

\begin{remark}[Change in Service Rate at Arrivals]
\label{rem:service-rate-jump-arrival}
The bounds derived in Lemma~\ref{lem:service-rate-jumps} can be trivially used to prove the following bounds for change in service rate at arrivals:
\begin{enumerate}
\item if $m > 1$, then $0 \leq s(y) - s(y^+) \leq (y_1+y_2)^m \left(1-2^{1-m} \right)$;
\item if $m \in (0,1)$, then $0 \leq s(y^+) - s(y) \leq \min\{y_1^m,y_2^m\}$,
\end{enumerate}
where $y_1$ and $y_2$ are the inter-vehicle distances behind and in front of the arriving vehicle respectively, at the moment of arrival.
\end{remark}

%\ksmargin{Is Lemma~\ref{lem:service-rate-bounds} true for $L \neq 1$ ?}

The following lemma will facilitate generalization of Lemma~\ref{lem:service-rate-dynamics-between-jumps}. In preparation for the lemma, let $f(y,m):=m \sum_{i=1}^N y_i^{m-1} \left( y_{i+1}^m - y_i^m\right)$ be the time derivative of service rate, as given in \eqref{eq:service-rate-derivative}.

\begin{lemma}
\label{lem:service-rate-dot-lower-bound}
For all $y \in \text{int}(\mc S_N^L)$, $N \in \NN \setminus \{1\}$, $L > 0$:
\begin{equation}
\label{eq:service-rate-der-m}
\frac{\partial}{\partial m} f(y,m)|_{m=1} = - L D\left(\frac{y}{L} || P^- \frac{y}{L}\right) \leq 0
\end{equation}
Additionally, if $L < e^{-2}$, then
\begin{equation}
\label{eq:service-rate-twice-der-m}
\frac{\partial^2}{\partial m^2} f(y,m)|_{m=1} \geq 0
\end{equation}
Moreover, equality holds true in \eqref{eq:service-rate-der-m} and \eqref{eq:service-rate-twice-der-m} if and only if $y = \frac{L}{N}\onebf$.
\end{lemma}
\begin{proof}
%\ksmargin{need to exclude from the proof all $y$ such that $y_i=0$ for some $i \in \until{n}$}
Taking the partial derivative of $f(y,m)$ with respect to $m$, we get that 
\begin{align*}
\frac{\partial}{\partial m} f(y,m) & = \frac{f(y,m)}{m} + m \sum_{i=1}^N \left( y_i^{m-1} y_{i+1}^m \left(\log y_i + \log y_{i+1} \right) - 2 y_i^{2m-1} \log y_{i} \right)
\end{align*}
In particular, for $m=1$: 
\begin{align*}
\frac{\partial}{\partial m} f(y,m) |_{m=1} & = f(y,1) + \sum_{i=1}^N \left(y_{i+1} \left(\log y_i + \log y_{i+1} \right) - 2 y_i \log y_i \right) \\
& = L \sum_{i=1}^N \frac{y_i}{L} \log \left(\frac{y_{i-1}/L}{y_i/L} \right) \\
& = - L D\left(\frac{y}{L} || P^- \frac{y}{L}\right)
\end{align*}
where, for the second equality, we used the trivial fact that $f(y,1)=0$. 
Taking second partial derivative of $f(y,m)$ w.r.t. $m$ gives:
\begin{align*}
\frac{\partial^2}{\partial m^2} f(y,m) = & \sum_{i=1}^N  y_i^{m-1}\log y_i  \left(y_{i+1}^m - y_i^m \right) + \sum_{i=1}^N y_i^{m-1} \left(y_{i+1}^m \log y_{i+1} - y_i^m \log y_i \right)\\
& + \sum_{i=1}^N \left( y_i^{m-1} y_{i+1}^m \left(\log y_i + \log y_{i+1} \right) - 2 y_i^{2m-1} \log y_{i} \right) \\
& + m \sum_{i=1}^N \left( y_i^{m-1} y_{i+1}^m \left(\log y_i + \log y_{i+1} \right)^2  - 4 y_i^{2m-1} \log^2 y_i \right)
\end{align*}
In particular, for $m=1$:
\begin{align}
\frac{\partial^2}{\partial m^2} f(y,m) |_{m=1} = & \sum_{i=1}^N \left(y_{i+1} - y_i \right) \log y_i + \sum_{i=1}^N \left(y_{i+1} \log y_{i+1} - y_i \log y_i \right) \nonumber \\
& + \sum_{i=1}^N \left(y_{i+1} \left(\log y_i + \log y_{i+1} \right) - 2 y_i \log y_i \right) \nonumber \\
& + \sum_{i=1}^N \left( y_{i+1} (\log y_i + \log y_{i+1})^2 - 4 y_i \log^2 y_i\right) \nonumber \\
\label{eq:second-derivative-m-final-eq}
= &  \sum_{i=1}^N \log^2 y_i \left(y_{i+1} - y_i \right) + 2 \sum_{i=1}^N \log y_i \left(y_{i+1} \log y_{i+1} + y_{i+1} - y_i \log y_i - y_i \right)  \\
%= &  \sum_{i=1}^n \log^2 y_i \left(y_{i+1} - y_i \right) + 2 \sum_{i=1}^n y_i \left(1 + \log y_i \right)\\
\nonumber
\geq & \, 0
\end{align}
It is easy to check that, $\log z$, $\log^2 z$ and $z + z \log z$ are strictly increasing, strictly decreasing and strictly decreasing functions, respectively, for $z \in (0,e^{-2})$. Therefore, Lemma~\ref{lem:appendix-general-summation} implies that each of the two terms in \eqref{eq:second-derivative-m-final-eq} is non-negative, and hence the lemma.
%\begin{align*}
%\frac{\partial^2}{\partial m^2} g(y,m) |_{m=1} & = - 2 D(y || P^- y) + \sum_{i=1}^n \left(y_{i+1} \left(\log y_i + \log y_{i+1} \right)^2 - 4 y_i \log^2 y_i \right) \\
%& = - 2 D(y || P^- y) + \sum_{i=1}^n y_i  \left(\log^2 y_{i-1} - \log^2 y_i \right) + 2 \sum_{i=1}^n y_i \log y_i \log \left( \frac{y_{i-1}}{y_i}\right) \\
%& = - 2 D(y || P^- y) + \sum_{i=1}^n y_i \log\left(\frac{y_{i-1}}{y_i} \right) \log (y_{i-1} y_i) + 2 \sum_{i=1}^n y_i \log y_i \log \left( \frac{y_{i-1}}{y_i}\right)
%\end{align*}
\qed
\end{proof}

\iffalse

\begin{lemma}
\label{lem:service-rate-dot-lower-bound}
For all $y \in \mc S_n^L$, $n \in \NN \setminus \{1\}$, $L > 0$:
\begin{equation}
\label{eq:service-rate-der-m}
\frac{\partial}{\partial m} f(y,m)|_{m=1} = - L D\left(\frac{y}{L} || P^- \frac{y}{L}\right) \leq 0
\end{equation}
Additionally, if $L < e^{-2}$, then
\begin{equation}
\label{eq:service-rate-twice-der-m}
\frac{\partial^2}{\partial m^2} f(y,m)|_{m=1} \geq 0
\end{equation}
Moreover, equality holds true in \eqref{eq:service-rate-der-m} and \eqref{eq:service-rate-twice-der-m} if and only if $y = \frac{L}{n}\onebf$.
\end{lemma}
\begin{proof}
\ksmargin{need to exclude from the proof all $y$ such that $y_i=0$ for some $i \in \until{n}$}
Taking the partial derivative of $f(y,m)$ with respect to $m$, we get that 
\begin{align*}
\frac{\partial}{\partial m} f(y,m) & = \frac{f(y,m)}{m} + m \sum_{i=1}^n \left( y_i^{m-1} y_{i+1}^m \left(\log y_i + \log y_{i+1} \right) - 2 y_i^{2m-1} \log y_{i} \right)
\end{align*}
In particular, for $m=1$: 
\begin{align*}
\frac{\partial}{\partial m} f(y,m) |_{m=1} & = f(y,1) + \sum_{i=1}^n \left(y_{i+1} \left(\log y_i + \log y_{i+1} \right) - 2 y_i \log y_i \right) \\
& = L \sum_{i=1}^n \frac{y_i}{L} \log \left(\frac{y_{i-1}/L}{y_i/L} \right) \\
& = - L D\left(\frac{y}{L} || P^- \frac{y}{L}\right)
\end{align*}
where, for the second equality, we used the trivial fact that $f(y,1)=0$. 
Taking second partial derivative of $f(y,m)$ w.r.t. $m$ gives:
\begin{align*}
\frac{\partial^2}{\partial m^2} f(y,m) = & \sum_{i=1}^n  y_i^{m-1}\log y_i  \left(y_{i+1}^m - y_i^m \right) + \sum_{i=1}^n y_i^{m-1} \left(y_{i+1}^m \log y_{i+1} - y_i^m \log y_i \right)\\
& + \sum_{i=1}^n \left( y_i^{m-1} y_{i+1}^m \left(\log y_i + \log y_{i+1} \right) - 2 y_i^{2m-1} \log y_{i} \right) \\
& + m \sum_{i=1}^n \left( y_i^{m-1} y_{i+1}^m \left(\log y_i + \log y_{i+1} \right)^2  - 4 y_i^{2m-1} \log^2 y_i \right)
\end{align*}
In particular, for $m=1$:
\begin{align}
\frac{\partial^2}{\partial m^2} f(y,m) |_{m=1} = & \sum_{i=1}^n \left(y_{i+1} - y_i \right) \log y_i + \sum_{i=1}^n \left(y_{i+1} \log y_{i+1} - y_i \log y_i \right) \nonumber \\
& + \sum_{i=1}^n \left(y_{i+1} \left(\log y_i + \log y_{i+1} \right) - 2 y_i \log y_i \right) \nonumber \\
& + \sum_{i=1}^n \left( y_{i+1} (\log y_i + \log y_{i+1})^2 - 4 y_i \log^2 y_i\right) \nonumber \\
\label{eq:second-derivative-m-final-eq}
= &  \sum_{i=1}^n \log^2 y_i \left(y_{i+1} - y_i \right) + 2 \sum_{i=1}^n \log y_i \left(y_{i+1} \log y_{i+1} + y_{i+1} - y_i \log y_i - y_i \right)  \\
%= &  \sum_{i=1}^n \log^2 y_i \left(y_{i+1} - y_i \right) + 2 \sum_{i=1}^n y_i \left(1 + \log y_i \right)\\
\nonumber
\geq & \, 0
\end{align}
It is easy to check that, $\log z$, $\log^2 z$, and $z + z \log z$ are strictly increasing, strictly decreasing and strictly decreasing functions, respectively, for $z \in (0,e^{-2})$. Therefore, Lemma~\ref{lem:appendix-general-summation} implies that each of the two terms in \eqref{eq:second-derivative-m-final-eq} is non-negative, and hence the lemma.
%\begin{align*}
%\frac{\partial^2}{\partial m^2} g(y,m) |_{m=1} & = - 2 D(y || P^- y) + \sum_{i=1}^n \left(y_{i+1} \left(\log y_i + \log y_{i+1} \right)^2 - 4 y_i \log^2 y_i \right) \\
%& = - 2 D(y || P^- y) + \sum_{i=1}^n y_i  \left(\log^2 y_{i-1} - \log^2 y_i \right) + 2 \sum_{i=1}^n y_i \log y_i \log \left( \frac{y_{i-1}}{y_i}\right) \\
%& = - 2 D(y || P^- y) + \sum_{i=1}^n y_i \log\left(\frac{y_{i-1}}{y_i} \right) \log (y_{i-1} y_i) + 2 \sum_{i=1}^n y_i \log y_i \log \left( \frac{y_{i-1}}{y_i}\right)
%\end{align*}
\end{proof}

\fi

Lemma~\ref{lem:service-rate-dot-lower-bound} implies that, for sufficiently small $L$, $f(y,m)$ is locally convex in $m$. One can use this property along with an exact expression for $\frac{\partial}{\partial m}f(y,m)$ in Lemma~\ref{lem:service-rate-dot-lower-bound} at $m=1$, and the fact that $f(y,1)=0$ for all $y$, to develop a linear approximation in $m$ of $f(y,m)$ around $m=1$. The following lemma derives this approximation, as also suggested by Figure~\ref{fig:service-rate-dot-vs-m}.

\begin{figure}[htb!]
 \centering
 \includegraphics[width=5cm]{service-rate-dot-vs-m} 
  \caption{$f(y,m)$ vs. $m$ for a typical $y \in \mc S_{10}$.}
    \label{fig:service-rate-dot-vs-m}
\end{figure}

%\ksmargin{the proof of Lemma~\ref{lem:service-rate-dot-deltay-bound} appears incomplete}
\begin{lemma}
\label{lem:service-rate-dot-deltay-bound}
For a given $y \in \text{int}(\mc S_N^L)$, $n \in \NN$, $L \in (0,e^{-2})$, there exists $\underbar{m}(y) \in [0,1)$ such that 
$$
\frac{d}{dt} s(y) \geq 2 \frac{(1-m)}{L} \left(\ymax - \ymin \right)^2 \, , \qquad \forall \, m \in [\underbar{m}(y),1]
$$
%$$
%\frac{d}{dt} s(y) \leq 2 (1-m) \left(\ymax - \ymin \right)^2
%$$
%$$
%\frac{d}{dt} s(y) \geq (1-m) D(y || P^- y) \geq 2 (1-m) \left(\ymax - \ymin \right)^2 \, , \qquad \forall \, m \in [\underbar{m}(y),\bar{m}(y)]
%$$
\end{lemma}
\begin{proof}
For a given $y \in \text{int}(\mc S_N^L)$, the local convexity of $f(y,m):=\frac{d}{dt} s(y)$ in $m$, and the expression of $\frac{\partial}{\partial m}f(y,m)$ at $m=1$ in Lemma~\ref{lem:service-rate-dot-lower-bound}  implies that $\frac{d}{dt} s(y) \geq (1-m) L D\left(\frac{y}{L} || P^-\frac{y}{L} \right)$ for sufficiently small $m<1$. Pinsker's inequality implies $D\left(\frac{y}{L} || P^-\frac{y}{L} \right) \geq \frac{\|y-P^-y\|_1^2}{2 L^2}$. This, combined with the fact that $\|y-P^-y\|_1 \geq 2(\ymax-\ymin)$ for all $y \in \text{int}(\mc S_N^L)$, gives the lemma.
\qed
\end{proof}

%\begin{remark}
%
%\end{remark}


==> 02- submission/simulations.tex <==
\section{Simulations}
\label{sec:simulations}
In this section, we present simulation results on throughput analysis, and compare with our theoretical results from previous sections. 
 
 
%\kscomment{(Legend of Figure~\ref{fig:m-1.5-M} to be changed: Theoretical Value $\to$ Lower Bound from \eqref{eq:sublinear-throughput-zero-initial-condition}; Lower bound $\to$ Lower Range of Numerical Estimate; Upper bound $\to$ Upper Range of Numerical Estimate)} 

 %\begin{figure}[htb!]
%\begin{center}
%\includegraphics[width=5cm]{lambda-M-m15-journal} 
%\caption{Comparison between theoretical lower bound on throughput given by \eqref{eq:sublinear-throughput-zero-initial-condition} for different values of $M$, 
%and the range of estimates obtained from simulations. The parameters used for this case are: $m = 1.5$, $L = 1$, $\delta = 0.1$, $\varphi = \delta_0$,  $\psi = \delta_L$, and $w_0=0$.}
%\label{fig:m-1.5-M}
%\end{center}
%\end{figure} 

 
%Figure~\ref{fig:m-1.5-M} concerns throughput computation for the super-linear case. In particular, it illustrates the dependence of the right hand side of \eqref{eq:sublinear-throughput-zero-initial-condition} on $M$, and hence the need to optimize over $M$ to get the best lower bound for throughput. This theoretical lower bound is also compared with the range of numerical estimates obtained from simulations. 

%We first study the lower bound on throughput for super-linear case for two different cases: empty (Theorem \ref{thm:superlinear-bound-empty}) and non-empty (Theorem \ref{thm:superlinear-bound-non-empty}) initial condition.
% 
%  Figure \ref{fig:m-1.5-M} shows values of the lower bound on the throughput for different values of the upper bound on the queue length for empty initial condition. Also, the lower and upper bounds on throughput that are found through simulations are depicted. It can be seen that the theoretical lower bound never exceeds the lower bounds found through simulations. From this figure, one can find the optimal value of $M$ to find the tightest lower bound on the throughput. 
%\kscomment{(Legend of Figure~\ref{fig:lambda-m-empty} to be changed: Theoretical lower bound $\to$ Theoretical estimates from Theorems~\ref{thm:stable}, \ref{thm:superlinear-bound-empty} and \ref{thm:main-sub-linear}; Lower bound from simulation $\to$ Lower Range of Numerical Estimate; Upper bound from simulation $\to$ Upper Range of Numerical Estimate. Legend of Figure~\ref{fig:phase-transition-non-empty} to be changed similarly.)}   


\begin{figure}
\centering
\subfigure[]{\includegraphics[width=5cm]{lambda-m-lowerUpper-w-phase-transition-separated-v2}}
\centering
\hspace{0.3in}
\subfigure[]{\includegraphics[width=5cm]{lambda-m-lowerUpper-uniform-w-phase-transition-separated-v2}}
\caption{Comparison between theoretical estimates of throughput from Theorem~\ref{thm:superlinear-bound-empty}, and range of numerical estimates from simulations, for zero initial condition. The parameters used for this case are: $L = 1$, $\delta = 0.1$, and (a) $\varphi = \delta_0$, $\psi = \delta_L$, (b)  $\varphi = U_{[0,L]}$, $\psi=U_{[0,L]}$.
 \label{fig:lambda-m-empty}}
\end{figure}

 \begin{figure}[htb!]
\begin{center}
\includegraphics[width=5cm]{lambda-m-busy-period-L100-v2} 
\caption{Comparison between theoretical estimates of throughput from Theorem  \ref{thm:superlinear-bound-empty}, and range of numerical estimates from simulations, for zero initial condition. The parameters used for this case are: $L = 100$, $\delta = 0.1$, $T=10$, and $\varphi = \delta_0$, $\psi = \delta_L$.}
\label{fig:superlinear-large-L}
\end{center}
\end{figure} 

 \begin{figure}[htb!]
\begin{center}
\includegraphics[width=5cm]{phase-transition-non-empty-separated-v2} 
\caption{Comparison between theoretical estimates of throughput from Theorem~\ref{thm:superlinear-bound-non-empty}, and range of numerical estimates from simulations.  The parameters used for this case are: $L = 1$, $\delta = 0.1$, $\varphi = \delta_0$,  $\psi = \delta_L$, $w_0=1$ and $n_0=4$, $x_1(0) =0.6, x_2(0) =0.7, x_3(0) =0.8, x_4(0) =0.9$.}
\label{fig:phase-transition-non-empty}
\end{center}
\end{figure}




%\ksmargin{Need to derive a theoretical expression for the blue solid line in Figure~\ref{fig:release-policy-vs-thm2}}
% \begin{figure}[htb!]
%\begin{center}
%\includegraphics[width=5cm]{batch-policy-vs-busy-period-bounds} 
%\caption{Comparison between theoretical lower bounds of throughput from Theorems~\ref{thm:stable} and the ones achieved by implementing the batch release policy for super-linear case. The parameters used for this case are: $L = 1$, $\varphi = U_{[0,L]}$,  $\psi = U_{[0,L]}$.}
%\label{fig:release-policy-vs-thm2}
%\end{center}
%\end{figure}


%\ksmargin{need to include analytical estimates from Theorem~\ref{thm:main-sub-linear} in Figures~\ref{fig:lambda-m-empty} and \ref{fig:phase-transition-non-empty}}  
Figures~\ref{fig:lambda-m-empty}, \ref{fig:superlinear-large-L} and \ref{fig:phase-transition-non-empty} show comparison between the lower bound on throughput over finite time horizons, as given by Theorems~\ref{thm:superlinear-bound-empty} and \ref{thm:superlinear-bound-non-empty}, and the corresponding numerical estimates from simulations. 
%compare the theoretical estimate of lower bound on throughput, and the range of numerical estimates obtained from simulations for various values of $m>1$. Our analytical results in Theorems~\ref{thm:stable} and \ref{thm:superlinear-bound-empty} show good comparison with numerical results for $m > 1$.
%The plot shows a sharp phase transition in the numerical estimate of throughput at $m=1$.
 %\kscomment{While our analytical results in Theorems~\ref{thm:stable} and \ref{thm:superlinear-bound-empty} show good comparison with numerical results for $m \geq 1$, Theorem~\ref{thm:main-sub-linear} does not necessarily imply unbounded throughput for all $m \in (0,1)$.} 
 Figures~\ref{fig:lambda-m-empty} and \ref{fig:superlinear-large-L} are for zero initial condition, and Figure~\ref{fig:phase-transition-non-empty} is for non-zero initial condition.

Figures~\ref{fig:sublinear-lowerbound} and \ref{fig:superlinear-batch} show comparison between the lower bound on throughput as given by the bacth release control policy, as per Theorems~\ref{thm:main-sub-linear} and \ref{thm:main-batch-super-linear}, respectively, under a couple of representative values of maximum permissible perturbation $\eta$. In particular, Figure~\ref{fig:sublinear-lowerbound} demonstrates that the lower bound achieved from Theorem \ref{thm:main-sub-linear} increases drastically as $m \to 0^+$. Both the figures also confirm that the throughput indeed increases with increasing maximum permissible perturbation $\eta$.

%Figure \ref{fig:superlinear-batch} depicts the theoretical estimates of the lower bound on throughput for super-linear case when batch release control policy with various maximum permissible perturbation is implemented. 
It is instructive to compare Figures~\ref{fig:lambda-m-empty}(b) and \ref{fig:superlinear-batch}(a), both of which depict throughput estimates for the sub-linear case, however obtained from different methods, namely busy period distribution and batch release control policy. Accordingly, one should bear in mind that the two bounds have different qualifiers attached to them: the bound in Figure~\ref{fig:lambda-m-empty}(b) is valid probabilistically only over a finite time horizon, whereas the bound in Figure~\ref{fig:superlinear-batch}(a) is valid with probability one, although under a perturbation to the arrival process. 

%the throughput bounds for the super-linear case obtained 
%By comparing Figures \ref{fig:lambda-m-empty}-b and \ref{fig:superlinear-batch}-a, one can observe that, for the same setup, the lower bounds on throughput provided by Theorem \ref{thm:superlinear-bound-empty} is better than the ones given by Theorem \ref{thm:main-batch-super-linear}. However, Theorem \ref{thm:superlinear-bound-empty} provides probabilistic guarantees over finite horizons, whereas Theorem \ref{thm:main-batch-super-linear}, by introducing perturbations, gives guarantees with probability one over infinite horizon. This reveals the trade-off among these two results for the super-linear case. 
%\mmcomment{However, Theorem~\ref{thm:main-sub-linear} does not necessarily imply unbounded throughput for all $m \in (0,1)$.}
 \begin{figure}[htb!]
\begin{center}
\includegraphics[width=5cm]{sublinear-lowerbound} 
\caption{Theoretical estimates of throughput from Theorems~\ref{thm:main-sub-linear} for different values of $\eta$.  The parameters used for this case are: $L = 1$, $\varphi = U_{[0,L]}$,  $\psi = U_{[0,L]}$, and $w_0=0$ . Note that the vertical axis is in logarithmic scale.}
\label{fig:sublinear-lowerbound}
\end{center}
\end{figure}

%\ksmargin{what are the initial location of vehicles ?}


  
%Similar results can be generated for different values of $m>1$. Figure \ref{fig:lambda-m-empty} illustrates the ultimate results for two different $\varphi$ and different $m>1$. One can observe that our analysis provided a lower bound on the throughput achieved through the simulations. Similar results for the non-empty initial condition are reported for non-empty initial condition in Figure \ref{fig:phase-transition-non-empty}. 
%Similar plot is shown in Figure \ref{fig:lambda-m-uniform} where the main difference is the arrival process which is not deterministic and the spatial distribution is uniform i.e. $\varphi=U_{[0,1]}$.  



\begin{figure}
\centering
\subfigure[]{\includegraphics[width=5cm]{sublinear-small-L}}
\centering
\hspace{0.3in}
\subfigure[]{\includegraphics[width=5cm]{superlinear-batch-new-v2}}
\caption{Theoretical estimates of throughput from Theorem \ref{thm:main-batch-super-linear}, and numerical estimates from simulations for different  The parameters used for this case are: $\varphi=U_{[0,L]}$, $\psi=U_{[0,L]}$, and (a) $L = 1$, (b) L = 100. \label{fig:superlinear-batch}}
\end{figure}

 \begin{figure}[htb!]
\begin{center}
\includegraphics[width=5cm]{upper-bound-queue-length-linear-large-lambdas} 
\caption{Comparison between the empirical expectation of the queue length and the upper bound suggested by Remark~\ref{remark:waiting-time}. We let the simulations run up to time $t=80,000$. The parameters used for this case are: $L=1$, $m=1$, $\varphi=\delta_0$, $\psi=\delta_L$. For these values, we have $\lambdamax=1$.}
\label{fig:queue-length-linear}
\end{center}
\end{figure}  

Finally, Figure~\ref{fig:queue-length-linear} shows a good agreement between queue length bound suggested by Remark~\ref{remark:waiting-time}, and the corresponding numerical estimates in the linear case. 

%\kscomment{  
%For linear car following model, $m=1$, we derived an upper bound on the average waiting time of the vehicles in Proposition \ref{prop:upperbound-on-mean-waitingtime}. Figure \ref{fig:upper-bound-queue-length-linear} reports the results of simulations, and it can be observed that the  average waiting time obtained through simulations is upper bounded by the value that is presented in Proportion \ref{prop:upperbound-on-mean-waitingtime}. Indeed, this upper bounds seems to be a tight upper bound. 
%} 
 
%In this section, we study the performance of the estimation provided in \eqref{eq:lowerbound-on-prob-queue-length} through simulations. Figure \ref{fig:m-lambda} illustrates $\lambda(M,\delta)$ for two different values of $M$ ($M=20$ and $M=40$), $\delta=0.1$ and different values of $m$. As \eqref{eq:lowerbound-on-prob-queue-length} suggests, $\lambda(M,\delta)$ provides a lower bound for the arrival rate for which the queue length will remain less than $M$ with a probability greater than $1-\delta$. As it is expected, in Figure \ref{fig:m-lambda}, as $m$ reaches to one (i.e. linear model) this lower bound increases. 

%In Figure \ref{fig:m-prob}, we compare the lower bound provided in \eqref{eq:lowerbound-on-prob-queue-length} and with actual probabilities. In order to obtain the actual probabilities, we conduct stochastic simulation for the given $m, L=1,\varphi(x)=\delta_{\{x=1\}}$ with the arrival rate as depicted in Figure \ref{fig:m-lambda} for $M=40$. We let the system evolve for a long time (i.e. $t=3000$) and then compute the duration of time the queue length is less than or equal to $M$ and divide this quantity by the total length of simulation. This procedure gives an empirical evaluation of $\Pr(N\leq M)$ and since simulation time is considered large enough, this probability should be close to the actual value. Figure \ref{fig:m-prob2} depicts the same with the arrival rate estimated by $\delta=0.1$ and $M=10$. It can be observed that \eqref{eq:lowerbound-on-prob-queue-length} provides an appropriate lower bound for the actual probabilities.  

% \begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=9cm]{m-lambda} 
%\caption{Lower bound on the arrival rate for which the queue length remains bounded by $M$ with probability greater than $0.9$}
%\label{fig:m-lambda}
%\end{center}
%\end{figure}

 %\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=9cm]{m-prob} 
%\caption{Lower bound for the probability of $N\leq M=40$ for the $\lambda(\delta=0.1,M=40)$ computed by \eqref{eq:lowerbound-on-prob-queue-length}.}
%\label{fig:m-prob}
%\end{center}
%\end{figure}


 
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=9cm]{m-prob3} 
%\caption{Lower bound for the probability of $N\leq M=10$ for the $\lambda(\delta=0.1,M=10)$ %computed by \eqref{eq:lowerbound-on-prob-queue-length}.}
%\label{fig:m-prob2}
%\end{center}
%\end{figure}


 %\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=10cm]{m-prob4} 
%\caption{Lower bound for the probability of $N\leq M=10$ for the $\lambda(\delta=0.1,M=10)$ computed by \eqref{eq:lowerbound-on-prob-queue-length}.}
%\label{fig:m-prob2}
%\end{center}
%\end{figure}


 %\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=10cm]{lambda-M-m11} 
%\caption{}
%\label{fig:m-prob2}
%\end{center}
%\end{figure}




 %\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=7cm]{lambda-m-lowerUpper-w-phase-transition} 
%\caption{Theoretical lower bound  and the bounds on throughput obtained through simulations ($L = 1$, $\delta = 0.1$, $\varphi = \delta_L$, and $\psi = \delta_0$)}
%\label{fig:lambda-m-uniform}
%\end{center}
%\end{figure}
% \begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=7cm]{lambda-m-lowerUpper-uniform-w-phase-transition} 
%\caption{Theoretical lower bound and the bounds on throughput obtained through simulations ($L = 1$, $\delta = 0.1$, $\varphi = U_{[0,1]}$, and $\psi = \delta_0$)}
%\label{fig:lambda-m-uniform}
%\end{center}
%\end{figure}



% \begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=10cm]{lambda-M-m20} 
%\caption{}
%\label{fig:m-prob2}
%\end{center}
%\end{figure}
 %\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=10cm]{lambda-M-m2-unif} 
%\caption{}
%\label{fig:m-prob2}
%\end{center}
%\end{figure}
 %\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=10cm]{lambda-M-m15-unif} 
%\caption{}
%\label{fig:m-prob2}
%\end{center}
%\end{figure}
%\subsubsection{\mmcomment{Counter Example}}
%\begin{theorem}
%For $\psi=\delta_{\{x=L\}}$, $\varphi=\delta_{\{x=0\}}$ and any $\delta\in(0,1)$, $L>0$, $m>1$, $M\in\mathbb{N}$, there exists a $x_0$ such that 
%$$\Pr(N(t)\geq M)\geq \delta \quad \text{as} \quad   t\to \infty$$
%\end{theorem}
%\begin{proof}
%\end{proof}


==> 02- submission/sublinear-new.tex <==
\subsection{Throughput Bounds under Batch Release Control Policy}
In this section, we consider a \emph{time-perturbed} version  of the arrival process. 
For a given realization of arrival times, $\{t_1,t_2,\cdots\}$, consider a perturbation map $t_i^{\prime} \equiv t_i^{\prime}(t_1,\ldots,t_i)$ satisfying $t_i^{\prime}\geq t_i$ for all $i$, which prescribes the perturbed arrival times. The magnitude of perturbation is defined as $\eta := E\left(t_i^{\prime}-t_i\right)$, where the expectation is with respect to the Poisson process with rate $\lambda$ that generates the arrival times.

We prove boundedness of the queue length under a specific perturbation map. This perturbation map is best understood in terms of a control policy that governs the release of arrived vehicles into HTQ. In order to clarify the implementation of the control policy, we decompose the proposed HTQ into two queues in series: denoted as HTQ1 and HTQ2, both of which have the same geometric characteristics as HTQ, i.e., a circular road segment of length $L$ (see Figure \ref{fig:htq1-htq2} for illustrations). The original arrival process for HTQ, i.e. spatio-temporal Poisson process with rate $\lambda$ and spatial distribution $\varphi$ is now the arrival process for HTQ1. Vehicles remain stationary at their arrival locations in HTQ1, until released by the control policy into HTQ2. Upon released into HTQ2, vehicles travel according to \eqref{eq:dynamics-moving-coordinates} until they depart after traveling a distance that is sampled from $\psi$, as in the case of HTQ. The time of release of the vehicles into HTQ2 correspond to their perturbed arrival times $t_1^{\prime}, t_2^{\prime}, \ldots$. The average waiting time in HTQ1 under the given release control policy is then the magnitude of perturbation in the arrival times. 


%Let the HTQ be composed of two queues in series: HTQ1 and HTQ2. External arrivals happen in HTQ1 according to the spatio-temporal Poisson process with rate $\lambda$, and spatial distribution $\varphi$ into HTQ1. Upon arrival, vehicles do not move in HTQ1  
%
%which we describe in this section. 
%We consider two queues, say HTQ1 and HTQ2, in series. HTQ1 is a vertical queue, and HTQ2 is a horizontal queue, and they are constructed as follows. Arrivals happen into HTQ1 according to the prescribed spatio-temporal Poisson process, and its departure is governed by a control policy to be described shortly. Vehicles in HTQ1 do not move, but start moving according to \eqref{eq:dynamics-moving-coordinates} as soon as released into HTQ2. Vehicles depart from HTQ2 as soon as they reach their departure locations (see Figure \ref{fig:htq1-htq2} for an illustration) 


\begin{figure}[htb!]
\begin{center}
\includegraphics[width=14cm]{htq1-htq2-decomposed} 
\caption{Decomposition of HTQ into HTQ1 and HTQ2 in series.}
\label{fig:htq1-htq2}
\end{center}
\end{figure}

We consider the following class of release control policy, for which we recall from the problem setup in Section~\ref{sec:problem-formulation} that $\text{supp}(\varphi)=[0,\ell]$ for some $\ell \in [0,L]$. 

%\begin{definition}[Batch Release Control Policy $\pi^b_\triangle$]
%\label{def:batch-release-control-policy}
%Divide $[0,\ell]$ into sub-intervals, each of length $\triangle$, enumerated as $1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil$. Let $T_1$ be the first time instant when there are no vehicles in $[L-\triangle,L] \cup [0,\ell + \triangle]$. At time $T_1$, release one vehicle each, if present, from all odd-numbered sub-intervals in $\{1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil\}$ simultaneously into HTQ2. Let $T_2$ be the next time instant when there are no vehicles in $[L-\triangle,L] \cup [0,\ell + \triangle]$. At time $T_2$, release one vehicle each, if present, from all even-numbered sub-intervals in $\{1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil\}$ simultaneously into HTQ2. Repeat this process of alternating between releasing one vehicle each from odd and even-numbered sub-intervals every time that no vehicle is in $[L-\triangle,L] \cup [0,\ell + \triangle]$.
%\end{definition}

\begin{definition}[Batch Release Control Policy $\pi^b_\triangle$]
\label{def:batch-release-control-policy}
Divide $[0,\ell]$ into sub-intervals, each of length $\triangle$, enumerated as $1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil$. Let $T_1$ be the first time instant when HTQ2 is empty. At time $T_1$, release one vehicle each, if present, from all odd-numbered sub-intervals in $\{1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil\}$ simultaneously into HTQ2. Let $T_2$ be the next time instant when HTQ2 is empty. At time $T_2$, release one vehicle each, if present, from all even-numbered sub-intervals in $\{1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil\}$ simultaneously into HTQ2. Repeat this process of alternating between releasing one vehicle each from odd and even-numbered sub-intervals every time that HTQ2 is empty.
\end{definition}


%\begin{definition}[Release Control Policy $\pi_\triangle$]
%\label{def:release-control-policy}
%For $\triangle > 0$, $\pi_{\triangle}$ denotes the class of control policies under which a vehicle $i$ waiting at location $x \in [0,L]$ in HTQ1 is released to the same location in HTQ2 at time $t_i^{\prime}$ only if the distances to the nearest vehicles in front and behind of $x \in [0,L]$ is at least $\triangle$ at time $t_i^{\prime}$.
%\end{definition}

\begin{remark}
\begin{enumerate}
\item Under $\pi^b_{\triangle}$, when vehicles are released into HTQ2, the inter-vehicle distances in the front and rear of each vehicle being released is at least equal to $\triangle$. 
%Note that Definition~\ref{def:release-control-policy} does not describe a specific release mechanism.
\item The order in which vehicles are released into HTQ2 from HTQ1 under $\pi^b_{\triangle}$ may not be the same as the order of arrivals into HTQ1.
%\item Multiple vehicles could be released simultaneously from HTQ1 into HTQ2, at different locations.
\end{enumerate}
\end{remark}

In the next two sub-sections, we analyze the performance of the batch release control policy for sub-linear and super-linear cases. 
\subsubsection{The Sub-linear Case}
In this section, we derive a lower bound on throughput when $m\in(0,1)$. We first derive a trivial lower bound in Proposition \ref{prop:throughput-bound-sublinear} implied by Lemma \ref{lem:service-rate-jumps} and Remark \ref{rem:service-rate-jump-arrival}. Next, we improve this lower bound in Theorem \ref{thm:main-sub-linear} under a under a batch release control policy, $\pi_{\triangle}^b$. 
\begin{proposition}
\label{prop:throughput-bound-sublinear}
For any $L > 0$, $m\in(0,1)$, $\varphi \in \Phi$, $\psi \in \Psi$, $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$:
$$
  \lambdamax(L,m,\varphi,\psi,x_0,\delta=0) \geq L^m/\bar{\psi} 
$$
\end{proposition}
\begin{proof}
Remark \ref{rem:service-rate-jump-arrival} implies that, for $m \in (0,1)$, the service rate does not decrease due to arrivals. Therefore, a simple lower bound on the service rate for any state is the service rate when there is only one vehicle in the system, i.e., $L^m$. Therefore,  
%
%For any $m\in(0,1)$, by Remark \ref{rem:service-rate-jump-arrival}, addition of a new vehicle increases the service rate; therefore, when there is only one vehicle on the road, the minimum non-zero service rate is achieved. Thus, for all $t\geq 0$ such that $n(t)\neq 0$, 
%\be\label{eq:service-rate-upperbound-sublinear}
%s(t)\geq L^m
%\ee
the workload process is upper bounded as
%\begin{equation*}
%\label{eq:workload-sublinear}
$w(t) = w_0+r(t)-\int_0^ts(z)\de z \leq w_0+r(t) -L^m(t-\mathcal{I}(t)), \quad \forall t\geq 0$, 
%\end{equation*}
where $r(t)$ and $\mathcal{I}(t)$ denote the renewal reward and the idle time processes, respectively, as introduced in the proof of Proposition \ref{prop:unstable}. Similar to the proof of Proposition \ref{prop:unstable}, it can be shown that, if $\lambda < L^m/\bar{\psi}$, then the workload, and hence the queue length, goes to zero in finite time with probability one. 
%
% and $(x_0,n_0)$ the upper bound on the workload in \eqref{eq:workload-sublinear} goes to zero in finite time, with probability one. This implies that, for any $\lambda < L^m/\bar{\psi}$ and $(x_0,n_0)$, the queue length does not grow unbounded, with probability one. 
%Assume that for some $\lambda < L^m/\bar{\psi}$, there exists some initial condition $(x_0,n_0)$ such that the queue length grows unbounded with some positive probability. 
%Since the workload brought by every vehicle is i.i.d., and the inter-arrival times are exponential, without loss of generality, we can assume that the queue length never becomes zero. That is, the idle time satisfies $I(t) \equiv 0$. Moreover, \eqref{eq:slln-renewal} implies that, for every $\varepsilon \in \left(0, L^m- \lambda \bar{\psi} \right)$, there exists $t_0 \geq 0$ such that, with probability one,
%\begin{equation}
%\label{eq:s-t-upperbound}
%\frac{r(t)}{t} \leq \lambda \bar{\psi} + \varepsilon/2 < L^m - \varepsilon/2 \qquad \forall t \geq t_0
%\end{equation} 
%Combining \eqref{eq:workload-sublinear} with \eqref{eq:s-t-upperbound}, and substituting $I(t) \equiv 0$, we get $w(t) < w_0 - \varepsilon t /2$, which implies that workload, and hence queue length, goes to zero in finite time after $t_0$, leading to a contradiction which implies that, for any $\lambda<L^m/\bar\psi$, the queue length remains bounded. This establishes this proposition.
\qed
\end{proof}

Next, we establish better throughput guarantees than Proposition~\ref{prop:throughput-bound-sublinear},  under a batch release control policy, $\pi_{\triangle}^b$.
%  for a given realization of the arrival times $\{t_1,t_2,\cdots\}$, we consider a perturbed version $\{t_1^{\prime},t_2^{\prime},\cdots\}$ satisfying:
%\begin{equation}
%\label{eq:perturbation-properties}
%t_i^{\prime} \equiv t_i^{\prime}(t_1,\ldots,t_i), \qquad t_i^{\prime}\geq t_i, \qquad \forall \, i 
%\end{equation}
%The magnitude of perturbation is defined as follows.
%\begin{definition}[Perturbation magnitude]
%The magnitude of a perturbation map satisfying \eqref{eq:perturbation-properties} is defined as 
%$\eta := E\left(t_i^{\prime}-t_i\right)$, where the expectation is with respect to the Poisson process with rate $\lambda$ that generates the arrival times.
%%Consider a perturbation of arrival times satisfying \eqref{eq:perturbation-properties}. 
%%
%%If $\{t_i\}_{i=1}^\infty$ and $\{t_i^{\prime}\}_{i=1}^\infty$ denote the actual realizations and perturbed versions of the arrival times satisfying \eqref{eq:perturbation-properties}, then 
%%
%%denote the arrival times of a Poisson process with rate $\lambda$. A perturbed version of this process is denoted by $\{t_i^{\prime}\}_{i=1}^\infty$ and $t_i^{\prime}\geq t_i$ for all $i$. The magnitude of perturbation is 
%%\begin{equation*}
%%\eta := E\left(t_i^{\prime}-t_i\right)
%%\end{equation*}
%\end{definition}
%The following result characterizes the stability of queue for a maximum allowed perturbation, $\eta_{\max}$.
%\subsubsection{Release Control Policy}\label{sec:release-control-policy}
%Monotonicity implies that the minimum inter-vehicle distance under $\pi_{\triangle}$ is at least $\triangle$.
 %It is easy to see that this policy belongs to $\pi_{\triangle}$. 
The next result characterizes the time interval between release of successive batches into HTQ2 under $\pi_\triangle^b$.

\begin{lemma}
\label{eq:successive-release-time-difference}
For given $\lambda>0$, $\triangle > 0$, $\varphi \in \Phi$, $\psi \in \Psi$ with $\supp(\psi)=[0,R]$, $R>0$, $m\in(0,1)$, $x_0\in[0,L]^{n_0}$, $L>0$, $n_0\in \mathbb{N}$, let $T_1$, $T_2$, $\ldots$ denote the random variables corresponding to time of successive batch releases into HTQ2 under $\pi_{\triangle}^b$. Then, $T_1 \leq \frac{n_0R}{L^m}$, $T_{i+1}-T_i \leq R/\triangle^m$ for all $i \geq 1$, and $\ymin(t) \geq \triangle$ for all $t \geq T_1$.
\end{lemma}
%\begin{lemma}
%\label{lem:T1-finite}
%%For any $L>0$, $\triangle > 0$, $m\in(0,1)$, $n_0\in \mathbb{N}$, and $x_0\in[0,L]^{n_0}$, $T_1$ is upper bounded as:
%%\begin{equation}
%%T_1\leq \frac{n_0R}{L^m}
%%\end{equation}
%For any $L>0$, $\triangle > 0$, $m\in(0,1)$, $x_0\in[0,L]^{n_0}$, $n_0\in \mathbb{N}$, we have $T_1\leq \frac{n_0R}{L^m}$.
%\end{lemma}
\begin{proof}
%We compute an upper bound on the time it takes for the system, starting from a non-zero initial condition with no new arrivals, to become idle. This, obviously, would be also an upper bound on $T_1$. 
Since the maximum distance to be traveled by every vehicle is upper bounded by $R$, the initial workload satisfies $w_0\leq n_0R$.  Since the minimum service rate for $m \in (0,1)$ is $L^m$ (see proof of Proposition~\ref{prop:throughput-bound-sublinear}), with no new arrivals, it takes at most $w_0/L^m=n_0 R/L^m$ amount of time for the system to become empty. This establishes the bound on $T_1$. 

Lemma~\ref{lem:vehicle-distance-monotonicity} implies that, under $\pi^b_{\triangle}$, the minimum inter-vehicle distance in HTQ2 is at least $\triangle$ after $T_1$. 
This implies that $\ymin(t) \geq \triangle$ for all $t \geq T_1$, and hence the minimum speed of every vehicle in HTQ2 is at least $\triangle^m$ after $T_1$. Since the maximum distance to be traveled by every vehicle is $R$, this implies that the time between release of a vehicle into HTQ2 and its departure is upper bounded by $R/\triangle^m$, which in turn is also an upper bound on the time required by all the vehicles released in one batch to depart from the system. 
%Therefore, the time difference between successive release from a typical sub-queue in HTQ1 during busy period is upper bounded by $2 R/\triangle^m$.
\qed
\end{proof}
%Lemma~\ref{eq:successive-release-time-difference} implies that, for a finite initial queue length, $T_1$ is also finite. 
%The conservative policy $\tilde{\pi}_\triangle$ is described as follows. 
Let $N_1(t)$ and $N_2(t)$ denote the queue lengths in HTQ1 and HTQ2, respectively, at time $t$. Lemma~\ref{eq:successive-release-time-difference} implies that, for every $\triangle>0$, $N_2(t)$ is upper bounded for all $t \geq T_1$. The next result identifies conditions under which $N_1(t)$ is upper bounded. 

%We wish to show that $N_1(t) + N_2(t)$ is bounded. 
%The following lemma implies that it is sufficient to show that $N_1(t)$ is bounded. 

%\ksmargin{finish the proof of Lemma~\ref{lem:HTQ2-upper-bound}}
%\begin{lemma}
%\label{lem:HTQ2-upper-bound}
%For every $\triangle > 0$, under control policy $\pi_{\triangle}$ and the car following behavior in \eqref{eq:dynamics-moving-coordinates} for any $m>0$, 
%$\ymin(t) \geq \triangle$, and hence $N_2(t) \leq L/\triangle$ for all $t \geq T_1$.
%\end{lemma}
%\begin{proof}
%Under $\pi_{\triangle}$, $\ymin(t)\geq \triangle$ for all $t \geq T_1$. This implies that, under this policy, at most $L/\triangle$ can be fitted in HTQ2. This establishes this lemma. 
%\end{proof}
%\ksmargin{need to think about the `for all' part}

%Release vehicles into HTQ2 as per the following iterations, starting from the first time instant when there is no vehicle in $\left[0,\min\{\ell+\triangle,L\}\right]$. 
%Release vehicles simultaneously from all odd segments, which ensures that $\ymin \geq \triangle$ at the time of release. Release vehicles from even segments the next time instant when no vehicle is in $[0,\ell+\triangle]$ in HTQ2, and so on. 

%\ksmargin{the load factor computation is only for $t \geq T_1$}
For $F>0$, let $\Phi_F:=\setdef{\varphi \in \Phi}{\sup_{x \in [0,\ell]} \varphi(x) \leq F}$. For subsequent analysis, we now derive an upper bound on the \emph{load factor}, i.e., the ratio of the arrival and departure rates, associated with a typical sub-queue of HTQ1 among  $\{1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil\}$. It is easy to see that, for every $\varphi \in \Phi_F$, $F>0$, the arrival process into every sub-queue is Poisson with arrival rate upper bounded by $\lambda F \triangle$.  Lemma~\ref{eq:successive-release-time-difference} implies that the departure rate is at least $\triangle^m/2R$. Therefore, the load factor for every sub-queue is upper bounded as 
\begin{equation}
\label{eq:load-factor-upper-bound}
\rho \leq \frac{2 R \lambda F \triangle}{\triangle^m}=2 R \lambda F \triangle^{1-m}
\end{equation}
In particular, if 
\be\label{eq:triangle-star}
\triangle < \triangle^*(\lambda):=\left(2 R \lambda F \right)^{-\frac{1}{1-m}},
\ee 
then $\rho<1$. It should be noted that for $n_0<+\infty$, by Lemma \ref{eq:successive-release-time-difference},  $T_1<+\infty$. The service rate is zero during $[0,T_1]$; however, since $T_1$ is finite, this does not affect the computation of load factor. 

%\begin{equation*}
%\Phi_F:=\setdef{\varphi \in \Phi}{\sup_{x \in [0,L]} \varphi(x) \leq F}.
%\end{equation*}

%\ksmargin{the effect of $T_1$ is not yet included in Proposition~\ref{prop:pi1-policy} -- this is also related to the initial condition}
\begin{proposition}
\label{prop:pi1-policy}
For any $\lambda>0$, $\varphi \in \Phi_F$, $F>0$, $\psi \in \Psi$ with $\supp(\psi)=[0,R]$, $R>0$, $m\in(0,1)$, $x_0\in[0,L]^{n_0}$, $L>0$, $n_0\in \mathbb{N}$, for sufficiently small $\triangle$, $N_1(t)$ is bounded for all $t \geq 0$ under $\pi_{\triangle}^b$, almost surely.
\end{proposition}
\begin{proof}
By contradiction, assume that $N_1(t)$ grows unbounded. This implies that there exists at least one sub-queue, say $ j \in \{1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil\}$, such that its queue length, say $N_{1,j}(t)$, grows unbounded. In particular, this implies that there exists $t_0 \geq T_1$ such that $N_{1,j}(t) \geq 2$ for all $t \geq t_0$. Therefore, for all $t \geq t_0$, the ratio of arrival rate to departure rate for the $j$-th sub-queue is given by \eqref{eq:load-factor-upper-bound}, which is a decreasing function of $\triangle$, and hence becomes strictly less than one for sufficiently small $\triangle$. A simple application of the law of large numbers then implies that, almost surely, $N_{1,j}(t)=0$ for some finite time, leading to a contradiction.
%Therefore, a vehicle departs from the $j$-th sub-queue every alternate time instant when there is no vehicle in $[L-\triangle,L] \cup [0,\ell + \triangle]$. We now compute an upper bound on the time difference between two such time instants. 
%
%Under any policy in $\pi_{\triangle}$, Lemma~\ref{lem:HTQ2-upper-bound} implies that the speed of every vehicle in HTQ2 is at least $\triangle^m$. Since the support of distribution for travel distances is $[0,R]$, this implies that the time between release of a vehicle into HTQ2 and its departure is upper bounded by $R/\triangle^m$, which in turn is also an upper bound on the time required by all vehicles released in one batch to depart from the system. Therefore, the time difference between successive release from the $j$-th sub-interval is upper bounded by $2 R/\triangle^m$. In other words, the departure rate from the $j$-th sub-interval is at least $\triangle^m/2R$ after $t_0$. The arrival process in the $j$-th sub-interval is Poisson with rate upper bounded by $\lambda \triangle F$. The ratio of the arrival rate to the departure rate for the $j$-th sub-interval is $\frac{2 R \lambda F \triangle}{\triangle^m}=2 R \lambda F \triangle^{1-m}$, which is a decreasing function of $\triangle$, and hence becomes strictly less than one for sufficiently small $\triangle$. A simple application of the law of large numbers then implies that, almost surely, $N_{1,j}(t)=0$ for some finite time, leading to a contradiction.
%
%
%exists at least one segment, say $j$-th, in HTQ1 that will be non-empty for all $t\geq t_0$ for some $t_0\geq 0$. Therefore, under $\tilde{\pi}_{\triangle}$, for all $t\geq t_0$, at every instant of vehicle release one vehicle gets released form $j$-th segment. This implies that, for all $t\geq t_0$, the departure rate of $j$-th segment is $\triangle^m/2R$. The ratio of the arrival rate to the departure rate for this segment is 
%\begin{equation}\label{eq:arrival-service-ratio}
%\rho_j:=\frac{\lambda_j}{\triangle^m/2R}=\frac{\lambda k_j \triangle/\ell}{\triangle^m/2R}\leq \frac{\lambda F \triangle/\ell}{\triangle^m/2R} < 1
%\end{equation}
%where the second inequality follows by \eqref{eq:varphi-condition}. This implies that the arrival rate at any segment that the number of vehicles in it is growing unbounded is strictly less than the departure rate. By law of large number arguments, this leads to a contradiction and queue length at any segment cannot grow unbounded and consequently $N_1(t)$ remains bounded. This establishes this proposition.
\qed 
\end{proof}

%Lemma~\ref{lem:HTQ2-upper-bound} and Proposition~\ref{prop:pi1-policy} together give the main result on the throughput analysis in the sub-linear case. 



%Note that the speed of every vehicle is at least $\triangle^m$ and the maximum distance that a vehicle wishes to travel upon arrival is upper bounded by $R$. If every sub-interval is non-empty at every time instant of vehicle release, then the time difference between successive instants of vehicle release (during a busy period) from each segment, is at most $2R/\triangle^m$.

%\begin{remark}
%$\tilde{\pi}_\triangle$ is conservative in the sense that it assumes that every sub-interval is non-empty at every instant of vehicle release. Nevertheless, the implementation of $\tilde{\pi}_\triangle$ will imply the desired bound on minimum inter-vehicle distances i.e. $y_{\min}\geq \triangle$.
%\end{remark}

%Let $u_i, i=1,\cdots,\ell/\triangle$ denote the beginning point of the $i$-th segment. Then, $p_i=\int_{u_i}^{u_{i+1}}\varphi(s)\de s$ represents the probability of falling a vehicle into $i$-th segment. Note that, for uniform distribution, this probability is equal to $\triangle/\ell$ for all $i$. For a general $\varphi$, however, we can write
%\begin{equation*}
%p_i = k_i \triangle/\ell =\int_{u_i}^{u_{i+1}}\varphi(z)\de z\leq \sup_{z\in[0,\ell]}\varphi(z)\triangle, \quad 0\leq k_i\leq F \quad \forall i
%\end{equation*}
%This implies that 
%\be\label{eq:varphi-condition}
%k_i \leq F:= \ell  \sup_{z\in[0,\ell]}\varphi(z), \quad \forall i\in\{1,2,\cdots,\ell/\triangle\}
%\ee
%Therefore, the arrival rate of $i$-th segment can be denoted as $\lambda_i=\lambda p_i = \lambda k_i\triangle/\ell$. 
%The next result quantifies the departure process from each segment under $\tilde{\pi}_\triangle$.

%\begin{lemma}
%\label{lem:htq1-departure-general}
%The departure rate from $i$-th segment, under $\tilde{\pi}_\triangle$, is equal to $\min{\{\lambda_i, \triangle^m/2R\}}$. 
%\end{lemma}
%\begin{proof}
%Implementation of $\tilde{\pi}_\triangle$ implies that that the departure rate from each segment can be at most $\triangle^m/2R$. Therefore, when the arrival rate for each segment is smaller than the maximum possible departure rate, the departure rate equals the arrival rate. Otherwise, the departure rate is restricted to the maximum value i.e. $\triangle^m/2R$. This establishes this lemma.
%\end{proof}

%Let $N_1(t)$ and $N_2(t)$ be the queue lengths of HTQ1 and HTQ2, respectively, at time $t$. Under policy $\tilde{\pi}_{\triangle}$, we have $N_2(t) \leq L/\triangle < +\infty$ for all $t \geq 0$. Therefore, in order to prove stability, it is sufficient to show that $N_1(t)$ remains bounded at all times. 

%\begin{proposition}
%\label{prop:pi1-policy}
% For all $\lambda> 0$, $\triangle< \left(\frac{ 2FR \lambda}{\ell}\right)^{-\frac{1}{1-m}}$, $m>1$, %$\kappa\in(0,1)$, % and $\kappa\in\left(0,\lambda\eta_{\max}/(2\lambda\eta_{\max}+1)\right)$, 
% $\varphi\in\Phi$, and $\psi\in\Psi$ such that $F<+\infty$,
% under the control policy $\tilde{\pi}_{\triangle}$, $N_1(t)$ is bounded for all $t \geq 0$, almost surely.
%\end{proposition}
%\begin{proof}
%By contradiction, assume that $N_1(t)$ grows unbounded. This implies that there exists at least one segment, say $j$-th, in HTQ1 that will be non-empty for all $t\geq t_0$ for some $t_0\geq 0$. Therefore, under $\tilde{\pi}_{\triangle}$, for all $t\geq t_0$, at every instant of vehicle release one vehicle gets released form $j$-th segment. This implies that, for all $t\geq t_0$, the departure rate of $j$-th segment is $\triangle^m/2R$. The ratio of the arrival rate to the departure rate for this segment is 
%\begin{equation}\label{eq:arrival-service-ratio}
%\rho_j:=\frac{\lambda_j}{\triangle^m/2R}=\frac{\lambda k_j \triangle/\ell}{\triangle^m/2R}\leq \frac{\lambda F \triangle/\ell}{\triangle^m/2R} < 1
%\end{equation}
%where the second inequality follows by \eqref{eq:varphi-condition}. This implies that the arrival rate at any segment that the number of vehicles in it is growing unbounded is strictly less than the departure rate. By law of large number arguments, this leads to a contradiction and queue length at any segment cannot grow unbounded and consequently $N_1(t)$ remains bounded. This establishes this proposition. 
%\end{proof}

The following result gives an estimate of the mean waiting time in a typical sub-queue in HTQ1 under the $\pi_{\triangle}^b$ policy.

\begin{proposition}
\label{eq:waiting-time}
For $\varphi \in \Phi_F$, $F>0$, $\psi \in \Psi$, $m \in (0,1)$, there exists a sufficiently small $\triangle$ such that the average waiting time in HTQ1 under $\pi_{\triangle}^b$ is upper bounded as: 
\begin{equation}
\label{eq:W-upper-bound}
W \leq R (2 R \lambda F )^{\frac{m}{1-m}} \left(\frac{2}{m^{\frac{m}{1-m}}} + \frac{m}{m^{\frac{m}{1-m}}-m^{\frac{1}{1-m}}}  \right).
\end{equation}
%\kscomment{$(\lambda R F)^{m/(1-m)} \theta(m)$, where $\theta(m)=$}.
\end{proposition}
\begin{proof}
It is easy to see that the desired waiting time corresponds to the system time of an M/D/1 queue with load factor given by \eqref{eq:load-factor-upper-bound} along with the arrival and departure rates leading to \eqref{eq:load-factor-upper-bound}. Note that, by Lemma \ref{eq:successive-release-time-difference}, for finite $n_0$, the value of $T_1$ is finite and does not affect the average waiting time. Therefore, using standard expressions for M/D/1 queue~\cite{Kleinrock:75}, we get that the waiting time in HTQ1 is upper bounded as follows for $\rho <1$:
\begin{align}
W \leq \frac{2R}{\triangle^m} + \frac{R}{\triangle^m} \frac{\rho}{1-\rho}  & \leq \frac{2R}{\triangle^m} + \frac{R}{\triangle^m} \frac{1}{1-\rho} \nonumber \\ 
\label{eq:waiting-time-upper-bound}
& \leq \frac{2R}{\triangle^m} + \frac{R}{\triangle^m -2 R \lambda F \triangle} 
\end{align} 
It is easy to check that the minimum of the second term in \eqref{eq:waiting-time-upper-bound} over $\big(0,\triangle^*(\lambda)\big)$ occurs at  $\triangle = \left(\frac{m}{2 R \lambda F} \right)^{\frac{1}{1-m}}$. Substitution in the right hand side of the first inequality in \eqref{eq:waiting-time-upper-bound} gives the result.
\qed
\end{proof}

\begin{remark}
\label{rem:W-limit}
\eqref{eq:W-upper-bound} implies that, for every $R>0$, $F>0$, $\lambda>0$, we have $W \to 2R$ as $m \to 0^+$. 
\end{remark}

%This allows us to state the main result on throughput analysis for the sub-linear case.
We extend the notation introduced in \eqref{eq:throughput-def} to $\lambdamax(L,m,\varphi,\psi,x_0,\delta,\eta)$ to also show the dependence on maximum allowable perturbation $\eta$. This is not to be confused with the notation for $\lambdamax$ used in Theorems~\ref{thm:superlinear-bound-empty} and \ref{thm:superlinear-bound-non-empty}, where we used the notion of throughput over finite time horizons. We choose to use the same notations to maintain brevity. 

In order to state the next result, for given $R>0$, $F>0$, $m \in (0,1)$ and $\eta \geq 0$, let $\tilde{W}(m,F,R,\eta)$ 
be the value of $\lambda$ for which the right hand side of \eqref{eq:W-upper-bound} is equal to $\eta$, if such a $\lambda$ exists and is at least $L^m/\bar{\psi}$, and let it be equal to $L^m/\bar{\psi}$, otherwise. The lower bound of $L^m/\bar{\psi}$ in the definition of $\tilde{W}$ is inspired by Proposition~\ref{prop:throughput-bound-sublinear}. The next result formally states $\tilde{W}$ as a lower bound on $\lambdamax$. 

%The following results give an estimate on the mean waiting time and queue length of the vehicles in each segment of HTQ1.
% 
%\begin{proposition}
%\label{prop:pi-waiting-time-bounds}
%For all $\lambda>0$, ${\triangle< \left(\frac{2FR \lambda}{\ell}\right)^{-\frac{1}{1-m}}}$, ${m>1}$, %${\kappa\in(0,1)}$, 
%%and $\kappa\in\left(0,\lambda\eta_{\max}/(2\lambda\eta_{\max}+1)\right)$, 
%$\varphi\in\Phi$, and $\psi\in\Psi$ such that $F<+\infty$,
%under policy $\tilde{\pi}_{\triangle}$, the mean value of the queue length, $Q_i$, %\mmcomment{ and waiting time, $W_i$,} 
%in the $i$-th$ ,i=\{1,\cdots,\ell/\triangle\}$, segment is upper bounded by
%\begin{equation}\label{eq:mean-queue-and-waiting}
%E[Q_i] \leq \frac{2\rho_i-\rho_i^2}{2(1-\rho_i) } ,  \quad \forall i
%\end{equation}
%%where $\rho_i := \lambda_i (2R/\triangle^m)$.
%\end{proposition}
%\begin{proof}
% We relate each segment to an M/D/1 queue. Under $\tilde{\pi}_{\triangle}$, the fixed time between successive vehicle releases in each segment equals $2R/\triangle^m$. However, note that whenever a vehicle finds a segment empty, its waiting time will be equal or less than ${D := 2R/\triangle^m}$. This implies that the waiting time and queue length in each segment is upper bounded by a corresponding M/D/1 queue. For an M/D/1 queue, the mean queue length, $Q$,  can be computed as \cite{Kleinrock:75}
% \begin{equation}\label{eq:md1-mean-queue-length}
% E[Q] = \frac{2\rho-\rho^2}{2(1-\rho)}
% \end{equation}
%where $\rho = \lambda D<1$. Note that by \eqref{eq:arrival-service-ratio}, $\rho_i <1$ for all $i$. This, combined with \eqref{eq:md1-mean-queue-length} implies the upper bound on the mean queue length on the segments. 
%\end{proof}



%\begin{proposition}
%\label{prop:pi1-policy}
% For all $\lambda\geq 0$, $\triangle\leq \left(\frac{ FR \lambda}{\kappa\ell}\right)^{-\frac{1}{1-m}}$, and $\kappa<\lambda\eta_{\max}/(2\lambda\eta_{\max}+1)$, under the control policy $\tilde{\pi}_{\triangle}$, $N_1(t)$ is bounded for all $t \geq 0$, almost surely.
%\end{proposition}
%\begin{proof}
%By contradiction, assume that $N_1(t)$ grows unbounded. This implies that there exists at least one segment, say $j$-th, in HTQ1 where it will be non-empty for all $t\geq t_0$ for some $t_0\geq 0$. Therefore, under $\tilde{\pi}_{\triangle}$, for all $t\geq t_0$, at every instant of vehicle release one vehicle gets released form $j$-th segment. This implies that, for all $t\geq t_0$, the departure rate of $j$-th segment is $\triangle^m/2R$. The ratio of the arrival rate to the departure rate for this segment is 
%\begin{equation}\label{eq:arrival-service-ratio}
%\frac{\lambda k_j \triangle/\ell}{\triangle^m/2R}\leq \frac{\lambda F \triangle/\ell}{\triangle^m/2R} = 2\kappa< 1
%\end{equation}
%where the second inequality follows by \eqref{eq:varphi-condition}. This implies that the arrival rate at any segment that the number of vehicles in it is growing unbounded is strictly less than the departure rate. By law of large number arguments, this leads to a contradiction and queue length at any segment cannot grow unbounded and consequently $N_1(t)$ remains bounded. This establishes this proposition. 
%\end{proof}

%The following result gives an estimate on the waiting time and queue length of the vehicles in each segment of HTQ1.
 
%\begin{proposition}
%\label{prop:pi-waiting-time-bounds}
%For all $\lambda \geq0$, $\triangle\leq \left(\frac{FR \lambda}{\kappa\ell}\right)^{-\frac{1}{1-m}}$, and $\kappa<\lambda\eta_{\max}/(2\lambda\eta_{\max}+1)$, under the control policy $\tilde{\pi}_{\triangle}$, the mean value of the queue length, $Q_i$ and waiting time, $W_i$, in the $i$-th $i=\{1,\cdots,\ell/\triangle\}$ segment is upper bounded by
%\begin{equation}\label{eq:mean-queue-and-waiting}
%E[Q_i] \leq \frac{\lambda_i D}{1-\lambda_i D}-\frac{(\lambda_i D)^2}{2(1-\lambda_i D)}\leq G , \quad E[W_i] = \frac{E[Q_i]}{\lambda_i}\leq \frac{D}{1-\lambda_i D}-\frac{\lambda_i D^2}{2(1-\lambda_i D)}\leq \eta_{\max} \quad \forall i
%\end{equation}
%where $D=2R/\triangle^m$.
%\end{proposition}
%\begin{proof}
 %we relate each segment to an M/D/1 queue. Under $\tilde{\pi}_{\triangle}$, the fixed service time $D$ (the time between successive vehicle releases) in each segment equals $2R/\triangle^m$. However, note that whenever a vehicle finds a segment empty, its waiting time will be equal or less than $D = 2R/\triangle^m$. This implies that the waiting time and queue length in each segment is upper bounded by a corresponding M/D/1 queue. For an M/D/1 queue, the mean queue length, $Q$,  can be computed as \cite{Kleinrock:75}
 %\begin{equation}\label{eq:md1-mean-queue-length}
 %E[Q] = \frac{\rho}{1-\rho}-\frac{\rho^2}{2(1-\rho)}
 %\end{equation}
%where $\rho = \lambda D<1$. By \eqref{eq:arrival-service-ratio} $\rho=\lambda_i D \leq 2\kappa<1$. This, combined with \eqref{eq:md1-mean-queue-length} implies the first upper bound on the mean queue length. Also, note that \eqref{eq:md1-mean-queue-length} is increasing in $\rho<1$. Therefore, in our case, since $\rho\leq 2\kappa<1$, the maximum is achieved at $\rho=2\kappa$ which equals to
%\be\label{eq:def-constant1}
%G: = \frac{2\kappa}{1-2\kappa}-\frac{(2\kappa)^2}{2(1-2\kappa)}\leq \frac{2\kappa}{1-2\kappa}\leq \lambda\eta_{\max}
%\ee
 %where the second inequality follows since $\kappa<\lambda\eta_{\max}/(2\lambda\eta_{\max}+1)$. This implies the second upper bound on the mean queue length and by applying Little's law, one can also get the upper bounds on the mean waiting time. 
%\end{proof}



%\subsubsection{Simple Case}\label{sec:simple-case}
%We first consider the case when the following assumption is satisfied. 

%\begin{assumption}
%\label{ass:arrival-departure-separation}
%$\text{dist}\left(\text{supp}(\varphi),\text{supp}(\psi)\right) > 0$. 
%\end{assumption}
%Assumption~\ref{ass:arrival-departure-separation} implies that the set of arrival locations is strictly separated from the set of departure locations. 

%\kscomment{
%We establish the result on throughput under the following assumption. 
%\begin{assumption}
%\label{ass:simple-case}
%Every vehicle in HTQ2 travels at unit speed at all time instants.
%%\item All the vehicles present initially in HTQ2 are uniformly spaced
%\end{assumption}
%Assumption~\ref{ass:simple-case} is likely to be true as $m \to 0^+$.
%}
%\mmcomment{Let 
%\begin{equation}
%\label{eq:Delta-selection}
%\triangle(\lambda):=(4 \lambda)^{-\frac{1}{1-m}}.
%\end{equation}}
%\begin{equation}
%\label{eq:n-tilde}
%\tilde{n} \geq 2 \lambda. 
%\end{equation}

%\begin{definition}[Release Control Policy $\pi_\triangle$]
%For $\triangle > 0$, $\pi_{\triangle}$ releases vehicle into HTQ2 so that the inter-vehicle distance in front and behind the vehicle being released is at least equal to $\triangle$. 
%\end{definition}
%Monotonicity implies that the minimum inter-vehicle distance under $\pi_{\triangle}$ is at least $\triangle$. 



%Now, we want to design a conservative policy $\tilde{\pi}_\triangle$. First, note that Assumption~\ref{ass:arrival-departure-separation} implies that, when releasing vehicles into HTQ2, $\tilde{\pi}_{\triangle}$ only has to be considerate of the distance to the vehicle in front. Without loss of generality,  let $\text{supp}(\varphi)=[0,\ell]$ for some $\ell \in [0,L)$. The conservative policy $\tilde{\pi}_\triangle$ is described as follows. Divide $[0,\ell]$ into sub-intervals, each of length $\triangle$. Release vehicles into HTQ2 as per the following iterations, starting from the first time instant when there is no vehicle in $[0,\ell+\triangle]$. 
%Release vehicles simultaneously from all odd segments, which ensures that $\ymin \geq \triangle$ at the time of release. Release vehicles from even segments the next time instant when no vehicle is in $[0,\ell+\triangle]$ in HTQ2, and so on. Note that the speed of every vehicle is at least $\triangle^m$. If every sub-interval is non-empty at every time instant of vehicle release, then the time difference between successive instants of vehicle release (during a busy period) from each segment, is at most $2(\ell + \triangle)/\triangle^m$.

%\begin{remark}
%$\tilde{\pi}_\triangle$ is conservative in the sense that it assumes that every sub-interval is non-empty at every instant of vehicle release. Nevertheless, the implementation of $\tilde{\pi}_\triangle$, under Assumption~\ref{ass:arrival-departure-separation}, will always imply the desired bound on minimum inter-vehicle distances i.e. $y_{\min}\geq \triangle$
%\end{remark}

%The next result quantifies the departure process from HTQ1 under $\tilde{\pi}_\triangle$.

%\begin{lemma}
%\label{lem:htq1-departure-simple-case-uniform}
%If Assumption~\ref{ass:arrival-departure-separation} holds true, and $\varphi$ is a uniform distribution, then the departure rate from each segment, under $\tilde{\pi}_\triangle$, is equal to $\min{\{\lambda\triangle/\ell, \triangle^m/2(\ell+\triangle)\}}$. 
%\end{lemma}
%\begin{proof}
% As we described earlier, under $\tilde{\pi}_\triangle$, we divide the support of $\varphi$ to segments of length $\triangle$. Since $\varphi$ is a uniform distribution, the probability of falling a vehicle into a specific segment equals $\triangle/\ell$. Therefore, the arrival rate of each segment would be $\lambda \triangle/\ell$. Implementation of $\tilde{\pi}_\triangle$ implies that that the departure rate from each segment can be at most $\triangle^m/2(\ell+\triangle)$. Therefore, when the arrival rate for each segment, $\lambda\triangle/\ell$ is smaller than the maximum possible departure rate, the departure rate equals the arrival rate. Otherwise, the departure rate is restricted to the maximum value i.e. $\triangle^m/2(\ell+\triangle)$. This establishes this lemma.
%\end{proof}

%The above result is for uniform $\varphi$. However, we can generalize it. Let $z_i, i=1,\cdots,\ell/\triangle$ denote the middle point of $i$-th segment. Then, $p_i=\varphi(z_i)\triangle$ represents the probability of falling a vehicle into $i$-th segment. Note that, for uniform distribution, this probability is equal to $\triangle/\ell$ for all $i$. We consider a general $\varphi$ that satisfies,

%\begin{equation}\label{eq:varphi-condition}
%p_i = \varphi(z_i)\triangle =k_i \triangle/\ell, \quad 0\leq k_i\leq F \quad \forall i
%\end{equation}
%Therefore, the arrival rate of $i$-th segment can be denoted as $\lambda_i=\lambda p_i = k_i\triangle/\ell$.
%Now, we state similar result as Lemma \ref{lem:htq1-departure-simple-case-uniform} for the distributions that satisfy \eqref{eq:varphi-condition}.

%\begin{lemma}
%\label{lem:htq1-departure-simple-case-general}
%If Assumption~\ref{ass:arrival-departure-separation} holds true, and $\varphi$ satisfies \eqref{eq:varphi-condition}. Then, the departure rate from $i$-th segment $i=\{1,\cdots,\ell/\triangle\}$, under $\tilde{\pi}_\triangle$, is equal to $\min{\{\lambda_i, \triangle^m/2(\ell+\triangle)\}}$. 
%\end{lemma}
%\begin{proof}
%The proof is similar to the proof of Lemma \ref{lem:htq1-departure-simple-case-uniform}. The arrival rate for $i$-th segment is $\lambda_i=\lambda k_i \triangle /\ell$, and the departure rate equals to the arrival rate until arrival rate is smaller than the maximum possible departure rate i.e. $\triangle^m/2(\ell+\triangle)$.
%\end{proof}
%Let $N_1(t)$ and $N_2(t)$ be the queue lengths of HTQ1 and HTQ2, respectively, at time $t$. Under policy $\tilde{\pi}_{\triangle}$, we have $N_2(t) \leq L/\triangle < +\infty$ for all $t \geq 0$. Therefore, in order to prove stability, it is sufficient to show that $N_1(t)$ remains bounded at all times. 
%\begin{proposition}
%\label{prop:pi1-policy}
%If Assumption~\ref{ass:arrival-departure-separation} holds true, $\varphi$ satisfies \eqref{eq:varphi-condition}, and $\triangle\leq (8 F \lambda)^{-\frac{1}{1-m}}$, then for every $\lambda > 0$, under the control policy $\tilde{\pi}_{\triangle}$, $N_1(t)$ is bounded for all $t \geq 0$, almost surely.
%\end{proposition}
%\begin{proof}
%By contradiction, assume that $N_1(t)$ grows unbounded. This implies that there exists at least one segment, say $j$-th, in HTQ1 where it will be non-empty for all $t\geq t_0$ for some $t_0\geq 0$. Therefore, under $\tilde{\pi}_{\triangle}$, for all $t\geq t_0$, at every instant of vehicle release (i.e. every $2(\ell + \triangle)/\triangle^m$ unit of time), at least one vehicle gets released form $j$-th segment. This implies that, for all $t\geq t_0$, the departure rate of $j$-th segment is $\triangle^m/2(\ell + \triangle)$. Also, the arrival rate to this segment is $\lambda k_j \triangle/\ell$. The ratio of the arrival rate to the departure rate is 
%\begin{equation}\label{eq:arrival-service-ratio}
%\frac{\lambda k_j \triangle/\ell}{\triangle^m/2(\ell + \triangle)}\leq \frac{\lambda F \triangle/\ell}{\triangle^m/4\ell} \leq \frac{1}{2}
%\end{equation}
%This implies that the arrival rate at any segment that the number of vehicles in it is growing unbounded is strictly less than the departure rate. By law of large number arguments, this leads to a contradiction and queue length at any segment cannot grow unbounded and consequently $N_1(t)$ remains bounded. This establishes this proposition. 
%\end{proof}

%\subsubsection{General Case}
%In this section, we extend results under relaxation of Assumption~\ref{ass:arrival-departure-separation}. Unlike the simple case, in the general case, when releasing vehicles, the release control policy also has to be cognizant of inter-vehicular distances in front and back of 
%the vehicle being released. We slightly modify $\tilde{\pi}_\triangle$ in section \ref{sec:simple-case}. Now, the time difference between successive instants of vehicle release at a segment is $C/2\triangle^m$. We start by generalizing Lemma~\ref{lem:htq1-departure-simple-case-general}.

%\begin{equation}
%\label{eq:Delta-selection-general-case}
%\triangle(\lambda):=\left(\frac{2 C}{\ell} \lambda \right)^{-\frac{1}{1-m}}.
%\end{equation}

%\begin{lemma}
%\label{lem:htq1-departure-general-case-general}
%If $\varphi$ satisfies \eqref{eq:varphi-condition}, then the departure rate from $i$-th segment, $i=\{1,\cdots,\ell/\triangle\}$, under $\tilde{\pi}_\triangle$, is equal to $\min{\{\lambda_i, \triangle^m/2C\}}$. 
%\end{lemma}
%\begin{proof}
%The proof is similar to the proof of Lemma \ref{lem:htq1-departure-general-case-general}. 
%\end{proof}

%Now, we show that $N_1(t)$ remains bounded all the time. 

%\begin{proposition}
%\label{prop:pi2-policy}
 %If $\varphi$ satisfies \eqref{eq:varphi-condition} and $\triangle\leq \left(\frac{4 FC \lambda}{\ell}\right)^{-\frac{1}{1-m}}$, then for every $\lambda > 0$, under the control policy $\tilde{\pi}_{\triangle}$, $N_1(t)$ is bounded for all $t \geq 0$, almost surely.
%\end{proposition}
%\begin{proof}
%By contradiction, assume that $N_1(t)$ grows unbounded. This implies that there exists at least one segment, say $j$-th one, in HTQ1 where it will be non-empty for all $t\geq t_0$ for some $t_0\geq 0$. Therefore, under $\tilde{\pi}_{\triangle}$, for all $t\geq t_0$, at every instant of vehicle release (i.e. every $2C/\triangle^m$ unit of time), at least one vehicle gets released from $j$-th segment. This implies that, for all $t\geq t_0$, the departure rate of $j$-the segment is $\triangle^m/2(\ell + \triangle)$. Also, arrival rate to this segment is $\lambda k_j \triangle/\ell$. The ratio of the arrival rate to the departure rate is 
%\begin{equation}\label{eq:arrival-service-ratio2}
%\frac{\lambda k_j \triangle/\ell}{\triangle^m/2C}\leq \frac{\lambda F \triangle/\ell}{\triangle^m/2C} \leq \frac{1}{2}
%\end{equation}
%This implies that the arrival rate at any segment that the number of vehicles in it is going to infinity is strictly less than the departure rate. By law of large number arguments, this leads to a contradiction and queue length at any segment cannot grow unbounded and consequently $N_1(t)$ remains bounded  This establishes this proposition. 
%\end{proof}

%The following result gives an estimate on the waiting time and queue length of the vehicles in each segment of HTQ1.
 
%\begin{proposition}
%\label{prop:pi1-policy}
% If $\varphi$ satisfies \eqref{eq:varphi-condition}, then for every $\lambda > 0$ and  $\triangle\leq (8 F \lambda)^{-\frac{1}{1-m}}$, under the control policy $\tilde{\pi}_{\triangle}$, the mean value of the queue length, $Q_i$ and waiting time, $T_i$, in the $i$-th $i=\{1,\cdots,\ell/\triangle\}$ segment is upper bounded by
%\begin{equation}\label{eq:mean-queue-and-waiting}
%E[Q_i] \leq \frac{\lambda_i D}{1-\lambda_i D}-\frac{(\lambda_i D)^2}{2(1-\lambda_i D)} , \quad E[T_i] = \frac{E[Q_i]}{\lambda_i}\leq \frac{D}{1-\lambda_i D}-\frac{\lambda_i D^2}{2(1-\lambda_i D)}
%\end{equation}
%where $D=2C/\triangle^m$.
%\end{proposition}
%\begin{proof}
% we relate each segment to an $M/D/1$ queue. Under $\tilde{\pi}_{\triangle}$, the fixed service time $D$ (the time between successive vehicle releases) in each segment equals $2C/\triangle^m$. However, note that whenever a vehicle finds a segment empty, its waiting time will be equal or less than $D = 2C/\triangle^m$. This implies that the waiting time and queue length in each segment is upper bounded by a corresponding $M/D/1$ queue. For an $M/D/1$ queue, the mean queue length, $Q$,  can be computed as \cite{Kleinrock:75}
 %\begin{equation}\label{eq:md1-mean-queue-length}
% E[Q] = \frac{\rho}{1-\rho}-\frac{\rho^2}{2(1-\rho)}
 %\end{equation}
%where $\rho = \lambda D<1$. By \eqref{eq:arrival-service-ratio2} $\rho=\lambda_i D \leq 1/2$. This, combined with \eqref{eq:md1-mean-queue-length} implies the upper bound on the mean queue length, and by applying Little's law, one can also get the upper bound on the mean waiting time. 
%\end{proof}

%\begin{remark}
%By Proposition \ref{prop:pi2-policy} we know that for every $\lambda \geq 0$ one can choose a $\triangle$ so that the system remains stable. Therefore, in \eqref{eq:mean-queue-and-waiting}, the mean waiting time for the segments will be very small for high values of $\lambda$. Since waiting time is a positive random variable, this also implies that waiting time is also very small for large values of $\lambda$. This implies that for large values of $\lambda$ the time perturbation of the arrival process is \mmcomment{small}.
%\end{remark}

%\subsubsection{Proof of Theorem \ref{thm:main-sub-linear}}\label{sec:proof-of-main-thm}


%The following result characterizes a $\triangle\in\left(0, \left(\frac{ 2FR \lambda}{\ell}\right)^{-\frac{1}{1-m}}\right)$ under which the system remains stable and the upper bound on the mean waiting time on segments is minimized.  
%\begin{proposition}\label{prop:p1-waiting-time}
%For all $\lambda \geq 0$, $m>1$, $\varphi\in\Phi$, $\psi\in\Psi$ such that $F<+\infty$, for $\triangle= \left(\frac{ 2(2-m) FR \lambda}{\ell}\right)^{-\frac{1}{1-m}}$, under policy $\tilde{\pi}_\triangle$ the mean waiting time on any segment, $W_i$, is upper bounded by 
%\begin{equation*}
%E[W_i]\leq  \frac{\left(2(2-m)\lambda FR\ell^{-1}\right)^{\frac{1}{1-m}}(2-m)}{\lambda F \ell^{-1}(1-m)}:=\tilde{W} \quad \forall i
%\end{equation*}
%\end{proposition}
%\begin{proof}
%Consider the range of $\triangle$ suggested in Proposition \ref{prop:pi1-policy} for which the queue remains stable. We focus on the busiest segment, say $j$-th, %, and define its load factor as $\tilde\rho:\max_{i}\rho_i$. 
%since the upper bounds derived for the busiest segment will be an upper bound for other segments, as well. Note that since the time between successive vehicle releases for all segments is the same, the busiest segment is the segment with the highest arrival rate, i.e. $k_j=F$, therefore $\lambda_j=\lambda F\triangle/\ell$ and ${\rho_j=2\lambda FR\triangle^{1-m} /\ell<1}$.  
%By Proposition \ref{prop:pi1-policy}, the mean queue length on $j$-th segment is upper bounded bounded by,
%\begin{equation*}
%E[Q_j] \leq \frac{2\rho_j-\rho_j^2}{2(1-\rho_j) } \leq \frac{\rho_j}{1-\rho_j } \leq \frac{1}{1-\rho_j}
%\end{equation*}
%where the second and third inequalities are easy to show. Now, by applying Little's law, we get the following upper bound on the mean waiting time
%\begin{equation}\label{eq:mean-waiting-busiest}
%E[W_j]=\frac{E[Q_j]}{\lambda_j}  \leq \frac{1}{\lambda_j(1-\rho_j)}
%\end{equation}
%Let $\tilde{f}(\triangle):=\lambda_j(1-\rho_j)=\lambda F\ell^{-1}\triangle(1-2\lambda FR\ell^{-1}\triangle^{1-m})$. Since $m<1$ and $F,R,\ell, \lambda > 0$, then $\tilde{f}(\triangle)$ is a concave function in $\triangle$. Thus, in order to minimize the upper bound in \eqref{eq:mean-waiting-busiest}, we maximize $\tilde{f}(\triangle)$. It turns out that for ${\triangle ^*:=\left(\frac{ 2(2-m) FR \lambda}{\ell}\right)^{-\frac{1}{1-m}}}$,  $\tilde{f}'(\triangle^*)=0$ and consequently $\tilde{f}$ is maximized. The upper bound for the mean waiting time is then derived by plugging $\triangle^*$ in \eqref{eq:mean-waiting-busiest}. 
%\end{proof}



\begin{theorem}\label{thm:main-sub-linear}
For any $\varphi \in \Phi_F$, $F>0$, $\psi \in \Psi$ with $\text{supp}(\psi)=[0,R]$, $R>0$, $m \in (0,1)$, $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$, $L>0$, and maximum permissible perturbation $\eta \geq 0$, 
$$
\lambdamax(L,m,\varphi,\psi,x_0,\delta=0,\eta) \geq \tilde{W}(m,F,R,\eta)
$$
In particular, if $\eta > 2R$, then $\lambdamax(L,m,\varphi,\psi,x_0,\delta=0,\eta) \to + \infty$ as $m \to 0^+$.
\end{theorem}
%\ksmargin{proof is incomplete}
\begin{proof}
Consider any $\lambda \leq\tilde{W}(m,F,R,\eta)$, and $\triangle \leq \left(\frac{m}{2 R \lambda F} \right)^{\frac{1}{1-m}}$. Under policy $\pi_\triangle^b$,  Lemma \ref{eq:successive-release-time-difference} and Proposition \ref{prop:pi1-policy} imply that, for finite $n_0$, $N_2(t)$ and $N_1(t)$ remain bounded for all times, with probability one. Also, for $\lambda = \tilde{W}(m,F,R,\eta)$, by Proposition \ref{eq:waiting-time} and the definition of $\tilde{W}(m,F,R,\eta)$, the introduced perturbation remains upper bounded by $\eta$. Since the right hand side of \eqref{eq:W-upper-bound} is monotonically increasing in $\lambda$, perturbations remain bounded by $\eta$ for all $\lambda \leq \tilde{W}(m,F,R,\eta)$. 
In particular, by Remark \ref{rem:W-limit}, we have $W\to 2R$ as $m\to 0^+$. In other words, as $m\to 0^+$, the magnitude of the introduced perturbation becomes independent of $\lambda$. 
Therefore, when $\eta >2R$, and $m\to 0^+$  throughput can grow unbounded while perturbation and queue length remains bounded.
%\kscomment{(Follows trivially from Propositions~\ref{prop:pi1-policy} and \ref{eq:waiting-time})}
\qed
\end{proof}

%\begin{theorem}\label{thm:main-sub-linear}
%For any $\lambda > 0$, $m>1$, , $\varphi\in\Phi$, $\psi\in\Psi$ such that $F<+\infty$,  there exists a perturbed arrival process with $\eta<\tilde{W}$ under which the queue length remains bounded, almost surely. 
%\end{theorem}
%\begin{proof}
%Pick $\triangle = \left(\frac{ 2(2-m) FR \lambda}{\ell}\right)^{-\frac{1}{1-m}}$ and implement the conservative release control policy, $\tilde{\pi}_{\triangle}$. Implementation of this policy implies the boundedness of HTQ2 for all the time. Also, by Proposition \ref{prop:pi1-policy} queue length in HTQ1 will also remain bounded, almost surely. Moreover, Proposition \ref{prop:p1-waiting-time} implies that the perturbation introduced by $\tilde{\pi}_\triangle$ is upper bounded by $\tilde{W}$. This establishes this theorem. 
%\end{proof}

%\begin{remark}
%Following Remark~\ref{rem:W-limit}, for given $\varphi \in \Phi_F$, $F>0$, $\psi \in \Psi$ with $\text{supp}(\psi)=[0,R]$, $R>0$, $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$, $n_0<\infty$, $L>0$, if $\eta > 2 R$, then $\lambdamax(L,m,\varphi,\psi,x_0,\delta=1,\eta) \to + \infty$ as $m \to 0^+$.
%\end{remark}

%\kscomment{(add a rigorous remark here as to why the perturbation method does not give a better lower bound on the throughput for the super-linear case)}

\begin{remark}
We emphasize that the only feature required in a batch release control policy is that, at the moment of release, the front and rear distances for the vehicles being released should be greater than $\triangle$. The requirement of the policy in Definition~\ref{def:batch-release-control-policy} for the road to be empty at the moment of release makes the control policy conservative, and hence affects the maximum permissible perturbation. In fact, for special spatial distributions, e.g., when $\varphi$ is a Dirac delta function and the support of $\psi$ is $[0,L-\triangle])$, one can relax the conservatism to guarantee unbounded throughput for arbitrarily small permissible perturbation. 
\end{remark}

\subsubsection{The Super-linear Case}

In this section, we study the throughput for the super-linear case under perturbed arrival process with a maximum permissible perturbation of $\eta$. For this purpose, we consider the batch release control policy $\pi_{\triangle}^b$, defined in Definition \ref{def:batch-release-control-policy}, for our analysis. Time intervals  between release of successive batches, under $\pi_{\triangle}^b$, are characterized the same as Lemma \ref{eq:successive-release-time-difference}. However, in the super linear case, by Lemma \ref{lem:service-rate-bounds}, the initial minimum service rate is $L^mn_0^{1-m}$. Therefore, the time of first release is bounded as $T_1<n_0^mR/L^m$. Moreover, similar to the proof of Lemma \ref{eq:successive-release-time-difference}, it can be shown that $\ymin(t)\geq \triangle$ for all $t\geq T_1$. 

During $[0,T_1]$, the service rate of all sub-queues remain zero; however, when $n_0<+\infty$, $T_1$ is finite and for the computation of load factor this time interval can be neglected. Therefore,  the load factor for each sub-queue will be the same as the sub-linear case \eqref{eq:load-factor-upper-bound}. In this case, however, in order to have $\rho<1$, we get the counterpart of \eqref{eq:triangle-star} as:
\begin{equation}\label{eq:triangle-star-superlinear}
\triangle > \triangle^*(\lambda).
\end{equation}
It should be noted that since the batch release control policy iteratively releases from odd and even sub-queues, we need at least two sub-queues to be able to implement this policy. As a result, $\triangle$ cannot be arbitrary large and $\triangle<\ell/2$. This constraint gives the following  bound on the admissible throughput under this policy
\begin{equation}\label{eq:lambda-star-superlinear}
\lambda<\lambda^*:=(\ell/2)^{m-1}/2RF
\end{equation}
% In order to have bounded queue length, the counter part to \eqref{eq:triangle-star} i.e. $\triangle > \triangle^*:=\left(2 R \lambda F \right)^{-\frac{1}{1-m}},$ should be satisfied. However, $\triangle^*$ is an increasing function of $m$ in this case, so there may not exist feasible $\triangle$ for all the $\lambda>0$. For example, for $\lambda = 1$, $L=1$, $\varphi=U_{[0,L]}$, $\psi=U_{[0,L]}$, and $m=2$, by \eqref{eq:triangle-star}, $\triangle^*=2$. However, there does not exist any $\triangle>\triangle^*$ because $L=1$. Thus, this policy is not generally applicable to the super-linear case, so we do not pursue its analysis in this case. 
 The following result shows that for the above range of throughput, the queue length in HTQ1, $N_1(t)$, remains bounded at all times. 
  \begin{proposition}
\label{prop:pi1-policy-super-linear}
For any $\lambda<\lambda^*$, $\triangle\in\big(\triangle^*(\lambda),\ell/2\big]$, $\varphi \in \Phi_F$, $F>0$, $\psi \in \Psi$ with $\supp(\psi)=[0,R]$, $R>0$, $m>1$, $x_0\in[0,L]^{n_0}$, $L>0$, $n_0\in \mathbb{N}$, $N_1(t)$ is bounded for all $t \geq 0$ under $\pi_{\triangle}^b$, almost surely.
\end{proposition}

\begin{proof}
The proof is similar to proof of Proposition \ref{prop:pi1-policy}. In particular, by \eqref{eq:triangle-star-superlinear} and \eqref{eq:lambda-star-superlinear}, one can show that load factor \eqref{eq:load-factor-upper-bound} remains strictly smaller than one. This implies that no sub-queue in HTQ1 can grow unbounded, and $N_1(t)$ remains bounded for all times, with probability one. 
%By contradiction, assume that $N_1(t)$ grows unbounded. This implies that there exists at least one sub-queue, say $ j \in \{1, 2, \ldots, \lceil \frac{\ell}{\triangle} \rceil\}$, such that its queue length, say $N_{1,j}(t)$, grows unbounded. In particular, this implies that there exists $t_0 \geq T_1$ such that $N_{1,j}(t) \geq 2$ for all $t \geq t_0$. Therefore, for all $t \geq t_0$, the ratio of arrival rate to departure rate for the $j$-th sub-queue is given by \eqref{eq:load-factor-upper-bound} which is an increasing function of $\lambda$. It is sufficient to show the result for $\lambda=\lambda^*$. For $\lambda=\lambda^*$, by \eqref{eq:lambda-star-superlinear} and \eqref{eq:triangle-star-superlinear}, we have $\triangle^* = \kappa_1\ell/2$. Consequently, there exists a $\triangle\in(\triangle^*,\ell/2]$ such that, by \eqref{eq:triangle-star-superlinear}, the ratio of arrival to departure rate is strictly smaller than one. Since $\triangle^*$ is an increasing function of $\lambda$, the same result follows for all $\lambda\leq \lambda^*$.  A simple application of the law of large numbers then implies that, almost surely, $N_{1,j}(t)=0$ for some finite time, leading to a contradiction.
\qed
\end{proof}

 %Moreover, Figure \ref{fig:release-policy-vs-thm2} shows that, for the cases that this policy is applicable, the lower bounds on throughput achieved from Theorem \ref{thm:superlinear-bound-empty} are better.  

\begin{proposition}
\label{eq:waiting-time-super-linear}
For any $\lambda<\lambda^*$, $\varphi \in \Phi_F$, $F>0$, $\psi \in \Psi$, $m> 1$, the average waiting time in HTQ1 under $\pi_{\triangle}^b$ for $\triangle = \ell/2$ is upper bounded as: 
\begin{equation}
\label{eq:waiting-time-super-linear-eq}
W \leq \frac{2R}{(\ell/2)^m}+\frac{R}{(\ell/2)^m}\frac{2R\lambda F(\ell/2)^{1-m}}{1-2R\lambda F(\ell/2)^{1-m}}
\end{equation}
%\kscomment{$(\lambda R F)^{m/(1-m)} \theta(m)$, where $\theta(m)=$}.
\end{proposition}
\begin{proof}
The proof is very similar to the proof of Proposition \ref{eq:waiting-time}. Thus, we get the following bounds:
\begin{align*}
W \leq \frac{2R}{\triangle^m} + \frac{R}{\triangle^m} \frac{\rho}{1-\rho}  \leq \frac{2R}{\triangle^m}+\frac{R}{\triangle^m}\frac{2R\lambda F\triangle^{1-m}}{1-2R\lambda F\triangle^{1-m}}
\end{align*} 
The right hand side of the above inequality is a decreasing function of $\triangle$; therefore, $\triangle = \ell/2$ minimizes it, and gives \eqref{eq:waiting-time-super-linear-eq}. 
%By relating each sub-queue to an M/D/1 queue, for a given load factor $\rho<1$, we can get the following upper bound on the average system time of a typical sub-queue. Also, for finite $n_0$, the value of $T_1$ is finite and does not affect the average waiting time. Therefore, we get that the waiting time in HTQ1 is upper bounded as follows:
%\begin{align*}
%W \leq \frac{2R}{\triangle^m} + \frac{R}{\triangle^m} \frac{\rho}{1-\rho}  
%\end{align*} 
\qed
\end{proof}

Let $\hat{W}(m,F,R,\eta)$ 
be the value of $\lambda$ for which the right hand side of \eqref{eq:waiting-time-super-linear-eq} is equal to $\eta$, if such a $\lambda\leq \lambda^*$ exists, and let it be equal to $\lambda^*$ otherwise. Note that since the right hand side of \eqref{eq:waiting-time-super-linear-eq} is monotonically increasing in $\lambda$, for all $\lambda\leq \hat{W}(m,F,R,\eta)$ the introduced perturbation remains upper bounded by $\eta$. 
\begin{theorem}\label{thm:main-batch-super-linear}
For any $\varphi \in \Phi_F$, $F>0$, $\psi \in \Psi$ with $\text{supp}(\psi)=[0,R]$, $R>0$, $m >1$, $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$, $L>0$, and maximum permissible perturbation $\eta \geq 0$, 
$$
\lambdamax(L,m,\varphi,\psi,x_0,\delta=0,\eta) \geq \hat{W}(m,F,R,\eta)
.$$
\end{theorem}
%\ksmargin{proof is incomplete}
\begin{proof}
For any $\lambda <\hat{W}(m,F,R,\eta)$, under $\pi_\triangle^b$, Lemma \ref{eq:successive-release-time-difference} and Proposition \ref{prop:pi1-policy-super-linear} imply that, for finite $n_0$, $N_2(t)$ and $N_1(t)$ remain bounded for all times, with probability one. Also, by Proposition \ref{eq:waiting-time-super-linear} and the definition of $\hat{W}(m,F,R,\eta)$, the introduced perturbation remains upper bounded by $\eta$. 
%Let us pick a $\triangle\in[\triangle^*,\ell/2]$, consider any $\lambda <\hat{W}(m,F,R,\eta)$, and implement policy $\pi_\triangle^b$. Lemma \ref{eq:successive-release-time-difference} and Proposition \ref{prop:pi1-policy-super-linear} imply that, for finite $n_0$, $N_2(t)$ and $N_1(t)$ remain bounded for all times, with probability one. Also, by Proposition \ref{eq:waiting-time-super-linear} and the definition of $\hat{W}(m,F,R,\eta)$, the introduced perturbation remains upper bounded by $\eta$. 
\qed
\end{proof}


%\begin{theorem}\label{thm:main-sub-linear}
%For any $\lambda > 0$, $\eta_{\max}> 0$, $m>1$, $\psi\in\Psi$, $\varphi\in\Phi$ such that $\sup_{z\in[0,\ell]}\varphi(z)<\infty$,  there exists a perturbed arrival process with $\eta\leq\eta_{\max}$ under which the queue length remains bounded. 
%\end{theorem}

%\begin{proof}
%Pick $\triangle := \left(\frac{FR \lambda}{\kappa\ell}\right)^{-\frac{1}{1-m}}$ and $\kappa<\lambda\eta_{\max}/(2\lambda\eta_{\max}+1)$. Consider the conservative release control policy $\tilde{\pi}_\triangle$ described in Section \ref{sec:release-control-policy}. Implementation of this policy implies that queue length in HTQ2 remains bounded for all the time. Also, by Proposition \ref{prop:pi1-policy} queue length in HTQ1 will also remain bounded. Moreover, Proposition \ref{prop:pi-waiting-time-bounds} implies that the perturbation is upper bounded by $\eta_{\max}$. This establishes this theorem. 
%\end{proof}

%\begin{remark}
%In Theorem \ref{thm:main-sub-linear} it is assumed that $\sup_{z\in[0,\ell]}\varphi(z)<\infty$ i.e. $F<\infty$. However, this assumption is not true when $\varphi$ is a Dirac delta function. For that case and when $R< L$, one can consider a modified policy in order to show the stability of queue for any $\lambda\geq0$. In this case, there is no need to dived the support of $\varphi$ and we consider only one queue. Also for the choice of $\triangle \leq \varepsilon:=(L-R)/2$ the policy does not need to be considerate of the rear distance. When HTQ2 is empty we release one vehicle from HTQ1. The time it takes for a vehicle to travel $\triangle$ after its release to HTQ2 is at most $\triangle^{1-m}$. Therefore, we release the next vehicle (if available) after waiting $\triangle^{1-m}$ and so on. By the proper choice of $\triangle$, one can show a similar result for Dirac delta function. 
%\end{remark}




%\kscomment{(The following is severely work in progress ...)}
%
%Let $N_1(t)$ and $N_2(t)$ be the queue lengths of HTQ1 and HTQ2 respectively at time $t$. An inter-vehicular distance $y_i$, $i \in N_2(t)$, is said to be \emph{large} if $y_i > 1/\tilde{n}$. Let $N_3(t)$ be the number of vehicles required to \emph{fill up} the large inter-vehicular distances in HTQ2 at time $t$. It is easy to see that 
%\begin{equation}
%\label{eq:N3-bound}
%N_3(t) \leq \tilde{n} \qquad \forall \, t \geq 0
%\end{equation}
%
%Consider the following control policy for releasing vehicles from HTQ1 into HTQ2. If $N_1(t) \leq N_3(t)$, then no vehicle is released into HTQ2. If $N_1(t) > N_3(t)$, then vehicles are released into HTQ2 to either fill up the gaps, or to place the vehicles in the middle of existing vehicles on HTQ2, as they are passing by. \eqref{eq:N3-bound} implies that vehicles are \kscomment{continuously} released from HTQ1 when $N_1(t) \geq \tilde{n}$.
%
%\begin{theorem}
%For any $\lambda \geq 1$, under the proposed control policy, $N_1(t) + N_2(t)$ is bounded for all $t$, almost surely. 
%\end{theorem}
%\begin{proof}
%Assume by contradiction that there exist realizations in which $N_1(t) + N_2(t)$ grows unbounded, which implies that, given $M>0$, there exists $\tilde{t}$, such that $N_1(t) + N_2(t) \geq M$ for all $t \geq \tilde{t}$. 
%Consider the following cases.
%
%\textbf{Case 1: $N_1(t)$ grows unbounded.} That is, there exists  $\tilde{t}_1 > 0$, such that $N_1(t) \geq \tilde{n}$ for all $t \geq \tilde{t}_1$. Given $\epsilon \in (0, \lambda/2)$, there exists $\tilde{t}_2>0$, such that, with probability one, the number of arrivals to HTQ1 over $[\tilde{t}_1,\tilde{t}_1+t]$ is at most $(\lambda + \epsilon)t=3 \lambda t/2$ for all $t \geq \tilde{t}_2$. Therefore, 
%\begin{equation}
%\label{eq:N1-upper-bound}
%N_1(t) \leq N_1(\tilde{t}_1) + 3 \lambda t/2, \qquad \forall \, t \geq \tilde{t}_2
%\end{equation}
%Since $N_1(t) \geq \tilde{n}$, under the proposed control policy, the time between release of successive vehicles from HTQ1 is upper bounded by $1/\tilde{n}$. Therefore, the number of departures from HTQ1 over $[\tilde{t}_1, \tilde{t}_1 + t]$ is lower bounded by $\tilde{n} t$. \eqref{eq:n-tilde} implies that $\tilde{n} \geq (2 \lambda)^{\frac{1}{1-m}} \geq 2 \lambda$, where the last inequality follows from the fact that $\lambda \geq 1$, and $m \in (0,1)$. Therefore, the number of departures over $[\tilde{t}_1, \tilde{t}_1 + t]$ is further lower bounded by $2 \lambda t$. Comparing this with \eqref{eq:N1-upper-bound} contradicts the assumption that $N_1(t)$ remains unbounded. 
%
%\textbf{Case 2: $N_2(t)$ grows unbounded.} \kscomment{(work in progress ...)}
%
%\end{proof}
















==> 02- submission/super-linear.tex <==
\subsection{Throughput Bounds for the Super-linear Case from Busy Period Calculations}\label{subsec:superlinear}
In this section, we derive lower bound on the throughput for the super-linear case. The next result computes a bound on the probability that the queue length of the HTQ satisfies a given upper bound over a given time interval, using the probability distribution functions from \eqref{eq:G-def}.
%Our analysis in this section uses the busy period calculations from Section~\ref{sec:busy-period}. 
%For our analysis, we focus on the busy period and the number of vehicles served in a busy period. We compute a lower bound on the probability of $N(t) \leq M\; \forall t\geq 0$. 
%This result leads to a probabilistic lower bound on the throughput of the system as it is stated in Theorem \ref{} and \ref{}.
%\mmcomment{We first assume an upper bound on the queue length}, i.e. $N(t)\leq M \; \forall t\geq0$, which by Lemma \ref{lem:service-rate-bounds} gives a lower bound on the service rate of the system i.e. $s(y(t))\geq L^mM^{1-m}\; \forall t\geq 0$. Then, we use this lower bound on the service rate to compare the system with a system with the same temporal-spatial arrival process but a slower decrease rate of workload . We use this comparison as a tool to find a lower bound on the probability of achieving the assumed upper bound on the queue length. This result leads to a probabilistic lower bound on the throughput of the system which is stated in Theorem \ref{}. Our analysis heavily depends on the probability distribution of busy periods which is described in the next section.
%\begin{lemma}\label{lemma:cdf-poisson}
%\mmmargin{find a proper reference}
%The cumulative distribution function of a Poisson random variable with mean $\mu > 0$ is decreasing in $\mu$.
%\end{lemma}
%\begin{proof}
%Let $X$ be a Poisson random variable with mean $\mu > 0$, then the cdf of $X$ for a fixed $n\in\mathbb{N}$ is given as \cite{?},\
%\be
%f(\mu) = \Pr(X\leq n) = \frac{\int_{\mu}^\infty t^{n}e^{-t}\de t}{n!}
%\ee 
%Since the integrand in the numerator is positive, the above function is decreasing in $\mu$.
%\end{proof}
In Propositions~\ref{prop:nbp-lower-bound} and \ref{prop:nbn-lower-bound}, for the sake of clarity, we add explicit dependence on $\lambda$ to this probability distribution function. 


% \begin{proposition}\label{prop:nbp-lower-bound}
%For any $m>1$, $M\in \mathbb{N}$, $L>0$, $\lambda >0$, $\varphi\in \Phi$, $\psi \in \Psi$, and zero initial condition $x_0=0$, the cumulative distribution function for the total number of departures from the queue during a busy period, $N_{bp}$, is given by 
%  $$\Pr(N_{bp}\leq M)\geq C^{}_{L^m M^{1-m}}(M,\lambda,\psi)$$
% \end{proposition}
% \begin{proof}
%Since the maximum queue length during a busy period is upper bounded by the total number of departures over the busy period, we have $N_{bp} \leq M$. This, combined with Lemma \ref{lem:service-rate-bounds} implies that the service rate is at least equal to $L^mM^{1-m} =: \tilde{p}$ during the busy period.  Motivated by our calculations in Section~\ref{sec:busy-period}, we compute bounds on the desired distribution of $N_{bp}$ for the actual queue, say {HTQ-F}, by comparing it with a queue, say {HTQ-S}, having constant service rate $\tilde{p}$. 
%Let consider the same realization for the arrival locations and timings of new vehicles and their desired distances to travel for both systems. Also, let  $N_{bp,f}$ and $N_{bp,s}$ be the total number of vehicles transiting through HTQ-F and HTQ-S, respectively, during a busy period. For those realizations for which $N_{bp,s}\leq M$ during the first busy, it is easy to see that the same property holds for HTQ-F i.e. $N_{bp,f}\leq M$ (see Figure \ref{fig:b1-b2} for an illustration). Because of the memoryless property of the arrival process, the same property holds for all other busy periods as well. Therefore, 
% \begin{equation*}
% \Pr(N_{bp,f}\leq M) \geq \Pr(N_{bp,s}\leq M)
% \end{equation*}
% By noting that $N_{bp}=N_{bn}+1$ for an empty initial condition, and considering \eqref{eq:busy-period-numofarrival-distribution}, we get the result.
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=7.5cm]{b1-b2} 
%\caption{Workload process for two systems under the same realization of the arrival process: a system with slower service rate (solid line) and a system with a faster service rate (dashed line).}
%\label{fig:b1-b2}
%\end{center}
%\end{figure}
% \end{proof}

\begin{proposition}\label{prop:nbp-lower-bound}
For any $m>1$, $M\in \mathbb{N}$, $L>0$, $\lambda >0$, $\varphi\in \Phi$, $\psi \in \Psi$, and zero initial condition $x_0=0$, the probability that the queue length is upper bounded by $M$ over a given time interval $[0,T]$ satisfies the following bound: 
\begin{equation}
\label{eq:nbp-lower-bound}
  \Pr \big(N(t) \leq M \quad \forall t \in [0,T] \big)\geq \sup_{r \in \NN} \, \sum_{n=1}^M \int_T^{\infty} G_{r,L^m M^{1-m}}(t,n,\psi,\lambda) \, \de t
  \end{equation}
 \end{proposition}
%\begin{proposition}\label{prop:nbp-lower-bound}
%For any $m>1$, $M\in \mathbb{N}$, $L>0$, $\lambda >0$, $\varphi\in \Phi$, $\psi \in \Psi$, and zero initial condition $x_0=0$, the cumulative distribution function for the maximum queue length during a busy period, $\Nmax$, satisfies the following bound: 
%  $$\Pr(\Nmax \leq M)\geq C^{}_{L^m M^{1-m}}(M,\lambda,\psi)$$
% \end{proposition}
 \begin{proof}
Let us denote the current queueing system as HTQ-f. We shall compare queue lengths between HTQ-f and a slower queueing system HTQ-s, which starts from the same (zero) initial condition, and experiences the same realizations of arrival times, locations and travel distances. Let every incoming vehicle into HTQ-s and HTQ-f be tagged with a unique identifier. At time $t$, let $\mc J(t)$ be the set of identifiers of vehicles present both in HTQ-s and HTQ-f, $\mc J_{s/f}(t)$ be the set of identifiers of vehicles present only in HTQ-s, and $\mc J_{f/s}(t)$ be the set of identifiers of vehicles present only in HTQ-f.
%\footnote{The case when there are vehicles present in HTQ-f, but not in HTQ-s, does not occur in our setup.} 
Let $v^f_i$ denote the speed of the vehicle in HTQ-f with identifier $i \in \mc J(t) \cup \mc J_{f/s}(t)$, as determined by the car-following behavior underlying \eqref{eq:dynamics-moving-coordinates}. The vehicle speeds in HTQ-s are not governed by the car following behavior, but are rather related to the speeds of vehicles in HTQ-f as: 
 \begin{equation}
 \label{eq:htq-s-speed}
		v^s_i(t) =\left\{\begin{array}{ll}
		\ds v^f_i(t) \frac{p}{v^f(t)} \frac{|\mc J(t)|}{|\mc J(t)| + |\mc J_{s/f}(t)|} 	&i \in \mc J(t)\\[15pt]
		\ds \frac{p}{|\mc J(t)| + |\mc J_{s/f}(t)|}& i \in \mc J_{s/f}(t)\,\end{array}\right.
	\end{equation}
%
%$v^s_i = v^f_i \frac{p}{s} \frac{|\mc I_f|}{|\mc I_f| + |\mc I_{s/f}|}$ if $i \in \mc I_f$, and $v^s_i = \frac{p}{|\mc I_f| + |\mc I_{s/f}|}$ if $i \in \mc I_{s/f}$, 
where $v^f(t):=\sum_{i \in \mc J(t)}v_i^f(t)$ is the sum of speeds of vehicles in HTQ-f that are also present in HTQ-s at time $t$, and $p$ is a parameter to be specified. Indeed, note that $\sum_{i \in \mc J(t) \cup \mc J_{s/f}(t)} v_i^s(t) \equiv p$, i.e., $p$ is the (constant) service rate of HTQ-s. 

Consider a realization where the number of arrivals into HTQ-s with $p=L^m M^{1-m}$ during any busy period overlapping with $[0,T]$ does not exceed $M$. We refer to such a realization as \emph{event} in the rest of the proof.  Since the maximum queue length during a busy period is trivially upper bounded by the number of arrivals during that busy period, conditioned on the event, we have 
\begin{equation}
\label{eq:slow-queue-queue-length-bound}
N_s(t) \leq M, \qquad t \in [0,T]
\end{equation}

Consider the union of departure epochs from HTQ-s and HTQ-f in $[0,T]$: $0=\tau_0 \leq \tau_1 \leq \ldots$. If $\mc J_{f/s}(\tau_k)=\emptyset$ for some $k \geq 0$, then $\mc J_{f/s}(t)=\emptyset$ for all $t \in (\tau_k,\tau_{k+1})$. Hence, the service rate for HTQ-f over the interval $(\tau_k,\tau_{k+1})$ is $v^f(t)$, which, conditioned on the event, is lower bounded by $L^m M^{1-m}=p$ by Lemma \ref{lem:service-rate-bounds}.
Therefore, $p/v^f(t) \leq 1$ over $(\tau_k,\tau_{k+1})$, and hence \eqref{eq:htq-s-speed} implies that all the vehicles with identifiers in $\mc J_f$ will travel slower in HTQ-s in comparison to HTQ-f. In particular, this implies that $\mc J_{f/s}(\tau_{k+1})=\emptyset$. This, combined with the fact that $\mc J_{f/s}(\tau_0)=\emptyset$ (both the queues start from the same initial condition), we get that, conditioned on the event, $\mc J_{s/f}(t) \equiv \emptyset$, and hence $N(t) \leq N_s(t)$ over $[0,T]$. Combining this with \eqref{eq:slow-queue-queue-length-bound} gives that, conditioned on the event, $N(t) \leq M$ over $[0,T]$. 


We now compute the probability of the occurrence of the event using busy period calculations from Section~\ref{sec:busy-period}. The event can be categorized by the maximum number of busy periods, say $r \in \NN$, that overlap with $[0,T]$, i.e., the $r$-th busy period ends after time $T$ (and each of these busy periods has at most $M$ arrivals). Since these busy periods are interlaced with idle periods, the probability of the $r$-th busy period ending after time $T$ is lower bounded by the probability that the sum of the durations of $r$ busy periods is at least $T$. \eqref{eq:G-def} implies that the latter quantity is equal to $\sum_{n=1}^M \int_T^{\infty} G_{r,L^m M^{1-m}}(t,n,\psi,\lambda) \, \de t$. The proposition then follows by noting that this is true for any $r \in \NN$.
%distribution  in \eqref{eq:busy-period-numofarrival-distribution} as $C_{L^m M^{1-m}}(M,\lambda,\psi)$. This probability will then be a lower bound on the unconditional (with respect to the event) probability of $\Nmax \leq M$. 
%Since the maximum queue length during a busy period is upper bounded by the total number of departures over the busy period, we have $N_{bp} \leq M$. This, combined with Lemma \ref{lem:service-rate-bounds} implies that the service rate is at least equal to $L^mM^{1-m} =: \tilde{p}$ during the busy period.  Motivated by our calculations in Section~\ref{sec:busy-period}, we compute bounds on the desired distribution of $N_{bp}$ for the actual queue, say {HTQ-F}, by comparing it with a queue, say {HTQ-S}, having constant service rate $\tilde{p}$. 
%Let consider the same realization for the arrival locations and timings of new vehicles and their desired distances to travel for both systems. Also, let  $N_{bp,f}$ and $N_{bp,s}$ be the total number of vehicles transiting through HTQ-F and HTQ-S, respectively, during a busy period. For those realizations for which $N_{bp,s}\leq M$ during the first busy, it is easy to see that the same property holds for HTQ-F i.e. $N_{bp,f}\leq M$ (see Figure \ref{fig:b1-b2} for an illustration). Because of the memoryless property of the arrival process, the same property holds for all other busy periods as well. Therefore, 
% \begin{equation*}
% \Pr(N_{bp,f}\leq M) \geq \Pr(N_{bp,s}\leq M)
% \end{equation*}
% By noting that $N_{bp}=N_{bn}+1$ for an empty initial condition, and considering \eqref{eq:busy-period-numofarrival-distribution}, we get the result.
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=7.5cm]{b1-b2} 
%\caption{Workload process for two systems under the same realization of the arrival process: a system with slower service rate (solid line) and a system with a faster service rate (dashed line).}
%\label{fig:b1-b2}
%\end{center}
%\end{figure}
\qed
 \end{proof}
 
 \begin{remark}
In the proof of Proposition~\ref{prop:nbp-lower-bound}, when deriving probabilistic upper bound on the queue length over a given time horizon $[0,T]$, we neglected the idle periods in $[0,T]$. This introduces conservatism in the bound on the right hand side of \eqref{eq:nbp-lower-bound}. Since the idle period durations are distributed independently and identically according to an exponential random variable (since the arrival process is Poisson), one could incorporate them into \eqref{eq:nbp-lower-bound} by taking convolution of $G$ with idle period distributions. Our choice for not doing so here is to ensure conciseness in the presentation of bounds in \eqref{eq:nbp-lower-bound}. The resulting conservatism is also present in Proposition~\ref{prop:nbn-lower-bound}, and carries over to Theorems~\ref{thm:superlinear-bound-empty} and \ref{thm:superlinear-bound-non-empty}, as well as to the corresponding simulations reported in Figures~\ref{fig:lambda-m-empty}, \ref{fig:superlinear-large-L} and \ref{fig:phase-transition-non-empty}. 
%the lower bound on the desired probability was 
% 
% 
% In the right hand side of \eqref{eq:sublinear-throughput-zero-initial-condition}, when we optimize over $r$  we are implicitly assuming contiguous busy periods. Therefore, Theorem \ref{thm:superlinear-bound-empty} is conservative. One could relax such an assumption by adding $r$ idle periods. Since the arrival process is Poisson, idle periods can be characterized and the above result can be improved by increasing the time horizon. For the sake of simplicity, we do not take this into account. 
\end{remark}
 
 The next result generalizes Proposition~\ref{prop:nbp-lower-bound} for non-zero initial condition. Note that the non-zero initial condition only affects the first busy period; all subsequent busy periods will necessarily start from with zero initial condition.

 \begin{proposition}\label{prop:nbn-lower-bound}
 For any $m>1$, $M\in\mathbb{N}$, $L>0$, $\lambda >0$, $\varphi\in \Phi$, $\psi \in \Psi$, initial condition $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$, with associated workload $w_0>0$, the probability that the queue length is upper bounded by $M+n_0$ over a given time interval $[0,T]$ satisfies the following: 
 %\ksmargin{should the argument of $C$ be $M+n_0$ instead of $M$ ?}
  $$\Pr \big(N(t) \leq M + n_0 \quad \forall t \in [0,T] \big)\geq \sup_{r \in \NN} \, \sum_{n=1}^M \int_T^{\infty} G_{L^m (M+n_0)^{1-m}}(\delta_{w_0}) * G_{r-1,L^m M^{1-m}}(\psi) (t,n,\lambda) \, \de t$$
 \end{proposition}
 \begin{proof}
The proof is similar to the proof of Proposition \ref{prop:nbp-lower-bound}; however, since we consider $M$ number of new arrivals in each of the busy periods, the \emph{event} of interest is when the queue length in HTQ-s does not exceed $M+n_0$ and $M$ in the first and subsequent busy periods, respectively, while operating with constant service rates $L^m (M+n_0)^{1-m}$ and $L^m M^{1-m}$, respectively. 
\qed
 \end{proof}



 
 %\begin{lemma} \label{lemma:st-order-queulength-nbp}
% The total number of customers served in a busy period of length $B$ is stochastically larger than the queue length in that busy period i.e. 
% $$N_{bp}\geq_{\text{st}}N(t)\;\; \forall t\in[0,B]$$
 %\end{lemma}
 %\begin{proof}
% For any $t\in[0,B]$ and $M\geq 1$, $N_{bp}\leq M$ implies $N(t)\leq M$. However, the converse is not true. This implies that event $N_{bp}\leq M$ is a subset of event $N(t)\leq M$, and therefore, ${\Pr(N(t)\leq M)\geq \Pr(N_{bp}\leq M)}$ which implies ${\Pr(N_{bp}> M)\geq \Pr(N(t)> M)}$. This establishes this lemma. 
% \end{proof}  
 
%  \begin{lemma} \label{lemma:st-order-queulength-nbp}
% For any $m>1$, $L>0$, $\lambda>0$, $\varphi\in\Phi$, $\psi \in \Psi$, a zero initial condition $x_0 =0$, the queue length $N(t)$ is stochastically upper bounded by $N_{bp}$.
% %The total number of customers served in a busy period is stochastically larger than the queue length in that busy period i.e. 
% %$$N_{bp}\geq_{\text{st}}N(t)\quad \forall t\geq 0$$
% \end{lemma}
% \begin{proof}
% Conditioned on the length of the busy period, $B$, 
% \begin{equation*}
% N_{bp}\leq M | B = b \implies N(t)\leq M | B = b \quad \forall t\in[0,b]
% \end{equation*}
% where $t=0$ denotes the time at which the considered busy period starts. Then,
% \begin{equation*}
% \Pr(N_{bp}\leq M | B = b) \leq \Pr(N(t)\leq M | B = b) \quad \forall t\in[0,b]
% \end{equation*}
% and by taking the expectation of the above with respect to length of the busy period, we get 
% \begin{equation*}
%  \Pr(N_{bp}\leq M) \leq \Pr(N(t)\leq M) \quad \forall t>0
% \end{equation*}
% which establishes the lemma. 
% \end{proof}  

%\ksmargin{Lemma~\ref{lemma:st-order-queulength-nbn} probably needs to be removed}
%\kscomment{
%\begin{lemma} \label{lemma:st-order-queulength-nbn}
% For any $m>1$, $L>0$, $\lambda>0$, $\varphi\in\Phi$, $\psi \in \Psi$, an initial condition $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$, with an associated workload $w_0 > 0$, the queue length during the first busy period is stochastically upper bounded by the total number of departures over the first busy period. 
%% 
%% $w_0>0$, $n_0\in\mathbb{N}$%The total number of customers served in a busy period is stochastically larger than the queue length in that busy period i.e. 
%% $$N_{bn}+n_0\geq_{\text{st}}N(t)\quad \forall t\in[0,t_{b_1}]$$
%% where $t_{b_1}$ is the duration of the first busy period. 
% \end{lemma}
% \begin{proof}
%The proof is similar to the proof of Lemma \ref{lemma:st-order-queulength-nbp}. 
% \end{proof}  
%}

%Now, we one can use Proposition \ref{} and Lemma \ref{} in order to probabilistically characterize the throughput of the system. Let fix a $\delta\in[0,1]$ in Definition \ref{}. Then, by Proposition \ref{} and Lemma \ref{}, we have the following relationship,
 %Now, we can establish the following relationship,
 

 We shall use Propositions~\ref{prop:nbp-lower-bound} and \ref{prop:nbn-lower-bound} to establish probabilistic lower bound for a finite time horizon version of the throughput defined in Definition \ref{def:throughput}: for $T>0$, let 
 \begin{equation*}
\label{eq:throughput-def-finite-horizon}
\lambdamax(L,m,\varphi,\psi,x_0,\delta,T):= \sup \left\{\lambda \geq 0: \, \Pr \left( N(t;L, m, \lambda, \varphi, \psi, x_0) < + \infty, \quad \forall t \in [0,T]  \right) \geq 1 - \delta  \right\}.
\end{equation*}
 
% In preparation for the next theorem, we define an additional quantity that can be derived from the busy period calculations in Section~\ref{sec:busy-period}:
%$$
%D_p(M,\lambda,\psi,n,T):=\Pr(\text{number of busy periods in } [0,T] \geq n).
%$$ 
 
%  \begin{theorem}\label{thm:superlinear-bound-empty}
% For $L>0$, $m>1$, $\varphi\in\Phi$, $\psi\in\Psi$, $\delta\in(0,1)$, $T>0$, zero initial condition $x_0=0$, 
% \begin{equation}
% \label{eq:sublinear-throughput-zero-initial-condition}
% \lambda_{\max}(L, m, \varphi, \psi, x_0,\delta,T)\geq \max_{M\geq 1, n \geq 1}\;\max\{\lambda>0 \;| C^{n}_{p}(M,\lambda,\psi) D_p(M,\lambda,\psi,n,T) \geq1-\delta\} 
% \end{equation}
% where $p =L^mM^{1-m}$.
% \end{theorem}
%It is straightforward to derive the following lower bounds on throughput from Propositions~\ref{prop:nbp-lower-bound} and \ref{prop:nbn-lower-bound}. 

\begin{theorem}\label{thm:superlinear-bound-empty}
 For $L>0$, $m>1$, $\varphi\in\Phi$, $\psi\in\Psi$, $\delta\in(0,1)$, $T>0$, zero initial condition $x_0=0$, 
 \begin{equation}
 \label{eq:sublinear-throughput-zero-initial-condition}
 \lambda_{\max}(L, m, \varphi, \psi, x_0,\delta,T)\geq \sup_{M \in \NN}\;\sup \Big\{\lambda \geq 0 \; \Big | \sup_{r \in \NN} \, \sum_{n=1}^M \int_T^{\infty} G_{r,L^m M^{1-m}}(t,n,\psi,\lambda) \, \de t \geq1-\delta \Big\} 
 \end{equation}
% where $p =L^mM^{1-m}$.
 \end{theorem}
 \begin{proof}
Follows from Proposition \ref{prop:nbp-lower-bound}.
\qed
 \end{proof} 
 
% \begin{theorem}\label{thm:superlinear-bound-empty}
% For $L>0$, $m>1$, $\varphi\in\Phi$, $\psi\in\Psi$, $\delta\in(0,1)$, zero initial condition $x_0=0$, 
% \begin{equation}
% \label{eq:sublinear-throughput-zero-initial-condition}
% \lambda_{\max}(L, m, \varphi, \psi, x_0,\delta)\geq \max_{M\geq 1}\;\max\{\lambda>0 \;| C^{}_{L^m M^{1-m}}(M,\lambda,\psi)\geq1-\delta\} 
% \end{equation}
% \end{theorem}
% \begin{proof}
% Let the right hand side of the inequality in \eqref{eq:sublinear-throughput-zero-initial-condition} be denoted by $\lambda_l$. It is sufficient to show that, for $\lambda = \lambda_l$,
% \begin{equation*}
% \Pr(N(t)< +\infty, \;\forall t\geq 0) \geq 1-\delta
% \end{equation*}
%For any $M\in\{2,3\cdots\}$, 
% \begin{equation*}
% \Pr(N(t)< +\infty, \;\forall t\geq 0)\geq \Pr(N(t) \leq M, \;\forall t\geq 0) \geq \Pr(N_{bp}\leq M) \geq  C^{}_{L^m M^{1-m}}(M,\lambda,\psi)
% \end{equation*}
%where the first inequality is trivial, and second and third inequalities follow by  Lemma \ref{lemma:st-order-queulength-nbp} and Proposition \ref{prop:nbp-lower-bound}, respectively. Therefore, based on Definition \ref{def:throughput},  $\tilde \lambda = \max\{\lambda>0 \;| C_{L^m M^{1-m}}(M,\lambda,\psi)=1-\delta\}$ gives a lower bound on $\lambda_{\max}$. In Definition \ref{def:throughput}, however, only boundedness of queue length matters. Thus, one can maximize $\tilde \lambda$ over $M\geq 2$ to get the tightest lower bound. 
% 
% 
% %The above inequality provides a tool to probabilistically characterize the throughput of the system. Let fix a $\delta\in[0,1]$ in Definition \ref{def:throughput} and assume an upper bound, $M$, for the queue length of the system. One can use \eqref{eq:prob-bound-queue} in order to find the maximum $\lambda$ such that 
% %\be\label{eq:relation-queue-nbp}
% %\Pr(N\leq M) \geq B_{L^mM^{1-m}}(N_{bp}\leq M)\geq 1-\delta
% %\ee
% %It should be noted that this $\lambda$ will be a function of $M$ as well as other arguments described in Definition \ref{def:throughput}. The value of $\lambda$ computed in this way ensures that, starting from empty initial condition, the queue length will not exceed $M$ with probability $1-\delta$. 
% \end{proof}
 
 
  \begin{theorem}\label{thm:superlinear-bound-non-empty}
 For $L>0$, $m>1$, $\varphi\in\Phi$, $\psi\in\Psi$, $\delta\in(0,1)$, $T>0$, initial condition $x_0 \in [0,L]^{n_0}$, $n_0 \in \NN$, with associated workload $w_0>0$, 
 \begin{multline*}
 \lambda_{\max}(L, m, \varphi, \psi, x_0,\delta,T) \\ \geq \sup_{M \in \NN}\;\sup \Big \{\lambda>0 \; \Big | \sup_{r \in \NN} \, \sum_{n=1}^M \int_T^{\infty} G_{L^m (M+n_0)^{1-m}}(\delta_{w_0}) * G_{r-1,L^m M^{1-m}}(\psi) (t,n,\lambda)\geq 1-\delta \Big\} 
 \end{multline*}
% \begin{multline*}
% \lambda_{\max}(L, m, \varphi, \psi, x_0,\delta,T) \\ \geq \max_{M_1,M_2\geq 1}\;\max\{\lambda>0 \;| C^{}_{L^m (M_1+n_0)^{1-m}}(M_1-n_0,\lambda,\delta_{w_0})C^{}_{L^m (M_2)^{1-m}}(M_2,\lambda,\psi)\geq (1-\delta)\} 
% \end{multline*}
 \end{theorem}
 \begin{proof}
 Follows from Proposition \ref{prop:nbn-lower-bound}.
 \qed
 \end{proof}
 
 \begin{remark}
 In Theorems~\ref{thm:superlinear-bound-empty} and \ref{thm:superlinear-bound-non-empty}, we implicitly assume the rather standard convention that supremum over an empty set is zero.
 \end{remark}

% \begin{proof}
% Let the right hand side of the above inequality be denoted by $\lambda_l$. Same as Theorem \ref{thm:superlinear-bound-empty}, we need to show that for $\lambda = \lambda_l$,
% \begin{equation*}
% \Pr(N(t)< +\infty, \;\forall t\geq 0) \geq 1-\delta
% \end{equation*}
%However, for non-zero initial condition, we also need to show that queue length during the first busy period, i.e. $t\in[0,t_{b_1}]$  remains bounded. For any $M_1\in{\{n_0,n_0+1,\cdots\}}$ and $M_2\in\{2,3\cdots\}$, 
% \begin{align*}
% \Pr(N(t)< +\infty, \;\forall t\geq 0)&\geq \Pr(N(t) \leq M_1, \;\forall t\geq [0,t_{b_1}]) \times\Pr(N(t) \leq M_2, \;\forall t> t_{b_1}) \nonumber \\
% &\geq \Pr(N_{bn}+n_0\leq M_1) \times \Pr(N_{bp}\leq M_2)\nonumber \\
% &  \geq  C^{}_{L^m (M_1+n_0)^{1-m}}(M_1-n_0,\lambda,\delta_{w_0})\times C^{}_{L^m M_2^{1-m}}(M_2,\lambda,\psi)
% \end{align*}
%where the first inequality is trivial, second one follows by by Lemmas \ref{lemma:st-order-queulength-nbp} and \ref{lemma:st-order-queulength-nbn} and the last inequality follows by Propositions \ref{prop:nbp-lower-bound} and \ref{prop:nbn-lower-bound}. Therefore, based on Definition \ref{def:throughput},  
%$${\tilde \lambda = \max\{\lambda>0 \;| C^{}_{L^m (M_1+n_0)^{1-m}}(M_1-n_0,\lambda,\delta_{w_0})C^{}_{L^m (M_2)^{1-m}}(M,\lambda,\psi)=1-\delta\} }$$
% gives a lower bound on $\lambda_{\max}$. In Definition \ref{def:throughput}, however, only boundedness of queue length matters. Thus, one can maximize $\tilde \lambda$ over $M_1$ and $M_2$ to get the tightest lower bound. 
% \end{proof}
 
 %In order to further clarify the analysis in this section, the following example shows the application of these results in order to probabilistically characterize the throughput of the system for a specific spatial distribution. 
 
% \begin{example}[Deterministic traveled distances] Assume that vehicles, upon arrival, wish to travel a deterministic distance of length $L>0$ i.e. $\varphi(x)=\delta_{\{x=L\}}$ and their motion is determined by a car following model with $m>1$. Also, further assume that the queue length does not exceed $M\in\{2,3,\cdots\}$. In this case, the lower bound on the service rate is $p=L^mM^{1-m}$. Application of \eqref{eq:busy-period-and-nbp-joint} gives,
 % \be\label{eq:busy-period-joint-deterministic}
 % D_p(t,N_{bp}=n) = \int_0^te^{-\lambda y}\frac{(\lambda y)^{n-1}}{n!}\delta_{\{y=nL/p\}}\de y=\begin{cases}0 & t\leq nL/p\\ e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!}& t> nL/p\end{cases}
%  \ee
% and by \eqref{eq:nbp-dist},
%\be
%B_p(N_{bp}=n)= e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!}
%\ee
%and by Lemma \ref{lemma:st-order-queulength-nbp} and Proposition \ref{prop:nbp-lower-bound},
%\be
% \Pr(N\leq M)\geq \Pr(N_{bp}\leq M)\geq C_{L^m M^{1-m}}(M,\lambda) = \sum_{i=1}^M e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!} \geq1-\delta.
%\ee
%The above inequality can be used in order to find the maximum throughput for which queue length remains bounded by $M$ with probability of at least $1-\delta$.
% \end{example}



==> 02- submission/throughput-analysis.tex <==
\section{Throughput Analysis}
\label{sec:throughput-analysis}

\input{linear}

\input{nonlinear}

\input{super-linear}

%\input{sublinear}

\input{sublinear-new}

==> busy-period.tex <==
\subsection{Analysis for $m>1$ case}
In this section, we assume that system starts from an empty initial condition and then we derive a probabilistic lower bound on the throughput of the system. For our analysis we focus on busy period and the number of vehicles served in a busy period. 

We first assume an upper bound on the queue length, i.e. $N(t)\leq M \; \forall t\geq0$, which by Lemma \ref{lem:service-rate-bounds} gives a lower bound on the service rate of the system i.e. $s(y(t))\geq L^mM^{1-m}\; \forall t\geq 0$. Then, we use this lower bound on the service rate to compare the system with a system with the same temporal-spatial arrival process but a slower decrease rate of workload . We use this comparison as a tool to find a lower bound on the probability of achieving the assumed upper bound on the queue length. This result leads to a probabilistic lower bound on the throughput of the system which is stated in Theorem \ref{}. Our analysis heavily depends on the probability distribution of busy periods which is described in the next section.


 
 \subsubsection{From busy period to throughput}
%\begin{lemma}\label{lemma:cdf-poisson}
%\mmmargin{find a proper reference}
%The cumulative distribution function of a Poisson random variable with mean $\mu > 0$ is decreasing in $\mu$.
%\end{lemma}
%\begin{proof}
%Let $X$ be a Poisson random variable with mean $\mu > 0$, then the cdf of $X$ for a fixed $n\in\mathbb{N}$ is given as \cite{?},\
%\be
%f(\mu) = \Pr(X\leq n) = \frac{\int_{\mu}^\infty t^{n}e^{-t}\de t}{n!}
%\ee 
%Since the integrand in the numerator is positive, the above function is decreasing in $\mu$.
%\end{proof}


 
  \begin{proposition}\label{prop:nbp-lower-bound}
 For any $m>1$, $w_0=0$, $L>0$, $\lambda > 0$ $\varphi \in \Psi$ and $M\in\{2,3,\cdots\}$, given $N(t)<M$ $\forall t>0$, then 
  $$\Pr(N_{bp}\leq M)\geq C^{(2)}_{L^m M^{1-m}}(M,\lambda)\qquad \forall n\in\mathbb{N}$$
 \end{proposition}
 \begin{proof}
 \mmmargin{service is not greater than this lower bound for all t because of idle time. revise it}
 For $m>1$, by Lemma \ref{lem:service-rate-bounds}, and the upper bound given on the queue length,
 \be
 s(t)\geq L^mM^{1-m} = p \quad \forall t>0
 \ee 
 
 We consider another system with the same realization of temporal-spatial arrival process but fixed service rate of $p$ and name it as the \emph{slower} system. Let $B_1$ and $B_2$ be random variables that denote the length of a busy period in actual and slower system, respectively. Since the realization of arrival processes are the same for both systems, and the decrease rate of workload in slower system is smaller it is clear that,
 \be\label{eq:workload-actual-slower}
 w_1(t)\leq w_2(t) \quad \forall t>0
 \ee
where $w_1(t)$ and $w_2(t)$ denote the the workload processes in actual and slower system, respectively. 

Now, let $t_s$ be the time at which a (random) busy period in the slower system ends and $t_1$ be the time at which the next busy period in that system ends (see Figure \ref{fig:b1-b2} for an illustration). Obviously, $w_1(t_s)=w_1(t_f)=0$. Also, by \eqref{eq:workload-actual-slower}, $w_2(t_s)=w_2(t_f)=0$. Let $t_1\in(t_s,t_f)$ be the time of the first arrival after $t=t_s$. Note that this time is the same in both systems. Therefore, in the slower system, the busy period that lies in $[t_s,t_f]$ has the length of $t_f-t_1$.  Let $t_2\in[t_1,t_f]$ be the time at which the actual system gets idle for the first time after $t=t_1$. We want to show that $t_2\leq t_f$. By contradiction, assume $t_2> t_f$. Thus, $w_1(t_f)>0$, but $w_2(t_f)=0$. This contradicts \eqref{eq:workload-actual-slower} and proves that $t_2\leq t_f$. This implies that the longest busy period in actual system contained in $[t_s,t_f]$ is no longer than the busy period in actual system. This argument holds for any busy period in slower system. Thus,  with probability one, 
 \be\label{eq:relation-b1-b2}
 B_1\leq B_2
 \ee  
 
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=9cm]{b1-b2} 
\caption{Workload process for two systems with the same realization temporal-spatial arrival process, a system with slower service rate (solid line) and a system with a faster service rate (dashed line).}
\label{fig:b1-b2}
\end{center}
\end{figure}

Now, let $N_{bp}$ and $\tilde N_{bp}$ be the number of customers served in a busy period in the actual system and slower system, respectively. Note that $N_{bp}$ and $\tilde{N}_{bp}$ are Poisson random variables with mean $\lambda B_1$ and $\lambda B_2$, respectively and by \eqref{eq:relation-b1-b2}, $\lambda B_1\leq \lambda B_2$. Poisson random variable is stochastically increasing in its mean (see e.g. \cite{Ross:96}), therefore
\be
\tilde{N}_{bp}\geq_{\text{st}}{N}_{bp}
\ee 
which establishes this proposition. %There exists a random variable $B_1^*$, independent of $B_2$, with the same distribution of $B_1$ such that, with probability one, $B_1^*\leq B_2$. Now, consider two Possoin random variables with means $\lambda B_1^*$ and $\lambda B_2$. Thus, by Lemma \ref{lemma:cdf-poisson}, $f(\lambda B_1^*)\geq f(\lambda B_2)$. Therefore, for any $M\in\mathbb{N}$,
 %\be
 %f(\lambda B_1^*)\leq f(\lambda B_2)
 %\ee 
 \end{proof}
 
\mmmargin{have we defined this notation ($n_0$) earlier?}
 \begin{proposition}\label{prop:nbn-lower-bound}
 For any $m>1$, $w_0>0$, \mmcomment{$n_0\in\mathbb{N}$}, $L>0$, $\lambda > 0$, $\varphi \in \Psi$ and $M\in\{2,3,\cdots\}$, given $N(t)<M$ $\forall t>0$, then 
  $$\Pr(N_{bn}\leq M)\geq C^{(1)}_{L^m (M+n_0)^{1-m}}(M,\lambda,w_0)\qquad \forall n\in\mathbb{N}$$
 \end{proposition}
 \begin{proof}
 The proof is very similar to the proof of Proposition \ref{prop:nbp-lower-bound}; however, in this case the upper bound on the queue length is $M+n_0$, and the lower bound on the service rate is $L^m(M+n_0)^{1-m}$. 
 \end{proof}



 
 %\begin{lemma} \label{lemma:st-order-queulength-nbp}
% The total number of customers served in a busy period of length $B$ is stochastically larger than the queue length in that busy period i.e. 
% $$N_{bp}\geq_{\text{st}}N(t)\;\; \forall t\in[0,B]$$
 %\end{lemma}
 %\begin{proof}
% For any $t\in[0,B]$ and $M\geq 1$, $N_{bp}\leq M$ implies $N(t)\leq M$. However, the converse is not true. This implies that event $N_{bp}\leq M$ is a subset of event $N(t)\leq M$, and therefore, ${\Pr(N(t)\leq M)\geq \Pr(N_{bp}\leq M)}$ which implies ${\Pr(N_{bp}> M)\geq \Pr(N(t)> M)}$. This establishes this lemma. 
% \end{proof}  
 
  \begin{lemma} \label{lemma:st-order-queulength-nbp}
 For any $m>1$, $L>0$, $\lambda>0$, $\varphi \in \Psi$, $w_0=0$,%The total number of customers served in a busy period is stochastically larger than the queue length in that busy period i.e. 
 $$N_{bp}\geq_{\text{st}}N(t)\quad \forall t\geq 0$$
 \end{lemma}
 \begin{proof}
 Conditioned on the length of busy period, $B$, 
 \be
 N_{bp}\leq M | B = b \implies N(t)\leq M | B = b \quad \forall t\in[0,b]
 \ee
 where here $t=0$ denotes the time at which busy period starts. Then,
 \be
 \Pr(N_{bp}\leq M | B = b) \leq \Pr(N(t)\leq M | B = b) \quad \forall t\in[0,b]
 \ee
 and by taking the expectation of the above with respect to length o busy period, we get 
 \be
  \Pr(N_{bp}\leq M) \leq \Pr(N(t)\leq M) \quad \forall t>0
 \ee
 which establishes this lemma. 
 \end{proof}  

%Now, we one can use Proposition \ref{} and Lemma \ref{} in order to probabilistically characterize the throughput of the system. Let fix a $\delta\in[0,1]$ in Definition \ref{}. Then, by Proposition \ref{} and Lemma \ref{}, we have the following relationship,
 %Now, we can establish the following relationship,
 Now, we are ready to state the main result in the following theorem which gives a probabilistic lower bound on the throughput of the system for $m>1$.
 \begin{theorem}
 Given $\delta\in(0,1)$, $L>0$, $m>1$, $\varphi\in\Psi$, $w_0=0$, then
 $$\lambda_{\max}(m, L, \varphi,\delta)\geq \max_{M\geq 2}\;\max\{\lambda>0 \;| C^{(2)}_{L^m M^{1-m}}(M,\lambda)\geq1-\delta\}$$
 \end{theorem}
 \begin{proof}
For a given upper bound on the queue length, $M\in\{2,3\cdots\}$, 
 \be\label{eq:prob-bound-queue}
 \Pr(N\leq M) \geq \Pr(N_{bp}\leq M) \geq  C^{(2)}_{L^m M^{1-m}}(M,\lambda)
 \ee
 where the first inequality follows by Lemma \ref{lemma:st-order-queulength-nbp} and the second inequality follows by Proposition \ref{prop:nbp-lower-bound}. Therefore, based on Definition \ref{def:throughput},  $\tilde \lambda = \max\{\lambda>0 \;| C_{L^m M^{1-m}}(M,\lambda)=1-\delta\}$ gives a lower bound on $\lambda_{\max}$. In Definition \ref{def:throughput}, however, only boundedness of queue length matters. Thus, one can maximize $\tilde \lambda$ over $M\geq 2$ to get tighter lower bound. 
 
 
 %The above inequality provides a tool to probabilistically characterize the throughput of the system. Let fix a $\delta\in[0,1]$ in Definition \ref{def:throughput} and assume an upper bound, $M$, for the queue length of the system. One can use \eqref{eq:prob-bound-queue} in order to find the maximum $\lambda$ such that 
 %\be\label{eq:relation-queue-nbp}
 %\Pr(N\leq M) \geq B_{L^mM^{1-m}}(N_{bp}\leq M)\geq 1-\delta
 %\ee
 %It should be noted that this $\lambda$ will be a function of $M$ as well as other arguments described in Definition \ref{def:throughput}. The value of $\lambda$ computed in this way ensures that, starting from empty initial condition, the queue length will not exceed $M$ with probability $1-\delta$. 
 \end{proof}
 
 
  \begin{theorem}
 Given $\delta_1,\delta_2\in(0,1)$, $L>0$, $m>1$, $\varphi\in\Psi$, $w_0>0$, $n_0\in\mathbb{N}$ then
 $$\lambda_{\max}(m, L, \varphi,\delta)\geq \max_{M_1,M_2\geq 2}\;\max\{\lambda>0 \;| C^{(1)}_{L^m (M+n_0)^{1-m}}(M,\lambda,w_0)C^{(2)}_{L^m (M_2)^{1-m}}(M,\lambda)\geq(1-\delta_1)(1-\delta_2)\geq (1-\delta)\}$$
 \end{theorem}
 \begin{proof}
\mmcomment{work in progress ...} 
 
 \end{proof}
 
 In order to further clarify the analysis in this section, the following example shows the application of these results in order to probabilistically characterize the throughput of the system for a specific spatial distribution. 
 
 \begin{example}[Deterministic traveled distances] Assume that vehicles, upon arrival, wish to travel a deterministic distance of length $L>0$ i.e. $\varphi(x)=\delta_{\{x=L\}}$ and their motion is determined by a car following model with $m>1$. Also, further assume that the queue length does not exceed $M\in\{2,3,\cdots\}$. In this case, the lower bound on the service rate is $p=L^mM^{1-m}$. Application of \eqref{eq:busy-period-and-nbp-joint} gives,
  \be\label{eq:busy-period-joint-deterministic}
  D_p(t,N_{bp}=n) = \int_0^te^{-\lambda y}\frac{(\lambda y)^{n-1}}{n!}\delta_{\{y=nL/p\}}\de y=\begin{cases}0 & t\leq nL/p\\ e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!}& t> nL/p\end{cases}
  \ee
% and by \eqref{eq:nbp-dist},
%\be
%B_p(N_{bp}=n)= e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!}
%\ee
and by Lemma \ref{lemma:st-order-queulength-nbp} and Proposition \ref{prop:nbp-lower-bound},
\be
 \Pr(N\leq M)\geq \Pr(N_{bp}\leq M)\geq C_{L^m M^{1-m}}(M,\lambda) = \sum_{i=1}^M e^{-\lambda nL/p}\frac{(\lambda nL/p)^{n-1}}{n!} \geq1-\delta.
\ee
The above inequality can be used in order to find the maximum throughput for which queue length remains bounded by $M$ with probability of at least $1-\delta$.
 \end{example}


